Supersonic OT: Fast Unconditionally Secure Oblivious Transfer

Oblivious Transfer (OT) is a fundamental cryptographic protocol with applications in secure Multi-Party Computation, Federated Learning, and Private Set Intersection. With the advent of quantum computing, it is crucial to develop unconditionally secure core primitives like OT to ensure their continued security in the post-quantum era. Despite over four decades since OT's introduction, the literature has predominantly relied on computational assumptions, except in cases using unconventional methods like noisy channels or a fully trusted party. Introducing "Supersonic OT", a highly efficient and unconditionally secure OT scheme that avoids public-key-based primitives, we offer an alternative to traditional approaches. Supersonic OT enables a receiver to obtain a response of size O(1). Its simple (yet non-trivial) design facilitates easy security analysis and implementation. The protocol employs a basic secret-sharing scheme, controlled swaps, the one-time pad, and a third-party helper who may be corrupted by a semi-honest adversary. Our implementation and runtime analysis indicate that a single instance of Supersonic OT completes in 0.35 milliseconds, making it up to 2000 times faster than the state-of-the-art base OT.

==> DQ-OT-Proof.tex <==



%%%%%%%%%%%% Proof %%%%%%%%%%%%%%%%%




\subsection{DQ-OT's Security Proof}\label{sec::DQ-OT-proof}
Below, we prove  DQ-OT's security, i.e., Theorem \ref{theo::DQ-OT-sec}.  


\begin{proof}
We consider the case where each party is corrupt, at a time.

\subsubsection{Corrupt Receiver \re} In the real execution, \re's view is: 

$\view_{\re}^{\st DQ\text{-}OT}\big(m_{\st 0}, m_{\st 1}, \empt,$ $  \empt, s\big) = \{r_{\st\re}, g, C, p, e_{\st 0}, e_{\st 1}, m_{\st s} \}$, where $g$ is a random generator, $C=g^{\st a}$ is a random public parameter, $a$ is a random value, $p$ is a large random prime number, and $r_{\st \re}$ is the outcome of the internal random coin of  \re and is used to generate $(r_{\st 1}, r_{\st 2})$.  
%
 Below, we construct an idea-model simulator  $\simm_{\st\re}$ which receives $(s, m_{\st s})$ from \re. 
 
 \begin{enumerate}
 %
 \item initiates an empty view and appends uniformly random coin $r'_{\st\re}$ to it, where $r'_{\st\re}$ will be used to generate \re-side randomness. 
%
It chooses a large random prime number $p$ and a random generator $g$.



%%%%%



 
 %
 \item sets $(e'_{\st 0}, e'_{\st 1})$ as follows: 
 %
 \begin{itemize}
 %
 \item splits $s$ into two shares: $\ses(1^{\st\lambda}, s, 2, 2)\rightarrow (s'_{\st 1}, s'_{\st 2})$.
 %
 \item picks uniformly random values: $C', r'_{\st 1}, r'_{\st 2},y'_{\st 0}, y'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.
 %
 %\item picks two additional uniformly random values: $y'_1, y'_2\stackrel{\$}\leftarrow\mathbb{Z}_{p-1}$.
 %
 \item sets $\beta'_s=g^{\st x}$, where $x$ is set as follows: 
 %
 \begin{itemize}
 %
 \item[$*$] $x = r'_{\st 2} + r'_{\st 1}$, if $(s = s_{\st 1} = s_{\st 2} = 0)$ or $(s = s_{\st 1} = 1\wedge s_{\st 2} = 0)$.
 %
 \item[$*$] $x = r'_{\st 2} - r'_{\st 1}$, if $(s =0 \wedge s_{\st 1} = s_{\st 2} = 1)$ or $(s = s_{\st 2} = 1\wedge s_{\st 1} = 0)$.
 %
 \end{itemize}
 %
 \item picks a uniformly random value $u\stackrel{\st\$}\leftarrow\mathbb{Z}_{p}$ and then sets $e'_{\st s} = (g^{\st y'_s}, \h(\beta'^{\st y'_s}_{\st s})\oplus m_{\st s})$ and $e'_{\st 1-s} = (g^{\st y'_{\st 1-s}}, u)$. 
 %
 \end{itemize}
 %
 \item  appends $(g, C', p, r'_{\st 1}, r'_{\st 2},  e'_{\st 0}, e'_{\st 1}, m_{\st s})$ to the view and outputs the view.
 %
 \end{enumerate}
 
 Now we discuss why the two views in the ideal and real models are indistinguishable. Since we are in the semi-honest model, the adversary picks its randomness according to the protocol description; thus, $r_{\st \re}$ and $r'_{\st \re}$ model have identical distributions, so do values $(r_{\st 1}, r_{\st 2})$ in the real model and $(r'_{\st 1}, r'_{\st 2})$ in the ideal model. Also, $C$ and $C'$ have been picked uniformly at random and have identical distributions. The same applies to values $g$ and $p$ in the real and ideal models. 
 
 
 Next, we argue that  $e_{\st 1-s}$ in the real model and $e'_{\st 1-s}$ in the ideal model are indistinguishable. In the real model, it holds that $e_{1-s}=(g^{\st y_{\st 1-s}}, \h(\beta^{y_{1-s}}_{\st 1-s})\oplus m_{\st 1-s})$, where $\beta^{\st y_{\st 1-s}}_{\st 1-s}=\frac{C}{g^{\st x}}=g^{\st a-x}$. Since $y_{\st 1-s}$ in the real model and $y'_{\st 1-s}$ in the ideal model have been picked uniformly at random and unknown to the adversary/distinguisher, $g^{\st y_{\st 1-s}}$ and $g^{\st y'_{\st 1-s}}$  have identical distributions. 
 
 
 
 
 Furthermore, in the real model, given $C=g^{\st a}$, due to DL problem, $a$ cannot be computed by a PPT adversary. Also, due to CDH assumption, \re cannot compute  $\beta^{y_{1-s}}_{1-s}$ (i.e., the input of $\h(.)$), given $g^{\st y_{\st 1-s}}$ and $g^{\st a-x}$. We also know that $\h(.)$ is modelled as a random oracle and its output is indistinguishable from a random value. Thus,  $\h(\beta^{\st y_{\st 1-s}}_{\st 1-s})\oplus m_{\st 1-s}$ in the real model and $u$ in the ideal model are indistinguishable. This means that $e_{\st 1-s}$ and $e'_{\st 1-s}$ are indistinguishable too, due to DL, CDH, and RO assumptions. Also, in the real and idea models, $e_{\st s}$ and $e'_{\st s}$ have been defined over $\mathbb{Z}_{\st p}$ and their decryption always result in the same value $m_{\st s}$. Thus, $e_{\st s}$ and $e'_{\st s}$ have identical distributions too. 
%
Also, $m_{\st s}$ has identical distribution in both models. 

We conclude that the two views are computationally indistinguishable, i.e., Relation \ref{equ::reciever-sim-} (in Section \ref{sec::sec-def}) holds. 



\subsubsection{Corrupt Sender \se} In the real model, \se's view is: 

$\view_{\se}^{\st DQ\text{-}OT}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, $ $s\big)= \{r_{\st\se}, C, \beta_{\st 0}, \beta_{\st 1}\}$, where $r_{\st \se}$ is the outcome of the internal random coin of  \se.  Next, we construct an idea-model simulator  $\simm_{\st\se}$ which receives $(m_{\st 0}, m_{\st 1})$ from \se. 

\begin{enumerate}
\item constructs an empty view and appends uniformly random coin $r'_{\st\se}$ to it, where $r'_{\st\se}$ will be used to generate random values for \se.
%
%\item picks two random values $r'_0, r'_1\stackrel{\$}\leftarrow\mathbb{Z}_{p-1}$.

\item picks random values $C', r'\stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.

\item sets $\beta'_{\st 0}=g^{\st r'}$ and $\beta'_{\st 1}=\frac{C'}{g^{\st r'}}$. 

\item appends $\beta'_{\st 0}$ and $\beta'_{\st 1}$ to the view and outputs the view. 

\end{enumerate}


Next, we explain why the two views in the ideal and real models are indistinguishable. Recall, in the real model, $(\beta_{\st s}, \beta_{\st 1-s})$ have the following form: $\beta_{s}=g^{\st x}$ and  $\beta_{\st 1-s}=g^{\st a-x}$, where $a=DL(C)$ and $C=g^{\st a}$. In this model, because $a$ and $x$ have been picked uniformly at random and unknown to the adversary, due to DL assumption,  $\beta_{\st s}$ and $\beta_{\st 1-s}$ have identical distributions and are indistinguishable. In the ideal model, $r'$ has been picked uniformly at random and we know that $a'$ in $C' = g^{\st a'}$ is a uniformly random value, unknown to the adversary; therefore, due to DL assumption, $\beta'_{\st 0}$ and $\beta'_{\st 1}$ have identical distributions too. Moreover, values $\beta_{\st s}, \beta_{\st 1-s}, \beta'_{\st 0}$, and $\beta'_{\st 1}$  have been defined over the same field, $\mathbb{Z}_{\st p}$. Thus, they have identical distributions and are indistinguishable. 

Therefore, the two views are computationally indistinguishable, i.e., Relation \ref{equ::sender-sim-} (in Section \ref{sec::sec-def}) holds.


\subsubsection{Corrupt Server $\p_{\st 2}$}  
 
 In the real execution, $\p_{\st 2}$'s view is: 
 
$\view_{\p_2}^{\st DQ\text{-}OT}\big((m_{\st 0}, m_{\st 1}), \empt,$ $ \empt, s\big)=\{g, C, p, s_{\st 2}, r_{\st 2}\}$. Below, we show how an ideal-model simulator $\simm_{\st \p_{\st 2}}$ works. 

\begin{enumerate}
%
\item initiates an empty view. It selects a random generator $g$ and a large random prime number $p$.
%
\item picks two uniformly random values $s'_{\st 2}\stackrel{\st\$}\leftarrow\mathbb U$ and $C', r'_{\st 2}\stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$, where $\mathbb{U}$ is the output range of $\ses(.)$. 
%
\item appends $s'_{\st 2}, C'$ and $r'_{\st 2}$ to the view and outputs the view. 
%
\end{enumerate}

Next, we explain why the views in the ideal and real models are indistinguishable.

Since values $g$ and $p$ have been picked uniformly at random in both models, they  have identical distributions in the real and ideal models. 
%
Since $r_{\st 2}$ and $r'_{\st 2}$ have been picked uniformly at random from  $\mathbb{Z}_{\st p}$, they have identical distributions. Also, due to the security of $\ses(.)$ each share $s_{\st 2}$ is indistinguishable from a random value $s'_{\st 2}$, where $s'_{\st 2}\in \mathbb{U}$. Also, both $C$ and $C'$ have been picked uniformly at random from $\mathbb{Z}_{\st p}$; therefore, they have identical distribution. 


Thus, the two views are computationally indistinguishable, i.e., Relation \ref{equ::server-sim-} w.r.t. $\p_{\st 2}$ (in Section \ref{sec::sec-def}) holds.



\subsubsection{Corrupt Server $\p_{\st 1}$}  


In the real execution, $\p_{\st 1}$'s view is: 
 
$\view_{\st\p_1}^{\st DQ\text{-}OT}\big((m_{\st 0}, m_{\st 1}), \empt,$ $ \empt, s\big)=\{ g, C, p, s_{\st 1}, r_{\st 1}, \delta_{\st 0}, \delta_{\st 1}\}$. Ideal-model $\simm_{\st\p_{1}}$ works as follows.  


\begin{enumerate}
%
\item initiates an empty view. It chooses a random generator $g$ and a large random prime number $p$. 
%
\item picks two random values $\delta'_{\st 0}, \delta'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$. 
%
\item picks two uniformly random values $s'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb U$ and \\  $C', r'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$, where $\mathbb{U}$ is the output range of $\ses(.)$. 
%
\item appends  $s'_{\st 1}, C', r'_{\st 1}, \delta'_{\st 0}, \delta'_{\st 1}$ to the view and outputs the view. 
 %
\end{enumerate}

Now, we explain why the views in the ideal and real models are indistinguishable. Values $g$ and $p$ have been picked uniformly at random in both models. Hence, $g$ and $p$ in the real and ideal models have identical distributions (pair-wise). 



Recall, in the real model, $\p_{\st 1}$ receives $\delta_{\st s_{\st 2}}=g^{\st r_{\st 2}}$ and  $\delta_{\st 1- s_2}=g^{\st a- r_2}$ from  $\p_{\st 2}$. 
%
Since $a$ and $r_{\st 2}$ have been picked uniformly at random and unknown to the adversary due to DL assumption,   $\delta_{\st s_2}$ and $\delta_{\st 1-{s_2}}$ (or $\delta_{\st 0}$ and $\delta_{\st 1}$) have identical distributions and are indistinguishable from random values (of the same field). 

In the ideal model, $\delta'_{\st 0}$ and  $\delta'_{\st 1}$ have been picked uniformly at random; therefore, they have identical distributions too. Moreover,  $\delta_{\st s}, \delta_{\st 1-s}, \delta'_{\st 0}$, and $\delta'_{\st 1}$  have been defined over the same field, $\mathbb{Z}_{\st p}$. So, they have identical distributions and are indistinguishable. 
%
Due to the security of $\ses(.)$ each share $s_{\st 1}$ is indistinguishable from a random value $s'_{\st 1}$, where $s'_{\st 1}\in \mathbb{U}$. Also, $(r_{\st 1}, C)$ and $(r'_{\st 1}, C')$ have identical distributions, as they are picked uniformly at random from $\mathbb{Z}_{\st p}$.


Hence, the two views are computationally indistinguishable, i.e., Relation \ref{equ::server-sim-} w.r.t. $\p_{\st 1}$ (in Section \ref{sec::sec-def}) holds.
%
%\hfill\(\Box\) 
\end{proof}

==> DQ-OT-proof-of-correctness.tex <==

\subsection{Proof of Correctness}\label{sec::DQ-OT-proof-of-correctness}

In this section, we discuss why the correctness of DQ-OT always holds. Recall, in the original OT of Naor and Pinkas \cite{Efficient-OT-Naor}, the random value $a$ (i.e., the discrete logarithm of random value $C$) is inserted by receiver \re into the query $\beta_{\st 1-s}$ whose index (i.e., $1-s$) is not interesting to \re while the other query $\beta_{\st s}$ is free from value $a$. As we will explain below, in our DQ-OT, the same applies to the final queries that are sent to \se.  
%
Briefly, in DQ-OT, when:

\begin{itemize}

\item[$\bullet$]  $s=s_{\st 1}\oplus s_{\st 2}=1$ (i.e., when $s_{\st 1}\neq s_{\st 2}$), then $a$ will always appear in $\beta_{\st 1-s}=\beta_{\st 0}$; however, $a$ will not appear in $\beta_{\st 1}$. 

\item[$\bullet$] $s=s_{\st 1}\oplus s_{\st 2} = 0$ (i.e., when $s_{\st 1}=s_{\st 2}$), then $a$ will always appear in $\beta_{\st 1-s}=\beta_{\st 1}$; but $a$ will not appear in $\beta_{\st 0}$.

\end{itemize}

This is evident in Table~\ref{tab:analysis} which shows what
$\delta_{\st i}$ and $\beta_{\st j}$ are for the different values of $s_{\st 1}$ and $s_{\st 2}$. Therefore, the query pair ($\beta_{\st 0}, \beta_{\st 1}$) has the same structure as it has in \cite{Efficient-OT-Naor}. 

%\vspace{-1mm}

\begin{table}[h]
%\vspace{-1mm}
\begin{center}
\scalebox{.76}{
  \begin{tabular}{|l||p{4.5cm}|p{4.5cm}|}
\hline
    &\multicolumn{1}{c|}{$s_{\st 2}=0$}&\multicolumn{1}{c|}{$s_{\st 2}=1$}\\
\hline
\hline
&\cellcolor{gray!20}$\delta_{\st 0} = g^{\st r_2}$, \hspace{3mm} $\delta_{\st 1} = g^{\st a-r_2}$&\cellcolor{gray!20} $\delta_{\st 0}=g^{\st a-r_2}$,\hspace{3mm} $\delta_{\st 1}=g^{\st r_2}$\\
\multirow{-2}{*}{$s_{\st 1}=0$}&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st r_2+r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st a-r_2-r_1}$&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st a-r_2+r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st r_2-r_1}$\\
\hline
&\cellcolor{gray!20}$\delta_{\st 0}=g^{\st r_2}$, \hspace{3mm} $\delta_{\st 1}=g^{\st a-r_2}$&\cellcolor{gray!20}$\delta_{\st 0}=g^{\st a-r_2}$, \hspace{3mm} $\delta_{\st 1}=g^{\st r_2}$\\
\multirow{-2}{*}{$s_{\st 1}=1$}&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st a-r_2-r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st r_2+r_1}$&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st r_2-r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st a-r_2+r_1}$\\
\hline
\end{tabular}
}
\end{center}
\caption{$\delta_{\st i}$ and $\beta_{\st j}$ are for the different values of $s_{\st 1}$ and $s_{\st 2}$.
We express each value as a power of $g$.}
\label{tab:analysis}
%\vspace{-3mm}
\end{table}

Next, we show why, in DQ-OT, \re can extract the correct message, i.e., $m_s$. Given \se's reply pair $(e_{\st 0}, e_{\st 1})$ and its original index $s$, \re knows which element to pick from the response pair, i.e., it picks $e_{\st s}$.  


%\vspace{-1mm}
Moreover, given $g^{\st y_s}\in e_{\st s}$, \re can  recompute $\h(g^{\st y_s})^{\st x}$, as it knows the value of $s, s_{\st 1}$, and $s_{\st 2}$.  Specifically, as Table~\ref{tab:analysis} indicates, when: 

\begin{itemize}
\item[$\bullet$]  $\overbrace{(s= s_{\st 1}=s_{\st 2}=0)}^{\st \text{Case 
 1}}$ or $\overbrace{(s=s_{\st 1}=1 \wedge s_{\st 2}=0)}^{\st \text{Case 
 2}}$, then \re can set $x = r_{\st 2} + r_{\st 1}$.

\begin{itemize}

 \item In Case 1, it holds $\h((g^{\st y_0})^{\st x})= \h((g^{\st y_0})^{\st r_2 +r_1})=q$. Also, $e_{\st 0}=\h(\beta_{\st 0}^{\st y_0})\oplus m_{\st 0}=\h((g^{\st r_2+r_1})^{\st y_0})\oplus m_{\st 0}$. Thus, $q\oplus e_{\st 0}=m_{\st 0}$.
 
 \item In Case 2, it holds $\h((g^{\st y_1})^{\st x})= \h((g^{\st y_1})^{\st r_2 +r_1})=q$. Moreover, $e_{\st 1}=\h(\beta_{\st 1}^{\st y_1})\oplus m_{\st 1}=\h((g^{\st r_2+r_1})^{\st y_1})\oplus m_{\st 1}$. Hence, $q\oplus e_{\st 1}=m_{\st 1}$.

 
 \end{itemize}

 \vspace{.6mm} 
 
%
\item[$\bullet$]  $\overbrace{(s=0 \wedge s_{\st 1}=s_{\st 2}=1)}^{\st \text{Case 
 3}}$ or $\overbrace{(s=s_{\st 2}=1 \wedge s_{\st 1}=0)}^{\st \text{Case 
 4}}$, then \re can set $x = r_{\st 2} - r_{\st 1}$.
%

\begin{itemize}

 \item In Case 3, it holds $\h((g^{\st y_0})^{\st x})= \h((g^{\st y_0})^{\st r_2 - r_1})=q$. On the other hand, $e_{\st 0}=\h(\beta_{\st 0}^{\st y_0})\oplus m_{\st 0}=\h((g^{\st r_2 - r_1})^{\st y_0})\oplus m_{\st 0}$. Therefore, $q\oplus e_{\st 0}=m_{\st 0}$.
 
 \item In Case 4, it holds $\h((g^{\st y_1})^{\st x})= \h((g^{\st y_1})^{\st r_2 -r_1})=q$. Also, $e_{\st 1}=\h(\beta_{\st 1}^{\st y_1})\oplus m_{\st 1}=\h((g^{\st r_2-r_1})^{\st y_1})\oplus m_{\st 1}$. Hence, $q\oplus e_{\st 1}=m_{\st 1}$.
 
 \end{itemize}

%
\end{itemize}

We conclude that DQ-OT always allows honest \re to recover the message of its interest, i.e., $m_s$.   

==> DQHT-OT.tex <==
%!TEX root = main.tex





%%%%%%%%%%%%%%
\begin{figure}[!h]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=81mm, left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\begin{enumerate}[leftmargin=5.2mm]
%
\item \underline{\textit{$\se$-side Initialization:}} 
%
$\mathtt{Init}(1^{\st \lambda})\rightarrow pk$
%
\begin{enumerate}

\item chooses a sufficiently large prime number $p$.

\item selects random element
$C \stackrel{\st \$}\leftarrow \mathbb{Z}_p$ and generator $g$.
\item publish $pk=(C, p, g)$. 

\end{enumerate}









\item \underline{\textit{$\re_j$-side Delegation:}}
%
$\mathtt{\re.Request}( 1^{\st \lambda}, s, pk)\rightarrow req=(req_{\st 1}, req_{\st 2})$
\begin{enumerate}

\item split  the private index $s$ into two shares $(s_{\st 1}, s_{\st 2})$ by calling  $\ses(1^{\st \lambda}, s, 2, 2)\rightarrow (s_{\st 1}, s_{\st 2})$.

\item pick two uniformly random values: $r_{\st 1}, r_{\st 2} \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.

\item send $req_{\st 1 }=(s_{\st 1}, r_{\st 1})$ to $\p_{\st1}$ and $req_{\st 2 }=(s_{\st 2}, r_{\st 2})$ to $\p_{\st 2}$.

\end{enumerate}


\item \underline{\textit{$\p_{\st 2}$-side Query Generation:}}
%
$\mathtt{\p_{\st 2}.GenQuery}(req_{\st 2}, ,pk)\rightarrow q_{\st 2}$

\begin{enumerate}

\item compute a pair of partial queries:
%
\vspace{-2mm}
%
  $$\delta_{\st s_2}= g^{\st r_2},\ \  \delta_{\st 1-s_2} = \frac{C}{g^{\st r_2}}$$
  
\item send $q_{\st 2}=(\delta_{\st 0}, \delta_{\st 1})$ to  $\p_{\st 1}$. 

\end{enumerate}

\item\underline{\textit{$\p_{\st 1}$-side Query Generation:}}
%
$\mathtt{\p_{\st 1}.GenQuery}(req_{\st 1}, q_{\st 2},pk)\rightarrow q_{\st 1}$

\begin{enumerate}

\item compute a pair of final queries as: 
%
%
\vspace{-2mm}
%
$$\beta_{\st s_1}=\delta_{0}\cdot g^{\st r_1},\ \ \beta_{\st 1-s_1}=\frac{\delta_{\st 1}} {g^{\st r_1}}$$

\item send $q_{\st 1}=(\beta_{\st 0}, \beta_{\st 1})$ to  $\se$.

\end{enumerate}

\item\underline{\textit{\se-side Response Generation:}} 
%
$\mathtt{GenRes}(m_{\st 0, 0}, m_{\st 1, 0},\ldots, m_{\st 0, z-1}, m_{\st 1, z-1},  pk, q_{\st 1})\rightarrow res$
%

\begin{enumerate}

\item abort if  $C \neq \beta_{\st 0}\cdot \beta_{\st 1}$.
    %
\item compute a response as follows. $\forall t, 0\leq t\leq z-1:$

\begin{enumerate}[leftmargin=3.5mm]

\item  pick two random values $y_{\st 0, t}, y_{\st 1, t}  \stackrel{\$}\leftarrow\mathbb{Z}_{\st p}$.
    %
\item compute response:
%
%
\vspace{-2mm}
%
   $$e_{\st 0, t} := (e_{\st 0, 0, t}, e_{\st 0, 1, t}) = (g^{\st y_{0, t}}, \h(\beta_{\st 0}^{\st y_{0, t}}) \oplus m_{\st 0, t})$$
    %
$$e_{\st 1, t} := (e_{\st 1, 0, t}, e_{\st 1, 1, t}) = (g^{\st y_{1, t}}, \h(\beta_{\st 1}^{\st y_{1, t}}) \oplus m_{\st 1, t}) $$


\end{enumerate}

 
\item send $res=(e_{\st 0, 0}, e_{\st 1, 0}),..., (e_{\st 0, z-1}, e_{\st 1, z-1})$ to $\p_{\st 1}$. 

\end{enumerate}


\item\underline{\textit{$\p_{\st 1}$-side Oblivious Filtering:}} 
%
$\mathtt{OblFilter}(res)\rightarrow  res'$

\begin{itemize}
\item[$\bullet$] forward $res'=(e_{\st 0, v}, e_{\st 1, v})$ to $\re_{\st j}$ and discard the rest of the messages received from \se. 
\end{itemize}

\item\underline{\textit{\re-side Message Extraction:}} 
%
%
$\mathtt{Retreive}(res', req,   pk)  \rightarrow m_{\st s}$
%



\begin{enumerate}

\item set $x=r_{\st 2}+r_{\st 1}\cdot(-1)^{\st s_2}$.

\item retrieve message $m_{\st s,v}$ by setting:  
%
 $$m_{\st s, v}=\h((e_{\st s, 0, v})^{\st x})\oplus e_{\st s, 1 v}$$

\end{enumerate}

\end{enumerate}
%%%%%%%%%%%%%%%
\end{tcolorbox}
\end{center}
\vspace{-2mm}
    \caption{\rdqothf: Our protocol that realizes \dqothf.}
    \label{fig::DQHT-OT}
    \vspace{-3mm}
\end{figure}

==> DUQ-MR-OT-Proof.tex <==
%%%%%YYYY
\subsection{\rduqothf's Security Proof}\label{sec::proof-of-DUQ-OT-HF}

%%%%%%%%%%%%%%%%**********

We prove the security of  \rduqothf, i.e., Theorem \ref{theo::DUQ-OTHF-2-sec}.

\begin{proof}
To prove the theorem, we consider the cases where each party is corrupt at a time.

\subsubsection{Corrupt \re} In the real execution, \re's view is: 

$\view_{\re}^{\st \rduqothf}\big(\bm{m}, (v, s, z)$ $  \empt, \empt, \empt\big) = \{r_{\st\re}, g, C, p, r_{\st 3}, s_{\st 2}, {o}_{\st 0}, {o}_{\st 1}, $ $m_{\st s, v} \}$, where 
$g$ is a random generator, $p$ is a large random prime number, 
%
${o}_{\st 0}:=({o}_{\st 0, 0}, {o}_{\st 0, 1})$, ${o}_{\st 1}:=({o}_{\st 1, 0}, {o}_{\st 1, 1})$, 
$C=g^{\st a}$ is a random value and public parameter, $a$ is a random value, and $r_{\st \re}$ is the outcome of the internal random coin of  \re that is used to (i) generate $(r_{\st 1}, r_{\st 2})$ and (ii) its public and private keys pair for additive homomorphic encryption. 



We will construct a simulator $\simm_{\re}$ that creates a view for \re such that (i) \re will see only a pair of messages rather than $z$ pairs, and (ii) the view is indistinguishable from the view of corrupt \re in the real model. 
%
$\simm_{\st \re}$ which receives $m_{\st s, v}$ from \re performs as follows. 
 
 
 
 \begin{enumerate}
 %
 \item initiates an empty view and appends uniformly random coin $r'_{\st\re}$ to it, where $r'_{\st\re}$ will be used to generate \re-side randomness. It selects a large random prime number $p$ and a random generator $g$.
 %
 
 
  \item sets response  as follows: 
  
  \begin{itemize}
 %%%%%%%%%%%%%%%%%%XXXXXX
 \item picks random values: $C', r'_{\st 1}, r'_{\st 2},y'_{\st 0}, y'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb{Z}_{p}$, $ r'_{\st 3}\stackrel{\st\$}\leftarrow\{0, 1\}^{\st\lambda}$, $s'\stackrel{\st\$}\leftarrow\{0,1\}$, and $u\stackrel{\st\$}\leftarrow\{0, 1\}^{\st\sigma+\lambda}$. %It also picks $s\in\{0,1\}$ with the same distribution used to pick $s$ in the real model. 
 
 \item sets $x=r'_{\st 2}+r'_{\st 1}\cdot (-1)^{\st s'}$ and $\beta'_{\st 0}=g^{\st x}$. 
 %
 \item sets $\bar{e}_{\st 0} := \big(\bar{e}_{\st 0,0}=g^{\st y'_0}, \bar{e}_{\st 0, 1}=\g(\beta'^{\st y'_0}_{\st 0})\oplus (m_{\st s,v}|| r'_{\st 3})\big)$ and $\bar{e}_{\st 1} := (\bar{e}_{\st 1,0}=g^{\st y'_{\st 1}}, \bar{e}_{\st 1,1}=u)$. 
 %
 
 \item encrypts the elements of the pair under $pk$ as follows. $\forall i,i', 0\leq i, i'\leq 1: \bar{o}_{\st i,i'}=\enc(pk, \bar{e}_{\st i,i'})$. Let $\bar{o}_{\st 0}:=(\bar{o}_{\st 0, 0}, \bar{o}_{\st 0, 1})$ and $\bar{o}_{\st 1}:=(\bar{o}_{\st 1, 0}, \bar{o}_{\st 1, 1})$. 
 
 
 
 \item randomly permutes the element of  pair $(\bar{o}_{\st 0}, \bar{o}_{\st 1})$. Let $(\bar{o}'_{\st 0}, \bar{o}'_{\st 1})$ be the result. 



 \end{itemize}
 %
 \item  appends $(g, C', p, r'_{\st 3}, s', \bar{o}'_{\st 0}, \bar{o}'_{\st 1}, m_{\st s, v})$ to the view and outputs the view.
 
 %%%%%%%%%%%%%%%XXXXXX
  %

 %
 \end{enumerate}


 Now, we argue that the views in the ideal and real models are indistinguishable. As we are in the semi-honest model, the adversary picks its randomness according to the protocol description; so, $r_{\st \re}$ and $r'_{\st \re}$ model have identical distributions, so do values $(r_{\st 3}, s_{\st 2})$ in the real model and $(r'_{\st 3}, s')$ in the ideal model, component-wise. Moreover,  values $g$ and $p$ in the real and ideal models, as they have been picked uniformly at random.  

%%XXXXXXX




For the sake of simplicity, in the ideal model let $\bar{e}'_{\st j}=\bar{e}_{\st 1} = (g^{y'_{\st 1}}, u)$ and in the real model let $e'_{\st i}=e_{\st 1-s}=(g^{\st y_{\st 1-s, v}}, \g(\beta^{\st y_{1-s, v}}_{\st 1-s})\oplus (m_{\st 1-s, v}||r_{\st 3}))$, where $i, j\in\{0,1 \}$.  Note that $\bar{e}'_{\st j}$ and $e'_{\st i}$ contain the elements that the adversary gets after decrypting the messages it receives from $\p_{\st 1}$ in the real model and from $\simm_{\st\re}$ in the ideal model.  





We will explain that  $e'_{\st i}$ in the real model and $\bar{e}'_{\st j}$ in the ideal model are indistinguishable. In the real model, it holds that $e_{\st 1-s}=(g^{\st y_{\st 1-s, v}}, \g(\beta^{\st y_{\st 1-s, v}}_{\st 1-s})\oplus (m_{1-s, v}||r_3))$, where $\beta^{\st y_{\st 1-s, v}}_{\st 1-s}=\frac{C}{g^{\st x}}=g^{\st a-x}$. Since $y_{\st 1-s, v}$ in the real model and $y'_{\st 1}$ in the ideal model have been picked uniformly at random and unknown to the adversary, $g^{\st y_{\st 1-s, v}}$ and $g^{\st y'_{1}}$  have identical distributions. Moreover, in the real model, given $C=g^{\st a}$, due to DL problem, $a$ cannot be computed by a PPT adversary.  Also, due to CDH assumption, \re cannot compute  $\beta^{\st y_{1-s, v}}_{\st 1-s}$, given $g^{\st y_{1-s}}$ and $g^{\st a-x}$. We know that $\g(.)$ is considered a random oracle and its output is indistinguishable from a random value. Therefore,  $\g(\beta^{\st y_{1-s, v}}_{\st 1-s})\oplus (m_{\st 1-s, v} || r_{\st 3})$ in the real model and $u$ in the ideal model are indistinguishable. This means that $e'_{\st i}$ and $\bar{e}'_{\st j}$ are indistinguishable too, due to DL, CDH, and RO assumptions. 
 
Also, ciphertexts $\bar{o}_{\st 1,0}=\enc(pk, g^{y'_{\st 1}})$ and $\bar{o}_{\st 1,1}=\enc(pk, u)$ in the ideal model and ciphertexts ${o}_{\st 1-s,0}=\enc(pk, g^{\st y_{1-s, v}})$ and ${o}_{\st 1-s,1}=\enc(pk, \g(\beta^{\st y_{1-s, v}}_{1-s})\oplus (m_{\st 1-s, v}||r_{\st 3}))$ in the real model have identical distributions due to IND-CPA property of the additive homomorphic encryption. 
 
 

 Further,  (i) $y_{\st s, v}$ in the real model and $y'_0$ in the ideal model have been picked uniformly at random and (ii) the decryption of both $e'_{\st 1-i}$ and $\bar{e}'_{\st 1-j}$ contain $m_{\st s, v}$; therefore, $e'_{\st 1-i}$ and $\bar{e}'_{\st 1-j}$ have identical distributions. Also, $m_{\st s, v}$ has identical distribution in both models.  Both $C$ and $C'$ have also been picked uniformly at random from $\mathbb{Z}_{\st p-1}$; therefore, they have identical distributions. 
 
 
 In the ideal model, $\bar{e}_{\st 0}$ always contains encryption of actual message $m_{\st s, v}$ while $\bar{e}_{\st 1}$ always contains a dummy value $u$. However, in the ideal model the encryption of the elements of pair  $(\bar{e}_{\st 0}, \bar{e}_{\st 1})$ and in the real model the encryption of the elements of pair $(e_{\st 0,v}, e_{\st 1,v})$ have been randomly permuted, which results in $(\bar{o}'_{\st 0}, \bar{o}'_{\st 1})$ and $(o_{\st 0}, o_{\st 1})$ respectively. 
 
 
Moreover, ciphertexts $\bar{o}_{\st 0,0}=\enc(pk, g^{\st y'_{\st 0}})$ and $\bar{o}_{\st 0,1}=\enc(pk, $ $\g(\beta'^{\st y'_0}_{\st 0})\oplus (m_{\st s,v}|| r'_{\st 3})))$ in the ideal model and ciphertexts ${o}_{\st s,0}=\enc(pk, g^{\st y_{\st s, v}})$ and ${o}_{\st s,1}=\enc(pk, \g(\beta^{y_{\st s, v}}_{\st s})\oplus (m_{\st s, v}||r_{\st 3}))$ have identical distributions due to IND-CPA property of the additive homomorphic encryption. Thus, the permuted pairs have identical distributions too. 


We conclude that the two views are computationally indistinguishable, i.e., Relation \ref{equ::DUQ-OT-HF-reciever-sim-} (in Section \ref{sec::Delegated-Unknown-Query-OT-HF}) holds. That means, even though \se holds $z$ pairs of messages and generates a response for all of them, \re's view is still identical to the case where \se holds only two pairs of messages. 



 \subsubsection{Corrupt \se}   This case is identical to the corrupt \se in the proof of DUQ-OT (in Appendix \ref{sec::DUQ-OT-Security-Proof}) with a minor difference. Specifically, the real-model view of \se in this case is identical to the real-model view of \se in DUQ-OT. Nevertheless, now $\simm_{\st\se}$ receives a vector $\bm{m}=[(m_{\st 0, 0},m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})]$ from \se, instead of only a single pair that $\simm_{\st\se}$ receives in the proof of DUQ-OT. $\simm_{\st\se}$ still carries out the same way it does in the corrupt \se case in the proof of DUQ-OT. Therefore, the same argument that we used (in Appendix \ref{sec::DUQ-OT-Security-Proof}) to argue why real model and ideal model views are indistinguishable (when \se is corrupt), can be used in this case as well.
 
 Therefore, Relation \ref{equ::DUQ-OT-HF-sender-sim-}  (in Section \ref{sec::Delegated-Unknown-Query-OT-HF}) holds.

\subsubsection{Corrupt $\p_{\st 2}$} This case is identical to the corrupt   $\p_{\st 2}$ case in the proof of DUQ-OT. Thus, Relation \ref{equ::DUQ-OT-HF-server-sim-}  (in Section \ref{sec::Delegated-Unknown-Query-OT-HF}) holds.

\subsubsection{Corrupt $\p_1$} In the real execution, $\p_{1}$'s view is: 
 
$\view_{\p_1}^{\st \rduqothf}\big(\bm{m}, (v, s, z), $ $ \empt, \empt, \empt \big)=\{g, C, p, s_1, \bm{w}_{\st j}, r_{\st 1}, \delta_{\st 0}, \delta_{\st 1},$\\ $ (e'_{\st 0,0}, e'_{\st 1,0}),$ $ ...,$ $ (e'_{\st 0, z-1},$ $ e'_{\st 1, z-1})\}$. Ideal-model $\simm_{\st\p_{\st 1}}$ operates as follows.  


\begin{enumerate}
%
\item initiates an empty view. It selects a large random prime number $p$ and a random generator $g$.
%
\item picks two random values $\delta'_{\st 0}, \delta'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb{Z}_{p}$. 
%

\item constructs an empty vector $\bm{w}'$. It picks $z$ uniformly at random elements $w'_{\st 0},..., w'_{\st z}$  from the encryption (ciphertext) range and inserts the elements into $\bm{w}'$. 

\item picks two uniformly random values $s'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb U$ and $C', r'_{\st 1}\stackrel{\st\$}\leftarrow\mathbb{Z}_{p}$, where $\mathbb{U}$ is the output range of $\ses(.)$. 

\item picks $z$ pairs of random values as follows  $(a_{\st 0,0}, a_{\st 1,0}),..., (a_{\st 0,z-1},$ $ a_{\st 1,z-1})\stackrel{\$}\leftarrow\mathbb{Z}_{\st p}$. 
%
\item appends  $s'_{\st 1},g, C', p, r'_{\st 1}, \delta'_{\st 0}, \delta'_{\st 1}$ and pairs $(a_{\st 0,0}, a_{\st 1,0}),..., (a_{\st 0,z-1},$ $ a_{\st 1,z-1})$ to the view and outputs the view. 
 %
\end{enumerate}

Next, we argue that the views in the ideal and real models are indistinguishable. The main difference between this case and the corrupt $\p_{\st 1}$ case in the proof of DUQ-OT (in Appendix  \ref{sec::DUQ-OT-Security-Proof}) is that now, in the real model, $\p_1$ has: (i) a vector $\bm{w}_{\st j}$ of ciphertexts and (ii) $z$ pairs $(e'_{\st 0,0}, e'_{\st 1,0}),..., (e'_{\st 0,z-1},$ $ e'_{\st 1,z-1})$.  Therefore, we can reuse the same argument we provided for the corrupt $\p_1$ case in the proof of DUQ-OT to argue that the views (excluding $\bm{w}_{\st j}$ and $(e'_{\st 0,0}, e'_{\st 1,0}),..., (e'_{\st 0,z-1},$ $ e'_{\st 1,z-1})$) have identical distributions. 


Due to Lemma \ref{lemma::two-pairs-indis-}, the elements of each pair  $(e'_{\st 0, i}, e'_{1, i})$ in the real model are indistinguishable from the elements of each pair  $(a_{\st 0, i}, a_{\st 1, i})$ in the ideal model, for all $i$, $0 \leq i \leq z-1$.  Also, due to the IND-CPA property of the additive homomorphic encryption scheme, the elements of $\bm{w}_{\st j}$ in the real model are indistinguishable from the elements of $\bm{w}'$ in the ideal model. 




Hence, Relation \ref{equ::DUQ-OT-HF-server-sim-} (in Section \ref{sec::Delegated-Unknown-Query-OT-HF}) holds.



\subsubsection{Corrupt $\tp$} This case is identical to the corrupt \tp in the proof of DUQ-OT, with a minor difference; namely, in this case, \tp also has input $z$ which is the total number of message pairs that \se holds. Thus, we can reuse the same argument provided for the corrupt \tp in the proof of DUQ-OT to show that the real and ideal models are indistinguishable. Thus, Relation \ref{equ::DUQ-OT-HF-t-sim-} (in Section \ref{sec::Delegated-Unknown-Query-OT-HF}) holds.
%
\end{proof}





%\clearpage


==> DUQ-MR-OT-Protocol-Part-2.tex <==
%%%%%%%%%%%%%%%%%%
%
\begin{figure}[!htbp]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=86mm,  left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\vspace{-1.5mm}


\begin{enumerate}[leftmargin=5.8mm,start=9]

%XXXXXXXXXXXXXXX
\item\label{DUQOT-HT::oblivius-filter}\underline{\textit{$\p_{\st 1}$-side Oblivious Filtering:}} 
%
$\mathtt{OblFilter}(res, pk_{\st j}, \bm{w}_{\st j})\hspace{-.7mm}\rightarrow\hspace{-.6mm} res'$

\begin{enumerate}

\item compresses \se's response using vector  $\bm{w}_{\st j}$ as follows. $\forall i,i', 0\leq i,i'\leq 1:$
    
$o_{\st i, i'}= (e'_{\st i, i',0}\hmul \bm{w}_{\st j}[0])\hadd...\hadd  (e'_{\st i,i', z-1}\hmul \bm{w}_{\st j}[z-1])$.
 
\item  send $res'=(o_{\st 0, 0}, o_{\st 0, 1}), (o_{\st 1, 0}, o_{\st 1, 1}) \text{ to } \re_{\st j}$.

\end{enumerate}



\item\label{DUQOT-HT::message-ext} \underline{\textit{\re-side Message Extraction:}}  
%
%
$\mathtt{Retreive}(res', req,  sk_{\st j}, pk,$ $ sp_{\st \re})\hspace{-.6mm}\rightarrow\hspace{-.8mm} m_{\st s}$
%

\begin{enumerate}


\item decrypt the response from $\p_{\st 1}$ as follows: 

 $\forall i,i', 0\leq i,i'\leq 1:$
%
$ \dec(sk_{\st j}, o_{\st i,i'})\rightarrow o'_{\st i,i'}$. 



\item set $x=r_{\st 2}+r_{\st 1}\cdot(-1)^{\st s_2}$.

\item retrieve message $m_{\st s, v}$ as follows. 
%
 $\forall i, 0\leq i\leq1:$

\begin{enumerate}

\item set $y=\g(({o}'_{\st i, 0})^{\st x})\oplus {o}'_{\st i, 1}$.

\item call $\parse(\gamma, y)\rightarrow (\ux, \uy)$.

\item  set $m_{\st s, v}=\ux$, if $\uy=r_{\st 3}$.

\end{enumerate}

\end{enumerate}



%*********

\end{enumerate}
\vspace{-1mm}
\end{tcolorbox}
\end{center}
\vspace{-1mm}
    \caption{Phases \ref{DUQOT-HT::oblivius-filter} and \ref{DUQOT-HT::message-ext} of \rduqothf.    
    }
    \label{fig::DQ-OT-with-unknown-query-and-HF-last-three-phases}
    \vspace{-1mm}
\end{figure}




==> DUQ-MR-OT-Protocol.tex <==
%%%%%%%%%%%%%%%%%%
%
\begin{figure}[!htbp]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=86mm,height=226mm,  left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\vspace{-2mm}

\begin{enumerate}[leftmargin=4.5mm]

\item\label{phase::s-init} \underline{\textit{$\se$-side Initialization:}} 
%
$\mathtt{Init}(1^{\st \lambda})\rightarrow pk$
%


It chooses a large random prime number $p$, random element
$C \stackrel{\st \$}\leftarrow \mathbb{Z}_p$, and generator $g$. It publishes $pk=(C, p, g)$. 






%
\item\label{DUQOT-HT::gen-key} \underline{\textit{$\re_{\st j}$-side One-off Setup:}}
%
$\mathtt{\re.Setup}(1^{\st \lambda})\rightarrow (pk_{\st j}, sk_{\st j})$
%

%\begin{enumerate}

It generates a key pair for the  homomorphic encryption, by calling $\keygen(1^{\st\lambda})\rightarrow(sk_{\st j}, pk_{\st j})$. It send $pk_{\st j}$  to \tp and $\se$.





\item  \underline{\textit{\tp-side One-off Setup:}}
%
$\mathtt{\tp.Setup}(z, pk_{\st j})\rightarrow \bm{w}_{\st j}$


\begin{enumerate}

\item initialize an empty vector $\bm{w}_{\st j}=[]$ of size $z$.

\item create a compressing vector, by setting $v$-th position of $\bm{w}_{\st j}$ to encrypted $1$ and setting the rest of $z-1$ positions to encrypted $0$. $ \forall t, 0\leq t\leq z-1:$
%

\begin{enumerate}

\item  set  $d=1$, if $t=v$; set $d=0$, otherwise.

\item  append $\enc(pk_{\st j}, d)$ to  $\bm{w}_{\st j}$.

\end{enumerate}

\item send $\bm{w}_{\st j}$ to $\p_{\st 1}$.

\end{enumerate}

\item \underline{\textit{$\re_{\st j}$-side Delegation:}}
%
$\mathtt{\re.Request}( pk)\hspace{-.6mm}\rightarrow\hspace{-.6mm} req=(req_{\st 1}, req_{\st 2})$

\begin{enumerate} 

\item pick random values: $r_{\st 1}, r_{\st 2} \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.

\item send $req_{\st 1} = r_{\st 1}$ to $\p_{\st 1}$ and $req_{\st 2}= r_{\st 2}$ to $\p_{\st 2}$.

\end{enumerate}

\item \underline{\textit{$\tp$-side Query Generation:}}
%
$\mathtt{\tp.Request}(1^{\st \lambda}, s,$ $ pk)\hspace{-1mm}\rightarrow\hspace{-1mm} (req'_{\st 1}, $ $req'_{\st 2},$ $ sp_{\st \se})$

\begin{enumerate}

\item split  the private index $s$ into two shares $(s_{\st 1}, s_{\st 2})$ by calling  $\ses(1^{\st \lambda}, s, 2, 2)\rightarrow (s_{\st 1}, s_{\st 2})$.

\item pick a uniformly random value: $r_{\st 3} \stackrel{\st\$}\leftarrow\{0,1\}^{\st\lambda}$.

% \item send $(s_{\st 2}, r_{\st 3})$ to $\re_{\st j}$, $s_{\st 1}$ to  $\p_{\st 1}$, $s_{\st 2}$ to  $\p_{\st 2}$,  $r_{\st 3}$ to \se. 

\item send $req'_{\st 1} =s_{\st 1}$ to  $\p_{\st 1}$, $req'_{\st 2}=s_{\st 2}$ to  $\p_{\st 2}$. It sends secret parameter $sp_{\st \se}=r_{\st 3}$ to \se and $sp_{\st \re} = (req'_{\st 2}, sp_{\st \se})$ to \re.

\end{enumerate}
\item \underline{\textit{$\p_{\st 2}$-side Query Generation:}}
%
$\mathtt{\p_{\st 2}.GenQuery}(req_{\st 2}, req'_{\st 2}, pk)\rightarrow q_{\st 2}$
%

\begin{enumerate}

\item compute queries:
%
  $\delta_{\st s_2}= g^{\st r_2},\ \  \delta_{\st 1-s_2} = \frac{C}{g^{\st r_{\st 2}}}$.
  %
\item send $q_{\st 2}=(\delta_{\st 0}, \delta_{\st 1})$ to  $\p_{\st 1}$. 

\end{enumerate}

\item\label{DUQOT-HT::gen-P1-side-q-gen}\underline{\textit{$\p_{\st 1}$-side Query Generation:}}
%
$\mathtt{\p_{\st 1}.GenQuery}(req_{\st 1},req'_{\st 1}, q_{\st 2},pk)\hspace{-1.1mm}\rightarrow\hspace{-1.1mm} q_{\st 1}$
%

\begin{enumerate}

\item compute  queries as: 
%
%\vspace{-2.5mm}
%
$\beta_{\st s_{\st 1}}=\delta_{\st 0}\cdot g^{\st r_1}, \beta_{\st 1-s_1}=\frac{\delta_{\st 1}} {g^{\st r_1}}$ 
%\vspace{-4.5mm}

\item send $q_{\st 1}=(\beta_{\st 0}, \beta_{\st 1})$ to  $\se$.
\end{enumerate}


%********

\item\label{DUQOT-HT::gen-res}\underline{\textit{\se-side Response Generation:}} 
%
$\mathtt{GenRes}(m_{\st 0,0}, m_{\st 1, 0},\ldots, m_{\st 0,z-1},$ $ m_{\st 1, z-1}, pk, q_{\st 1}, sp_{\st \se})\rightarrow res$
%

\begin{enumerate}

\item abort if  $C \neq \beta_{\st 0}\cdot \beta_{\st 1}$.

\item compute a response as follows. $\forall t, 0\leq t \leq z-1:$
%
\begin{enumerate}[leftmargin=1.2mm]
\item   pick two random values $y_{\st 0, t}, y_{\st 1, t}  \stackrel{\$}\leftarrow\mathbb{Z}_{\st p}$.  
  
\item  compute  response:

 $ e_{\st 0, t} := (e_{\st 0, 0, t}, e_{\st 0, 1, t}) = (g^{\st y_{\st 0, t}}, \g(\beta_{\st 0}^{\st y_{0, t}}) \oplus (m_{\st 0, t}||r_{\st 3}))$
      
$e_{\st 1, t} := (e_{\st 1, 0, t}, e_{\st 1, 1, t}) = (g^{\st y_{1, t}}, \g(\beta_{\st 1}^{\st y_{\st 1, t}}) \oplus (m_{\st 1, t}||r_{\st 3})) $ 
   
\item   randomly permute the elements of each pair $(e_{\st 0, t}, e_{\st 1, t})$ as $\pi(e_{\st 0, t}, e_{\st 1, t})\rightarrow ({e}'_{\st 0, t}, {e}'_{\st 1, t})$.
   
\end{enumerate}

\item     send $res=(e'_{\st 0, 0}, e'_{\st 1, 0}),\ldots, (e'_{\st 0, z-1}, e'_{\st 1, z-1}) \text{ to } \p_{\st 1}$.
\end{enumerate}


% %XXXXXXXXXXXXXXX
% \item\label{DUQOT-HT::oblivius-filter}\underline{\textit{$\p_{\st 1}$-side Oblivious Filtering:}} 
% %
% $\mathtt{OblFilter}(res, pk_{\st j}, \bm{w}_{\st j})\hspace{-.7mm}\rightarrow\hspace{-.6mm} res'$

% \begin{enumerate}

% \item compresses \se's response using vector  $\bm{w}_{\st j}$ as follows. $\forall i,i', 0\leq i,i'\leq 1:$
    
% $o_{\st i, i'}= (e'_{\st i, i',0}\hmul \bm{w}_{\st j}[0])\hadd...\hadd  (e'_{\st i,i', z-1}\hmul \bm{w}_{\st j}[z-1])$.
 
% \item  send $res'=(o_{\st 0, 0}, o_{\st 0, 1}), (o_{\st 1, 0}, o_{\st 1, 1}) \text{ to } \re_{\st j}$.

% \end{enumerate}



% \item\label{DUQOT-HT::message-ext}\hspace{-2mm} \underline{\textit{\re-side Message Extraction:}} 
% \hspace{-2mm} 
% %
% %
% $\mathtt{Retreive}(res', req,  sk_{\st j}, pk,$ $ sp_{\st \re})\hspace{-.6mm}\rightarrow\hspace{-.8mm} m_{\st s}$
% %

% \begin{enumerate}


% \item decrypt the response from $\p_{\st 1}$ as follows: 

%  $\forall i,i', 0\leq i,i'\leq 1:$
% %
% $ \dec(sk_{\st j}, o_{\st i,i'})\rightarrow o'_{\st i,i'}$. 



% \item set $x=r_{\st 2}+r_{\st 1}\cdot(-1)^{\st s_2}$.

% \item retrieve message $m_{\st s, v}$ as follows. 
% %
%  $\forall i, 0\leq i\leq1:$

% \begin{enumerate}

% \item set $y=\g(({o}'_{\st i, 0})^{\st x})\oplus {o}'_{\st i, 1}$.

% \item call $\parse(\gamma, y)\rightarrow (\ux, \uy)$.

% \item  set $m_{\st s, v}=\ux$, if $\uy=r_{\st 3}$.

% \end{enumerate}

% \end{enumerate}



%*********

\end{enumerate}
\vspace{-1mm}
\end{tcolorbox}
\end{center}
\vspace{-2mm}
    \caption{Phases \ref{phase::s-init}--\ref{DUQOT-HT::gen-res} of \rduqothf. 
    }
    \label{fig::DQ-OT-with-unknown-query-and-HF-first-eight-phases}
    \vspace{-2mm}
\end{figure}




==> Noar-OT.tex <==

\subsection{The Original OT of Naor and Pinkas}\label{sec::OT-of-Naor-Pinkas}

Figure \ref{fig::Noar-OT} restates the original OT of Naor and Pinkas \cite[pp. 450, 451]{Efficient-OT-Naor}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!h]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=85mm, left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\vspace{-2mm}
\begin{enumerate}[leftmargin=5.2mm]


\item \underline{\textit{$\se$-side Initialization:}} 
%
$\mathtt{\se.Init}(1^{\st\lambda})\rightarrow pk$

\begin{enumerate}

\item  choose a random large prime number $p$ (where $\log_{\st 2}p=\lambda$), a random element
$C \stackrel{\st \$}\leftarrow \mathbb{Z}_{\st p}$ and random generator $g$.
\item publish $pk=(C, g, p)$. 

\end{enumerate}

\item \underline{\textit{$\re$-side Query Generation:}} 
%
$\mathtt{\re.GenQuery}(pk, s)\rightarrow (q, sp)$

\begin{enumerate}

\item pick a random value $r \stackrel{\st \$}\leftarrow \mathbb{Z}_p\setminus\{0\}$ and sets $sp=r$. 
%
\item set $\beta_{\st s}=g^{\st r}$ and $\beta_{\st 1-s}=\frac{C}{\beta_{\st s}}$.


\item send $q=\beta_{\st 0}$ to \se and locally stores $sp$. 


\end{enumerate}

\item \underline{\textit{$\se$-side Response Generation:}} 
%
$\mathtt{\se.GenRes}(m_{\st 0}, m_{\st 1}, pk, q)\rightarrow res$

\begin{enumerate}

\item compute $\beta_{\st 1}=\frac{C}{\beta_{\st 0}}$.

\item choose two random values, $y_{\st 0}, y_{\st 1}\stackrel{\st \$}\leftarrow \mathbb{Z}_p$. 

\item encrypt the elements of the pair $(m_{\st 0}, m_{\st 1})$ as follows: 
%
$$e_{\st 0}:=(e_{\st 0,0}, e_{\st 0,1})=(g^{\st y_0}, \h(\beta_{\st 0}^{\st y_0}) \oplus m_{\st 0})$$
%
$$e_{\st 1}:=(e_{\st 1,0}, e_{\st 1,1})=(g^{\st y_1}, \h(\beta_{\st 1}^{\st y_1}) \oplus m_{\st 1})$$

\item send $res=(e_{\st 0}, e_{\st 1})$ to \re.
\end{enumerate}

\item\underline{\textit{\re-side Message Extraction:}} 
%
$\mathtt{\re.Retreive}(res, sp, pk, s)\rightarrow m_{\st s}$

\begin{itemize}
\item retrieve the related message $m_{\st s}$ by computing 
%
$$m_{\st s}=\h((e_{\st s,0})^{\st r})\oplus e_{\st s, 1}$$

\end{itemize}

\end{enumerate}
%%%%%%%%%%%%%%%
\end{tcolorbox}
\end{center}
%\vspace{-4mm}
\caption{Original OT proposed by  Naor and Pinkas \cite[pp. 450, 451]{Efficient-OT-Naor}. In this protocol, the input of \re is a private binary index $s$ and the input of \se is a pair of private messages $(m_{\st 0}, m_{\st 1})$.} 
%\vspace{-4mm}
\label{fig::Noar-OT}
\end{figure}




==> biography.tex <==
% !TEX root =main.tex

\begin{IEEEbiography}[{\includegraphics[width=1.09in,height=1.25in,clip,keepaspectratio]{aydin}}]{Aydin Abadi}
holds BSc and MSc degrees from the University of Lahijan, Iran, and the University of Leeds, UK, respectively. He obtained his PhD degree from the Department of Computer Science at the University of Strathclyde. Currently, he serves as an Assistant Professor at Newcastle University. His primary research interests include information security, privacy, and cryptography, with a particular focus on cryptanalysis, time-lock puzzles, private set intersection, online financial fraud, and blockchain.  
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.09in,height=1.2in,clip]{Files/TDSC-24/yvo-2-modified.jpeg}
}]{Yvo Desmedt}
is the Jonsson Distinguished Professor at the University of Texas at Dallas. He was Chair of Information Communication Technology at University College London. He was a pioneer of threshold cryptography and is an International Association for Cryptologic Research Fellow.  His main research interests include access control, Internet voting, bridging theory and practice, combinatorics, cryptanalysis, distributed and network security, and public key cryptography. 



\end{IEEEbiography}

==> blank.tex <==
%!TEX root = main.tex



\section{Introduction}





==> old-content.tex <==



\vspace{-2mm}
\section{Introduction}\label{sec:intro}


%\vspace{-0.4mm}


Databases play a vital role in e-commerce, advertising, intelligence analysis, combating crime, knowledge discovery, and conducting scientific research. Privacy breaches involving databases, impacting both organizations and individuals, have become headline news. 
%
%Privacy violations of databases affecting organizations and individuals have made the news. 
%
%Databases can be highly valuable to their owners and the owners' rivals.  
Some databases (e.g., Fortune 500 companies' databases about customers purchase history)  can be valued at millions of dollars.   


% Often the user of a database is not the one who created it. 

Privacy issues arise when users seek access to databases they do not own or create. Furthermore, many databases are now hosted in the cloud,  adding another layer of complexity to the privacy landscape.
%
To simultaneously protect the privacy of the user and the database itself from each other, the cryptographic-based technology, called Oblivious Transfer (OT) has been proposed. It allows a user (called a receiver) interested in the $s$-th element of a database  $(m_{\st 0}, m_{\st 1})$  (held by a sender) to learn only $m_{\st s}$ while preserving the privacy of (i) index $s\in\{0, 1\}$ from the sender and (ii) the rest of the database's elements from the receiver. Numerous variants have been developed since OT's introduction in 1981 \cite{Rabin-OT}. 

Nevertheless, as evidenced by this work, numerous research gaps persist in this domain. Many real-world applications have been overlooked, and it is revealed that these oversights align with gaps in the research on OT, as expounded upon in the next section.

\vspace{-2mm}
\section{Motivations and Survey}
In this section, we motivate the paper using real-world scenarios, discuss gaps in the OT research line, and outline our contributions. 

\vspace{-1mm}
\subsection{Motivations}

\subsubsection{Dealing with Insiders, e.g., in Financial Institutions}\label{sec::} 
Insider attacks pose genuine and imminent threats to various organizations and their clients, such as financial institutions and their customers.  Insiders may collaborate with external fraudsters, obtaining highly valuable data. The ``Swiss Leaks'' \cite{leigh2015hsbc} is a good example to illustrate the problem of insider leaks in the banking world.  In the Swiss Leaks case, an insider attempted to sell information about accounts held by HSBC in Geneva. Later, when he failed, he leaked the information to the public.  As another example, in the case of ``JPMorgan Chase Insider Thief'' \cite{JPMorgan}, a former JPMorgan Chase personal banker has been arrested by the FBI on charges that he stole customers' account information and sold it to an undercover informant. 


In this context, an insider can exclusively target high-profile wealthy individuals and sell the victims' information to their rivals, who might make strategic investments, often remaining stealthy from the victims' perspective. For an insider, a data breach in private banking or private financial advising can be more alluring than leaking hundreds of bank accounts. Indeed, the former could yield a higher payoff while concurrently posing a lower risk of exposure.

In this setting, financial advisors, within a financial institution, frequently maintain paid subscriptions to a valuable database (e.g., containing real estate market information, market trends, and capital flows) offered by third-party providers such as CoreLogic\footnote{\url{https://www.corelogic.com/data-solutions/property-data-solutions/discovery-platform}},  Multiple Listing Service\footnote{\url{https://www.mls.com}}, or Real Capital Analytics\footnote{\url{https://www.msci.com/our-solutions/real-assets/real-capital-analytics}}.  In contrast, clients of these advisors do not necessarily need to subscribe to the database themselves. Instead, they interact with the advisors and direct their queries to them. 
%
Outsiders who infiltrate the computers of an individual advisor or the third-party database can compromise the privacy of customers' queries as well.

Hence, there is a pressing need to (i) protect customer query privacy from advisors and databases, (ii) ensure the privacy of the database from both customers and advisors, and (iii) secure the privacy of customers in the event of a data breach on the advisor's or database's side. As explained in Section \ref{sec::gap-delegated-Q-OT}, current OTs fall short of providing these features simultaneously.


\vspace{-1.4mm}
\subsubsection{Multi-Receiver OT}\label{sec:Delegated-Query-OT-w-HF}



The adoption of cloud computing has been accelerating. The ``PwC’s 2023 Cloud Business Survey'' suggests that 78\% of executives participating in the survey have mentioned that their companies had adopted cloud in most or all parts of the business \cite{PwC2023}. Moreover, multiple (sensitive) databases belonging to different parties have been merged and hosted by a single cloud provider.  Indeed, the recent cyber attack revealed that data belonging to British Airways, Boots, BBC, and Aer Lingus was kept by the same cloud \cite{BBB-hack}. 
%
The current OTs do not allow us to deal with this scenario, as we will elaborate in Section \ref{sec::gap-Querying-Merged-Databases}. %We present a fully private multi-receiver OT is necessary to ensure user privacy in real-world cloud settings. 





\vspace{-1.2mm}
\subsubsection{Querying Databases with Hidden Fields}\label{sec::delegated-Unknown-Query-OT-motivation}

%In the context of financial institutions,

In specific applications, such as finance or healthcare, sensitive details about customers or patients must be withheld from them. In the financial sector, this may include  
(a) a binary flag that determines whether a certain customer is deemed suspicious \cite{arora2023privacy,DrivenData}, or (b) proprietary banking strategies tailored to individual clients. In the medical sector, such information may involve a binary flag indicating whether a patient has a certain condition. In certain cases, revealing specific details about an illness or test result might endanger the patient \cite{exchange-of-health-info,Withholding-Information}. 
%
Hence, in some scenarios, the result that a client/receiver obtains for its request (e.g., seeking investment advice) depends on the private flag/query $s$,  provided by a third party to its advisor who is directly dealing with the client, while the client itself is not aware of the value of $s$. We will further discuss it in Section \ref{sec::Hidden-Fields}.










% %%%%%%%%%move below

% To enable their staff members to access the organisation's remote database in a privacy-preserving manner, each organisation might be tempted to use one of the following approaches.

% \begin{itemize}%[leftmargin=4mm]

% \item  \underline{\textit{Using an existing single-receiver OT, e.g., in \cite{IshaiKNP03}}}. However, this approach suffers from information leakage. It allows the server to learn not only which organisation is accessing the data but potentially even which specific staff member is utilising a particular portion of the data. 

% \item \underline{\textit{Using an existing multi-receiver OT, e.g., in \cite{CamenischDN09}}}. Nevertheless, this will also come with a privacy cost. The existing multi-receiver OTs reveal the size of the entire database to each receiver. In this scenario, a receiver can learn the number of private records other companies have in the same database. This type of leakage is particularly significant, especially when coupled with specific auxiliary information. %For instance, the recent cyber attack revealed that data belonging to British Airways, Boots, BBC, and Aer Lingus was kept by the same cloud  \cite{BBB-hack}. 

% \end{itemize}

% Hence, a fully private multi-receiver OT is necessary to ensure user privacy in real-world cloud settings. 



\vspace{-2.4mm}
\subsection{Research Gaps}

\subsubsection{Support for Delegated-Query OT}\label{sec::gap-delegated-Q-OT} 
%
Current technologies assume that a receiver which generates the query \textit{always} has \emph{direct subscription/access to databases} and enough computation resources to generate queries that are sent to the sender. This assumption has to be relaxed when receivers are not subscribed to the database (e.g., they cannot afford it) or when receivers are thin clients, e.g., IoT devices with limited computational resources or battery lifespan. We introduce \textit{Delegated-Query Oblivious Transfer} to address these limitations and deal with the insider attacks (see Section \ref{sec:protocol}). 

%se section x for solution-- repeat it for any gap


\vspace{-1.2mm}
\subsubsection{Querying Merged Databases.} \label{sec::gap-Querying-Merged-Databases}
%
Existing techniques do not support querying \emph{merged databases} in a full privacy-preserving manner. Specifically, they  
 are not suitable for the \emph{real-world multi-receiver setting} where a sender maintains multiple records\footnote{A database table consists of records/rows and fields/columns. Each record in a table represents a set of related data, e.g., last name and address.} each belonging to a different receiver.   The existing techniques do not allow a receiver to privately query such records without disclosing (i) the records the receiver accesses to the sender and (ii) the number of records other users of the database have to each receiver. Receivers with different levels of security form a natural example. The existing OTs reveal the entire database's size to receivers enabling them to acquire non-trivial information. The mere existence of private data itself can be considered sensitive information \cite{securityy}. We propose several \textit{Multi-Receiver OTs} to support querying merged databases in a privacy-preserving fashion (see Section \ref{sec::Multi-Receiver-OT}).



%Secondly, existing techniques are not suitable for the \emph{real-world multi-receiver setting} where a sender (e.g., multi-tenant cloud) maintains multiple records\footnote{A database table consists of records/rows and fields/columns. Each record in a table represents a set of related data, e.g., last name and address.} each belonging to independent receivers, where the records/receivers are defined by a hidden (sensitive) field.  The existing techniques do not allow a receiver to privately query such records without disclosing (i) the records the receiver accesses to the sender and (ii) the number of records other users of the database have. Receivers with different levels of security form a natural example. The existing OTs reveal the entire database's size to receivers enabling them to acquire non-trivial information. The mere existence of private data itself can be considered sensitive information  \cite{pfleeger1988security}. 
%



% To tackle the size-leakage issue, one might consider two tempting approaches: (a) assigning a physically separated database to each receiver, resulting in more physical databases and increased maintenance costs compared to the single-database scenario, while also enabling the sender to learn which receiver can access specific records; or (b) allowing the receiver to disclose the record's index/ID of interest to the sender, which in itself presents a leakage.









%The database can use an extra field\footnote{Field is a column in a database, e.g., first name or street name.} in the database to
%indicate the owner. In other words, using this hidden field, the database
%allows the organization to only access their own data.
%Minimal privacy means that users of organisation $A$ should
%not know about data of organization $B$. If $A$ is, e.g., an
%intelligence agency, the database should not know who is accessing the
%data. Moreover, in the last case the database should not know what record was
%accessed. Note that using OT in a trivial way will leak the size of the
%database, which will allow $B$ to guess there is extra information.\textcolor{blue}{do we need the next two paragraphs?}


%For instance, consider the case where a database of an aircraft manufacturer (e.g., Boeing or Airbus) holds two sets of records one set for specifications of a commercial airplane and the other one for specifications of a top-secret military airplane. In this case, if a receiver (e.g., aerospace engineer) that does not have a top-secret clearance interacts with the database by using one of the existing OT protocols to access a record for the commercial airplane will immediately learn that there is another set(s) of records for a top-secret military airplane. To address the issue, one may be tempted to (i) allocate a separate database to each receiver (or a set of receivers), which would (i) increase the size of the entire database linearly with the number of receivers or types of security clearance and (ii) allow the sender to learn the type of security clearance that each receiver has.

%use physical separation. 

%For instance,  in the case where a (cloud) database holds records of multiple companies if an employee of one of the companies uses an existing technique to interact with the database, it will learn the entire size of the database. In this case, the receiver can learn the number of records other companies had in the same database, given some public auxiliary information. An example of this auxiliary information is that British Airways, Boots, and BBC data were kept by the same cloud, according to the very recent cyber-attack \cite{BBB-hack}. To address the size-leakage issue, one may be tempted to (a) allocate a physically separated database to each receiver (or a set of receivers), which would (i) increase the size of the entire database linearly with the number of receivers or types of security clearance and (ii) allow the sender to learn the type of security clearance that each receiver has(i.e., which receiver can access to which records), or (b) allow the receiver to declare to the sender the record's index/ID it wants to access which would also enable the sender to learn the security clearance of the receiver.   

\vspace{-1.2mm}
\subsubsection{Databases with Hidden Fields.} \label{sec::Hidden-Fields}
%
The current OT concept assumes the receiver knows the full query, which may not always be desired, as discussed in Section  \ref{sec::delegated-Unknown-Query-OT-motivation}. We will propose OT variants supporting a (partially) \textit{unknown query} (see Sections \ref{sec::DUQ-OT-protocol} and \ref{sec::DUQ-OT-HF}). 


\vspace{-1.2mm}
\subsubsection{Constant Size Response}
The current techniques that allow a receiver to obtain  response with a \emph{constant size} for its query necessitate the receiver to possess a storage space proportional to the size of the database, to locally store the database encryption. However, meeting this demanding requirement will become challenging for a thin client (e.g., in IoT settings), if its available storage space is significantly smaller than the database size. We will introduce a generic compiler that transforms any OT with a non-constant response size to one with a constant response size (see Section \ref{sec::the-compiler}).


\vspace{-1mm}
\subsubsection{Unconditionally Secure OT} 
The state-of-the-art \emph{unconditionally secure} OTs either (i) depend on the multi-sender setting, where each sender possesses a database replica, (ii) utilize a specific communication channel (i.e., noisy channel), or (iii) require the presence of a fully trusted initializer. Nevertheless, distributing the same database across multiple servers, establishing a highly specific communication channel, or involving a fully trusted party would increase the overall deployment cost of these schemes. We will propose Supersonic OT, an unconditionally secure highly efficient OT that does not have the above limitations (see Section \ref{sec::supersonice-OT}). We also implement it and evaluate its overhead in Section \ref{sec::supersonic-OT}. 



%Fourthly, the state-of-the-art \emph{unconditionally secure} techniques either (i) rely on the multi-sender setting where each of the senders holds a replica of the database, (ii) use a specific communication channel (i.e., noisy channel), or (iii) require the involvement of a fully trusted initialiser. However, distributing the same database among multiple servers, setting up (or using) a very specific communication channel, or involving a  fully trusted party would increase the overall deployment cost of the schemes.

\vspace{-3mm}


\subsection{Our Contributions}

\vspace{-1mm}


In this paper, we propose solutions to the aforementioned limitations using the following new techniques:

\vspace{-1mm}
\begin{enumerate}[leftmargin=5.5mm]
%
\item \underline{$1$-out-of-$2$ Delegated-Query Oblivious Transfer} \underline{(\dqot)}: a new notion of OT that (in addition to offering OT's basic features) enables a receiver to \emph{delegate} (i) the computation of the
query and (ii) interacting with the sender to a couple of potentially semi-honest parties, $\p_{\st 1}$
and $\p_{\st 2}$, while ensuring that the sender and receiver privacy is also protected from $\p_{\st 1}$ and $\p_{\st 2}$. Section \ref{sec::sec-def} presents \dqot. 
%
\begin{enumerate}

\item \underline{Delegated-Query OT (DQ-OT)}: a protocol that realizes\\   \dqot.  Section \ref{sec::DQ-OT} presents DQ-OT.

\item \underline{Delegate-Unknown-Query OT (DUQ-OT)}:  a variant of DQ-OT which allows the receiver to extract the related message $m_s$ even if it does not (and must not) know the related index $s$. Section \ref{sec::DUQ-OT-protocol} presents  DUQ-OT.
%
\end{enumerate}

\item {$1$-out-of-$2$ Delegated-Query Multi-Receiver OT} (\dqothf): a new notion of OT that (in addition to offering OT's primary features) ensures (i) a receiver learns nothing about the total number of records and their field elements and (ii) the sender who maintains $z$ records $[(m_{\st 0, 0}, m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})]$ does not find out which query belongs to which record. Section \ref{sec::DQOT-HF} presents \dqothf. 

\begin{enumerate}%[leftmargin=3.5mm]
%
\item  \underline{Delegated-Query Multi-Receiver OT (\rdqothf)}: an efficient protocol that realizes \dqothf. It is built upon DQ-OT and inherits its features. \rdqothf achieves its goal by allowing $\p_{\st 1}$ to know which record is related to which receiver.   Section \ref{sec::rdqothf} presents \rdqothf.
%
\item  \underline{Delegate-Unknown-Query Multi-Receiver OT}  \underline{(\rduqothf)}: a variant of \rdqothf which considers the case where  $\p_{\st 1}$ and $\p_{\st 2}$ do not (and must not) know which record in the database belongs to which receiver. Section \ref{sec::DUQ-OT-HF} presents \rduqothf. 
%
\end{enumerate}
%The protocols (such as \rdqothf and \rduqothf ) that realise \dqothf allow multiple physically separated sensitive databases to securely merge together.  

\item  \underline{A compiler}: a generic compiler that transforms any $1$-out-of-$n$ OT that requires the receiver to receive $n$ messages (as a response) into a $1$-out-of-$n$ OT that allows a receiver to (i) receive only a \emph{constant} number of messages and (ii) have constant storage space. Section \ref{sec::the-compiler} presents the compiler. 

\item \underline{Supersonic OT}: an unconditionally secure $1$-out-of-$2$ OT that \emph{does not} need to rely on (i) multiple senders, (ii) noisy channel, or (iii) the involvement of a trusted initializer. Section \ref{sec::supersonice-OT} presents Supersonic OT. Notably, Supersonic OT:

\begin{itemize}[leftmargin=4mm]
\item is fast as it does not involve any public-key-based tool.

\item enables the receiver to obtain a response of size $O(1)$.

\item takes only 0.35 milliseconds to complete its single execution. 

\item is about $10^{\st 3}$ times faster than the base OT in \cite{AsharovL0Z13} and up to around $2\times 10^{\st 3}$ times faster than the base OT in \cite{Efficient-OT-Naor}.
 
%\item is unconditionally secure

\end{itemize}


\end{enumerate} 

\vspace{-1mm}

\section{Preliminaries}

%\vspace{-1mm}
\subsection{Notations}\label{sec::notations}
By $\empt$ we mean an empty string.  

When $y$ represents a single value, $|y|$ refers to the bit length of $y$. However, when $y$ is a tuple, $|y|$ denotes the number of elements contained within $y$. We denote a sender by $\se$ and a receiver by $\re$. We assume parties interact with each other through a regular secure channel. 
%
We define a parse function as $\parse(\lambda, y)\rightarrow (\ux, \uy)$, which takes as input a value $\lambda$ and a value $y$ of length at least  $\lambda$-bit. It parses $y$ into two values  $\ux$ and $\uy$ and returns $(\ux, \uy)$ where the bit length of $\ux$ is $|y|-\lambda$ and the bit length of $\uy$ is  $\lambda$. 
%
Also, $U$ denotes a universe of messages $m_{\st 1},\ldots, m_{\st t}$. We define $\sigma$ as the maximum size of messages in $U$, i.e., $\sigma=Max(|m_{\st 1}|,\ldots, |m_{\st t}|)$. 
%
We use two hash functions $\h:\{0, 1\}^{\st *}\rightarrow \{0, 1\}^{\sigma}$ and $\g:\{0, 1\}^{\st *}\rightarrow \{0, 1\}^{\st\sigma+\lambda}$ modelled as random oracles \cite{Canetti97}. 


\vspace{-1mm}

\subsection{Security Model}\label{sec::sec-model}

In this paper, we use the simulation-based paradigm of secure multi-party computation \cite{GoldwasserMR85,DBLP:books/cu/Goldreich2004} to define and prove the proposed protocol. Since we focus on the  passive (semi-honest) adversarial model, we will restate the security definition in this model. 
%
 
 \subsubsection{Two-party Computation} A two-party protocol $\Gamma$ problem is captured by specifying a random process that maps pairs of inputs to pairs of outputs, one for each party. Such process is referred to as a functionality denoted by  $f:\{0,1\}^{\st  *}\times\{0,1\}^{\st  *}\rightarrow\{0,1\}^{ \st *}\times\{0,1\}^{ \st *}$, where $f:=(f_{\st  1},f_{\st  2})$. For every input pair $(x,y)$, the output pair is a random variable $(f_{\st  1} (x,y), f_{\st  2} (x,y))$, such that the party with input $x$ wishes to obtain $f_{\st  1} (x,y)$ while the party with input $y$ wishes to receive $f_{\st  2} (x,y)$. 
%
 %When $f$ is deterministic, then $f_{\st  1} =f_{ \st 2}$. 
 In the setting where $f$ is asymmetric and only one party (say the first one) receives the result, $f$ is defined as $f:=(f_{\st  1}(x,y), \empt)$. 
 
 
 \subsubsection{Security in the Presence of Passive Adversaries}  In the passive adversarial model, the party corrupted by such an adversary correctly follows the protocol specification. Nonetheless, the adversary obtains the internal state of the corrupted party, including the transcript of all the messages received, and tries to use this to learn information that should remain private. Loosely speaking, a protocol is secure if whatever can be computed by a party in the protocol can be computed using its input and output only. In the simulation-based model, it is required that a party’s view in a protocol's 
 execution can be simulated given only its input and output. This implies that the parties learn nothing from the protocol's execution. More formally, party $i$’s view (during the execution of $\Gamma$) on input pair  $(x, y)$ is denoted by $\mathsf{View}_{\st  i}^{\st  \Gamma}(x,y)$ and equals $(w, r_{\st  i}, m_{\st  1}^{\st  i}, ..., m_{\st  t}^{\st  i})$, where $w\in\{x,y\}$ is the input of $i^{\st  th}$ party, $r_{\st  i}$ is the outcome of this party's internal random coin tosses, and $m_{\st  j}^{\st  i}$ represents the $j^{\st  th}$ message this party receives.  The output of the $i^{\st  th}$ party during the execution of $\Gamma$ on $(x, y)$ is denoted by $\mathsf{Output}_{\st  i}^{\st  \Gamma}(x,y)$ and can be generated from its own view of the execution.  
\vspace{-1mm}
\begin{definition}
Let $f$ be the deterministic functionality defined above. Protocol $\Gamma$ securely computes $f$ in the presence of a  passive adversary if there exist polynomial-time algorithms $(\mathsf {Sim}_{\st  1}, \mathsf {Sim}_{\st  2})$ such that:
\end{definition}
%
\vspace{-1mm}
  \begin{equation*}
  \{\mathsf {Sim}_{\st 1}(x,f_{\st 1}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 1}^{\st \Gamma}(x,y) \}_{\st x,y}
  \end{equation*}
  %
  \begin{equation*}
    \{\mathsf{Sim}_{\st 2}(y,f_{\st 2}(x,y))\}_{ \st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 2}^{\st \Gamma}(x,y) \}_{\st x,y}
  \end{equation*}
  %
  \subsection{Random Permutation}
A random permutation $\pi(e_{\st 0} ,..., e_{\st n})\rightarrow(e'_{\st 0},..., e'_{\st n})$ is a probabilistic function that takes a set of $n$ elements $A=\{e_{\st 0}, ..., e_{\st n}\}$ and returns the same set elements in a permuted order $B=\{e'_{\st 0},..., e'_{\st n}\}$. The security of $\pi(.)$ requires that given set $B$ the probability that one can find the original index of an element $e'_{\st i}\in B$ is $\frac{1}{n}$.  In practice, the Fisher-Yates shuffle algorithm \cite{Knuth81} can permute a set of $n$ elements in time $O(n)$. We will use $\pi(.)$ in the protocols presented in Figures \ref{fig::DQ-OT-with-unknown-query} and \ref{fig::DQ-OT-with-unknown-query-and-HF-first-sevene-phases}.   





\subsection{Controlled Swap}\label{Customised-Random-Swap}
The idea of controlled swap was initially introduced by Fredkin and Toffoli  \cite{FredkinT02a}. It can be defined as a function $\cper(.)$ which takes two inputs: a binary value $s$ and a pair $(c_{\st 0}, c_{\st 1})$. When $s=0$, then it returns the input pair $(c_{\st 0}, c_{\st 1})$, i.e., it does not swap the elements. However, when $s=1$, then it returns $(c_{\st 1}, c_{\st 0})$, effectively swapping the elements. 
%
It is evident that if $s$ is uniformly chosen at random, then $\cper(.)$ represents a random permutation, implying that the probability of swapping or not swapping is $\frac{1}{2}$. We will use $\bar{\pi}(.)$ in the protocol presented in Figure \ref{fig::Ultrasonic-OT}.



\vspace{-2mm}
\subsection{Diffie-Hellman Assumption}\label{sec::dh-assumption}
Let $G$ be a group-generator scheme, which on input $1^{\st\lambda}$ outputs $(\mathbb{G}, p, g)$ where $\mathbb{G}$ is the description of a group, $p$ is the order of the group which is always a prime number, $\log_{\st 2}(p)=\lambda$ is a security parameter and $g$ is a generator of the group. In this paper, $g$ and $p$ can be selected by sender \se (in the context of OT). 

\subsubsection{Computational Diffie-Hellman (CDH) Assumption} 
We say that $G$ is hard under CDH assumption, if for any probabilistic polynomial time (PPT) adversary $\mathcal{A}$, given $(g^{\st a_1}, g^{\st a_2})$ it has only negligible probability to correctly compute $g^{\st a_1\cdot a_2}$. More formally, it holds that $Pr[\mathcal{A}(\mathbb{G}, p, g, g^{\st a_1}, g^{\st a_2})\rightarrow g^{\st a_1\cdot a_2}]\leq \mu(\lambda)$, where $(\mathbb{G}, p, g) \stackrel{\st\$}\leftarrow G(1^{\st\lambda})$, $a_{\st 1}, a_{\st 2} \stackrel{\st\$}\leftarrow \mathbb{Z}_{\st p}$, and $\mu$ is a negligible function  \cite{DiffieH76}.

%%%%%%%%%%%%%%%%%%%%%%%   DDH   %%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Decisional Diffie-Hellman (DDH) Assumption.} Informally, we say that $G$ is hard under the DDH assumption, if the distributions $(g^{a_1}, g^{a_2}, g^{a_1\cdot a_2})$ and $(g^{a_1}, g^{a_2}, g^w)$ are computationally indistinguishable when $a_1, a_2$, and $w$ are drawn at random from $\mathbb{Z}_p$. More formally,  
%for any PPT adversary $\mathcal{A}$, it holds that: 
%\vspace{-2mm}
%$$|Pr[\mathcal{A}(\mathbb{G}, p, g, g^{a_1}, g^{a_2}, g^{a_1\cdot a_2})]-Pr[\mathcal{A}(\mathbb{G}, p, g, g^{a_1}, g^{a_2}, g^w)]|\leq \epsilon(\lambda)$$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Oblivious Transfer (OT)}
% 
% OT is one of the important building blocks of cryptographic protocols and has been used in various protocols, such as Private, Set Intersection, Private Information Retrieval, and Zero-Knowledge Proofs. 
% %
% A 1-out-of-2 OT (\ot) is a protocol that often involves two parties, a sender and a receiver.  The sender has a pair of input messages $(m_0, x_1)$ and the receiver has a bit/index $s$. The aim of \ot is to allow the receiver to receive $m_s$, without revealing anything about $s$ to the sender, and without allowing the receiver to learn anything about  $m_{1-s}$. The \ot functionality is defined as $\mathcal{F}_{\ot}:((m_0, m_1), s) \rightarrow (\empt, m_s)$, where $\empt$ denotes the empty string. The security of \ot (in the passive adversarial model) requires that the view of each party during the protocol's execution can be simulated given only its input and output.  


\subsection{Secret Sharing}\label{sec::secret-haring}

A (threshold) secret sharing $\mathtt{SS}^{\st(t,n)}$  scheme is a cryptographic protocol that enables a dealer to distribute a string $s$, known as the secret, among $n$ parties in a way that the secret $s$ can be recovered when at least a predefined number of shares, say $t$, are combined. However, if the number of shares in any subset is less than $t$, the secret remains unrecoverable and the shares divulge no information about $s$. This type of scheme is commonly referred to as $(n, t)$-secret sharing or \secsh for brevity. 

In the case where $t=n$, there exists a highly efficient XOR-based secret sharing \cite{blakley1980one}. In this case, to share the secret $s$, the dealer first picks $n-1$ random bit strings $r_{\st 1}, ..., r_{\st n-1}$ of the same length as the secret. Then, it computes $r_{\st n} = r_{\st 1} \oplus, ..., \oplus  r_{\st n} \oplus s$. It considers each $r_{\st i}\in\{r_{\st 1},..,r_{\st n}\}$ as a share of the secret. To reconstruct the secret, one can easily compute $r_{\st 1}\oplus,..., \oplus r_{\st n}$. Any subset of less than $n$ shares reveals no information about the secret. We will use this scheme in this paper. A secret sharing scheme involves two main algorithms; namely, $\ses(1^{\st \lambda}, s, n, t)\rightarrow (r_{\st 1}, ..., r_{\st n})$: to share a secret and $\mathtt{RE}(r_{\st 1}, ..., r_{\st t}, n, t)\rightarrow s$ to reconstruct the secret. 


\subsection{Additive Homomorphic Encryption}\label{sec::AHE}


Additive homomorphic encryption involves three algorithms: (1) key generation: $\keygen(1^{\st\lambda})\rightarrow (sk, pk)$, which takes a security parameter as input and outputs a secret and public keys pair, (2) encryption: $\enc(pk, m)\rightarrow c$, that takes public key $pk$ and a plaintext message $m$ as input and returns a ciphertext $c$, and (3) decryption: $\dec(sk, c)\rightarrow m$, which takes secret key $sk$ and ciphertext $c$ as input and returns plaintext message $m$.  It has the following properties: 
 
 \begin{itemize}
 \item [$\bullet$]  Given two ciphertexts $\enc(pk, m_{\st 1})$ and $\enc(pk, m_{\st 2})$, one can compute the encryption of the sum of related plaintexts: 
 %
  $\dec(sk,\mathtt{Enc}(pk, m_{\st 1})\hadd \enc(pk, m_{\st 2}))= m_{\st 1}+m_{\st 2}$, where $\hadd$ denotes homomorphic addition.

  % $\mathtt{Enc}(pk, m_{\st 1})\hadd \enc(pk, m_{\st 2})=\enc(pk, m_{\st 1}+m_{\st 2})$
  
 \item [$\bullet$] Given a ciphertext $\mathtt{Enc}(pk, m)$ and a plaintext message $c$, one can compute the encryption of the product of related plaintexts: 
 %
 %$\enc(pk, m)\hmul c = \enc(pk, m\cdot c)$
 %
  $\dec(sk, \enc(pk, m)\hmul c) = m\cdot c$, where $\hmul$ denotes homomorphic multiplication.
 \end{itemize}
We require that the encryption scheme satisfies indistinguishability against chosen-plaintext attacks (IND-CPA).  We refer readers to \cite{KatzLindell2014} for a formal definition. One such scheme that meets the above features is the Paillier public key cryptosystem, proposed in \cite{Paillier99}. 



%Also, $\hadd$ and $\hmul$ denote homomorphic addition and multiplication respectively


\vspace{-2mm}
\section{Related Work}\label{sec::related-work}

%\subsection{Banking and Insider Threats}



 
 Oblivious Transfer (OT) is one of the important building blocks of cryptographic protocols and has been used in various mechanisms, such as private set intersection, generic secure multi-party computation, and zero-knowledge proofs. 
 %
 The traditional $1$-out-of-$2$ OT (\ot) is a protocol that involves two parties, a sender \se and a receiver \re.  \se has a pair of input messages $(m_{\st 0}, m_{\st 1})$ and \re has an index $s$. The aim of \ot is to allow \re to obtain $m_{\st s}$, without revealing anything about $s$ to \se, and without allowing \re to learn anything about  $m_{\st 1-s}$. The traditional \ot functionality is defined as $\mathcal{F}_{\st\ot}:((m_{\st 0}, m_{\st 1}), s) \rightarrow (\empt, m_{\st s})$.   %In general, OTs consider either active adversaries or passive ones. In this paper, our focus will be on the passive adversarial model.  The security of \ot (in the passive adversarial model) requires that the view of each party during the protocol's execution can be simulated given only its input and output.  
  
The notion of $1$-out-of-$2$ OT was initially proposed by Rabin \cite{Rabin-OT} which consequently was generalized by Even \et \cite{EvenGL85}. Since then, numerous variants of OT have been proposed. For instance, (i) $1$-out-of-$n$ OT, e.g., in \cite{NaorP99,Tzeng02,LiuH19}: which allows \re to pick one entry out of $n$ entries held by \se, (ii) $k$-out-of-$n$ OT, e.g., in \cite{ChuT05,JareckiL09,ChenCH10}: which allows \re to pick $k$ entries out of $n$ entries held by \se, (iii) OT extension, e.g., in \cite{IshaiKNP03,Henecka013,Nielsen07,AsharovL0Z13}: that supports efficient executions of OT (that mainly relies on symmetric-key operations), in the case OT needs to be invoked many times, and (iv) distributed OT, e.g., in \cite{NaorP00,CorniauxG13,ZhaoSJMZX20}: that allows the database to be distributed among $m$ servers/senders. %Since the latter variant is closest to our work, in the remainder of this section we elaborate on this variant. 

In the remainder of this section, we discuss several variants of OT  that have extended and enhanced the original OT in \cite{Rabin-OT}. 

\vspace{-2mm}
\subsection{Distributed OT} 

 Naor and Pinkas \cite{NaorP00} proposed several protocols for distributed OT where the role of sender \se (in the original OT) is divided between several servers.  In these schemes, a receiver must contact a threshold of the servers to run the OT. 
 
 The proposed protocols are in the semi-honest model. They use symmetric-key primitives and do not involve any modular exponentiation that can lead to efficient implementations.  These protocols are based on various variants of polynomials (e.g., sparse and bivariate), polynomial evaluation, and pseudorandom function. In these distributed OTs, the security against the servers holds as long as less than a predefined number of these servers collude. 
 %
 Later, various distributed OTs have been proposed\footnote{Distributed OT has also been called proxy OT in \cite{YaoF06}.}. For instance, Corniaux and Ghodosi \cite{CorniauxG13} proposed a verifiable $1$-out-of-$n$ distributed OT that considers the case where a threshold of the servers are potentially active adversaries. The scheme is based on a sparse $n$-variate polynomial, verifiable secret sharing, and error-correcting codes. 
 
 Moreover, Zhao \et  \cite{ZhaoSJMZX20} has proposed a distributed version of OT extension that aims to preserve the efficiency of OT extension while delegating the role of \se to multiple servers a threshold of which can be potentially semi-honest. The scheme is based on a hash function and an oblivious pseudorandom function.  

 
 
 
 But, there exists no OT that supports the delegation of the query computation to third-party servers in a privacy-preserving manner. 

\vspace{-3mm}

\subsection{Multi-Receiver OT}\label{sec::multi-rec-ot}

Camenisch \et \cite{CamenischDN09} proposed a protocol for ``OT with access control''. This protocol involves a set of receivers and a sender which maintains records of the receivers. It offers a set of interesting features; namely, (i) only authorized receivers can access certain records; (ii) the sender does not learn which record a receiver accesses, and (iii) the sender does not learn which roles (or security clearance) the receiver has when it accesses the records. 
%
In this scheme, during the setup, the sender encrypts all records (along with their field elements) and publishes the entire encrypted database for the receivers to download. Subsequently, researchers proposed various variants of OT with access control, as seen in \cite{CamenischDNZ11,CamenischDEN12,CamenischDN10,AielloIR01,WangTS10}. 

Nevertheless, in all of the aforementioned schemes, the size of the entire database is revealed to the receivers.




\vspace{-2mm}

\subsection{OT with Constant Response Size}

Researchers have proposed several OTs, e.g., those proposed in \cite{CamenischNS07,GreenH08,ZhangLWR13,KurosawaNP10,CamenischDN09},  that enable a receiver to obtain a constant-size response to its query. To achieve this level of communication efficiency, these protocols require the receiver to locally store the encryption of the entire database, in the initialization phase. During the transfer phase, the sender assists the receiver with locally decrypting the message that the receiver is interested in. 

The main limitation of these protocols is that a thin client with limited available storage space cannot use them, as it cannot locally store the encryption of the entire database.  


\vspace{-2mm}

\subsection{Unconditionally Secure OT}\label{sec::uncon-sec-OT} There have been efforts to design (both-sided) unconditionally secure OTs. Some schemes, e.g., the ones in   \cite{NaorP00,BlundoDSS07,CorniauxG13}, rely on multiple servers/senders that maintain an identical copy of the database.  Other ones, e.g., those in \cite{CrepeauK88,CrepeauMW04,IshaiKOPSW11}, rely on a specific network structure, i.e., a noisy channel, to achieve unconditionally secure OT.   There is also a scheme in \cite{rivest1999unconditionally} that achieves unconditionally secure OT using a fully trusted initializer.  

Hence, there exists no (efficient) unconditionally secure OT that does not rely on noisy channels, multi-server, and fully trusted initializer. 
%
We refer readers to \cite{OT-Survey} for a recent survey of OT.
%

\vspace{-2mm}
\section{Delegated-Query OT}\label{sec:protocol}
In this section, we present the notion of Delegated-Query $1$-out-of-$2$ OT (\dqot) and a protocol that realizes it. 
%
 \dqot involves four parties; namely, sender \se, receiver \re, and two helper servers $\p_{\st 1}$ and $\p_{\st 2}$ that assist \re to compute the query.  



Informally, \dqot enables \re to delegate (i) the computation of query and (ii) the interaction with \se to $\p_{\st 1}$ and $\p_{\st 2}$, who jointly compute \re's query and send it to \se.  
%
\dqot (in addition to offering the basic security of OT) ensures that \re's privacy is preserved from  $\p_{\st 1}$ and $\p_{\st 2}$, in the sense that  $\p_{\st 1}$ and $\p_{\st 2}$ do not learn anything about the actual index (i.e., $s\in\{0,1\}$) that \re is interested in, as long as they do not collude with each other. 



%\subsection{Motivation}\label{sec::motivation-DQ-OT}


%%%%%%%

%For instance,  in the case where a (cloud) database holds records of multiple companies if an employee of one of the companies uses an existing technique to interact with the database, it will learn the entire size of the database. In this case, the receiver can learn the number of records other companies had in the same database, given some public auxiliary information. An example of this auxiliary information is that British Airways, Boots, and BBC data were kept by the same cloud, according to the very recent cyber-attack \cite{BBB-hack}. To address the size-leakage issue, one may be tempted to (a) allocate a physically separated database to each receiver (or a set of receivers), which would (i) increase the size of the entire database linearly with the number of receivers or types of security clearance and (ii) allow the sender to learn the type of security clearance that each receiver has(i.e., which receiver can access to which records), or (b) allow the receiver to declare to the sender the record's index/ID it wants to access which would also enable the sender to learn the security clearance of the receiver.   

%%%%%%%%


%
%\subsubsection{Dealing with Insider in Financial Institutions} 
%Insider attacks are real and imminent threats to the financial institutions and their customers. Insider adversaries may collude with and help external fraudsters. The data that insider adversaries can gather about their customers is extremely valuable. The ``Swiss Leaks''~\cite{leigh2015hsbc} is a good example to illustrate the problem of insider leaks in the banking world.  In the Swiss Leaks case, an insider attempted to sell information about accounts held by HSBC in Geneva. Later, when he failed, he leaked the information to the public.  As another example, in the case of ``JPMorgan Chase Insider Thief'' \cite{JPMorgan}, a former JPMorgan Chase personal banker has been arrested by the FBI on charges that he stole customer account information and sold it to an undercover informant. 
%
%
%In this context, an insider can exclusively target  high-profile wealthy individuals and sell the victims' information to their rivals, who might make strategic investments, often remaining stealthy from the victims' perspective. For an insider, a data breach in private banking or private financial advising can be more alluring than leaking hundreds of bank accounts. Indeed, the former could yield a higher payoff while concurrently posing a lower risk of exposure.
%
%In this setting, financial advisors, within a financial institution, frequently maintain paid subscriptions to a valuable database (e.g., containing real estate market information, market trends, and capital flows) offered by third-party providers such as CoreLogic\footnote{\url{https://www.corelogic.com/data-solutions/property-data-solutions/discovery-platform/}},  Multiple Listing Service\footnote{\url{https://www.mls.com/}}, or Real Capital Analytics\footnote{https://www.msci.com/our-solutions/real-assets/real-capital-analytics}.  In contrast, clients of these advisors do not necessarily need to subscribe to the database themselves. Instead, they interact with the advisors and direct their queries to them.
%
%
%Outsiders who infiltrate the computers of an individual advisor or the third-party's database can compromise the privacy of customers' queries as well.
%
%Hence, there is a pressing need to (i) safeguard the privacy of customers' queries from advisors and databases, (ii) ensure the privacy of the database from both customers and advisors, and (iii) secure the privacy of customers in the event of a data breach on the advisor's or database's side. Achieving these objectives constitutes the primary goal of this section.





\vspace{-1.4mm}
\subsection{Functionality Definition}

Informally, the functionality that \dqot computes takes as input (i) a pair of messages $(m_{\st 0}, m_{\st 1})$ from \se, (ii) empty string  \empt from $\p_{\st 1}$, (iii)  empty string  \empt from $\p_{\st 2}$, and (iv) the index  $s$ (where $s\in \{0, 1\}$) from \re. It outputs an empty string $\empt$ to  \se, $\p_{\st 1}$, and $\p_{\st 2}$, and outputs the message with index $s$, i.e., $m_{\st s}$, to \re.  Formally, we define the functionality as: 
%
 $\mathcal{F}_{\scriptscriptstyle\dqot}:\big((m_{\st 0}, m_{\st 1}), \empt, \empt, s\big) \rightarrow (\empt, \empt, \empt, m_{\st s})$.
 
 
 
 \vspace{-1.2mm}
 \subsection{Security Definition}\label{sec::sec-def}
 \vspace{-1mm}
 
 Next, we present a formal definition of \dqot. 


\begin{definition}[\dqot]\label{def::DQ-OT-sec-def} Let $\mathcal{F}_{\scriptscriptstyle\dqot}$ be the delegated-query OT functionality defined above. We say protocol $\Gamma$ realizes $\mathcal{F}_{\scriptscriptstyle\dqot}$ in the presence of passive adversary \se, \re, $\p_{\st 1}$, or $\p_{\st 2}$ if for  every non-uniform PPT adversary \adv
in the real model, there exists a non-uniform PPT adversary (or simulator) \simm  in
the ideal model, such that:
%
\vspace{-1mm}
%{\small{
\begin{equation}\label{equ::sender-sim-}
\begin{split}
\Big\{\simm_{\st\se}\big((m_{\st 0}, m_{\st 1}), \empt\big)\Big\}_{\st m_{\st 0}, m_{\st 1}, s}\stackrel{c}{\equiv}\\ \Big\{\view_{\st\se}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, s\big) \Big\}_{ m_{\st 0}, m_{\st 1}, s}
\end{split}
\end{equation}

\begin{equation}\label{equ::server-sim-}
\begin{split}
\Big\{\simm_{\st\p_i}(\empt, \empt)\Big\}_{\st m_{\st 0}, m_{\st 1}, s}\stackrel{c}{\equiv} \\    \Big\{\view_{\st\p_i}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, s\big) \Big\}_{\st\st m_{\st 0}, m_{\st 1}, s}
\end{split}
\end{equation}

\begin{equation}\label{equ::reciever-sim-}
\begin{split}
\Big\{\simm_{\st\re}\Big(s, \mathcal{F}_{\scriptscriptstyle\dqot}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, s\big)\Big)\Big\}_{\st m_{\st 0}, m_{\st 1}, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\re}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, s\big) \Big\}_{\st m_{\st 0}, m_{\st 1}, s}
\end{split}
\end{equation}
%}}
\vspace{-2mm}
for all $i$,  $i\in \{1,2\}$.


%%
%%
\end{definition}
Intuitively, Relation \ref{equ::sender-sim-} states that the view of a corrupt \se during the execution of protocol $\Gamma$ (in the real model) can be simulated by a simulator $\simm_{\st\se}$ (in the ideal model) given only \se's input and output, i.e., $(m_{\st 0}, m_{\st 1})$ and \empt respectively. 

Relation \ref{equ::server-sim-} states that the view of each corrupt server $\p_{\st i}$ during the execution of  $\Gamma$ can be simulated by a simulator $\simm_{\st\p_i}$ given only $\p_{\st i}$'s input and output, i.e., $\empt$ and $\empt$ respectively. 

Relation \ref{equ::reciever-sim-} states that the view of a corrupt \re during the execution of $\Gamma$ can be simulated by a simulator $\simm_{\st\re}$ given only \re's input and output, i.e., $s$ and $m_{\st s}$ respectively. 



A \dqot scheme meets two properties, \textit{efficiency} and \textit{sender-push communication} (\spc). 
%
Informally, efficiency states that the query generation of the receiver is faster compared to traditional (non-delegated) OT. 
%
\spc, on the other hand, stipulates that the sender transmits responses to the receiver without requiring the receiver to directly initiate a query to the sender.

Appendix \ref{sec::properties-definitions}, presents formal definitions of efficiency and \spc. 



\subsection{Protocol}\label{sec::DQ-OT}
Now, we present an efficient 1-out-of-2 OT protocol, called DQ-OT, that realizes \dqot. 
%DQ-OT allows the receiver to delegate the generation and sending of its query (i.e., encoded index) to two non-colluding servers that are potentially passive adversaries, e.g., they may try to learn about the index in which the sender is interested, or the sender's plaintext message(s) $(m_0, m_1)$.  
%
We build DQ-OT upon the \ot proposed by  Naor and Pinkas  \cite[pp. 450, 451]{Efficient-OT-Naor}. Our motivation for this choice is primarily didactic. Appendix \ref{sec::OT-of-Naor-Pinkas} restates this OT. 


The high-level idea behind the design of DQ-OT is that \re splits its index into two shares and sends each share to each $\p_{\st i}$. Subsequently, each $\p_{\st i}$ computes a (partial) query and sends the result to  \se which generates the response for \re in the same manner as the original OT in \cite{Efficient-OT-Naor}. 
%
%The primary challenge is to \emph{ensure correctness} while preserving privacy. 
%
Below, we provide an explanation of how  DQ-OT operates, followed by an explanation of how it achieves  correctness. 



First, \re splits the index that it is interested in into two binary shares,  $(s_{\st 1}, s_{\st 2})$. Then, it picks two random values, $(r_{\st 1}, r_{\st 2})$, and then sends each pair $(s_{\st i}, r_{\st i})$ to each $\p_{\st i}$. 

Second, to compute a partial query, $\p_{\st 2}$ treats $s_{\st 2}$ as the main index that \re is interested in and computes a partial query, $\delta_{\st s_2}=g^{\st r_2}$. Also $\p_{\st 2}$  generates another query, $\delta_{\st 1-s_2}=\frac{C}{g^{\st r_2}}$, where $C$ is a random public parameter (as defined in \cite{Efficient-OT-Naor}). $\p_{\st 2}$ sorts the two queries in ascending order based on the value of $s_{\st 2}$ and sends the resulting $(\delta_{\st 0}, \delta_{\st 1})$ to $\p_{\st 1}$. 



Third, to compute its queries, $\p_{\st 1}$ treats $\delta_{\st 0}$ as the main index (that \re is interested) and computes $\beta_{\st s_1}=\delta_{\st 0}\cdot g^{\st r_1}$. Additionally, it generates another query $\beta_{\st 1-s_1}=\frac{\delta_{\st 1}}{g^{\st r_1}}$. Subsequently, $\p_{\st 1}$ sorts the two queries in ascending order based on the value of ${s_{\st 1}}$ and sends the resulting $(\beta_{\st 0}, \beta_{\st 1})$ to $\re$. 

Forth, given the queries, \se computes the response in the same manner it does in the original OT in \cite{Efficient-OT-Naor} and sends the result to \re who extracts from it, the message that it asked for, with the help of $s_i$ and $r_i$ values.  
%
The detailed  DQ-OT  is presented in Figure \ref{fig::DQ-OT}. 


\vspace{-1mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!htbp]
\vspace{-2mm}
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=85mm, height=131mm, left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\vspace{-2.2mm}
\begin{enumerate}[leftmargin=4.8mm]
%

\item \underline{\textit{$\se$-side Initialization:}} 
%
$\mathtt{Init}(1^{\st \lambda})\rightarrow pk$
%
\begin{enumerate}

\item chooses a sufficiently large prime number $p$.

\item selects random element
$C \stackrel{\st \$}\leftarrow \mathbb{Z}_p$ and generator $g$.
\item publish $pk=(C, p, g)$. 

\end{enumerate}









\item \underline{\textit{\re-side Delegation:}}
%
$\mathtt{Request}(1^{\st \lambda}, s, pk)\hspace{-.6mm}\rightarrow\hspace{-.6mm} req=(req_{\st 1}, req_{\st 2})$
%


\begin{enumerate}

\item split  the private index $s$ into two shares $(s_{\st 1}, s_{\st 2})$ by calling  $\ses(1^{\st \lambda}, s, 2, 2)\rightarrow (s_{\st 1}, s_{\st 2})$.

\item pick two uniformly random values: $r_{\st 1}, r_{\st 2} \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.

\item send $req_{\st 1}=(s_{\st 1}, r_{\st 1})$ to $\p_{\st 1}$ and $req_{\st 2}=(s_{\st 2}, r_{\st 2})$ to $\p_{\st 2}$.

\end{enumerate}

\item \underline{\textit{$\p_{\st 2}$-side Query Generation:}}
%
$\mathtt{\p_{\st 2}.GenQuery}(req_{\st 2}, ,pk)\rightarrow q_{\st 2}$
%

\begin{enumerate}

\item compute a pair of partial queries:
%
  $$\delta_{\st s_2}= g^{\st r_2},\ \  \delta_{\st 1-s_{\st 2}} = \frac{C}{g^{\st r_2}}$$
  
\item send $q_{\st 2}=(\delta_{\st 0}, \delta_{\st 1})$ to  $\p_{\st 1}$. 

\end{enumerate}

\item\underline{\textit{$\p_{\st 1}$-side Query Generation:}}
$\mathtt{\p_{\st 1}.GenQuery}(req_{\st 1}, q_{\st 2},pk)\rightarrow q_{\st 1}$


\begin{enumerate}

\item compute a pair of final queries as: 
%
$$\beta_{s_{\st 1}}=\delta_{\st 0}\cdot g^{\st r_{\st 1}},\ \ \beta_{\st 1-s_1}=\frac{\delta_{\st 1}} {g^{\st r_{\st 1}}}$$

\item send $q_{\st 1}=(\beta_{\st 0}, \beta_{\st 1})$ to  $\se$.

\end{enumerate}

\item\underline{\textit{\se-side Response Generation:}}  
%
$\mathtt{GenRes}(m_{\st 0}, m_{\st 1}, pk, q_{\st 1})\rightarrow res$
%
\begin{enumerate}

\item abort if  $C \neq \beta_{\st 0}\cdot \beta_{\st 1}$.
    %
\item pick two uniformly random values: 
%
$y_{\st 0}, y_{\st 1}  \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.
    %
\item compute a response pair $(e_{\st 0}, e_{\st 1})$ as follows:
 $$e_{\st 0} := (e_{\st 0,0}, e_{\st 0,1}) = (g^{\st y_0}, \h(\beta_{\st 0}^{\st y_0}) \oplus m_{\st 0})$$
    %
$$e_{\st 1} := (e_{\st 1,0}, e_{\st 1,1}) = (g^{\st y_1}, \h(\beta_{\st 1}^{\st y_1}) \oplus m_{\st 1})$$
    %  
\item send $res=(e_{\st 0}, e_{\st 1})$ to \re. 

\end{enumerate}

\item\underline{\textit{\re-side Message Extraction:}} 
%
$\mathtt{Retreive}(res, req, pk)\hspace{-.6mm}\rightarrow\hspace{-.8mm} m_{\st s}$
%
\begin{enumerate}

\item set $x=r_{\st 2}+r_{\st 1}\cdot(-1)^{\st s_{\st 2}}$

\item retrieve the related message: 

$m_{\st s}=\h((e_{\st s, 0})^{\st x})\oplus e_{\st s, 1}$

\end{enumerate}

\end{enumerate}
%%%%%%%%%%%%%%%
\end{tcolorbox}
\end{center}
\vspace{-3mm}
\caption{DQ-OT: Our $1$-out-of-$2$ OT that supports query delegation. The input of \re is a private binary index $s$ and the input of \se is a pair of private messages $(m_{\st 0}, m_{\st 1})$. Note, $g$ is a generator and $C=g^{\st a}$ is a random public value (e.g., both of which initially generated by \se), $\ses(.)$ is the share-generation algorithm (of a secret sharing) defined in Section \ref{sec::secret-haring}, $\h(.)$ is a hash function, and $\$$ denotes picking a value uniformly at random.} 
\vspace{-3mm}
\label{fig::DQ-OT}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{theorem}\label{theo::DQ-OT-sec}
%
Let $\mathcal{F}_{\scriptscriptstyle\dqot}$ be the functionality defined in Section \ref{sec::sec-def}. If  
Discrete Logarithm (DL), Computational Diffie-Hellman (CDH), and Random Oracle (RO) assumptions hold, then DQ-OT (presented in Figure \ref{fig::DQ-OT}) securely computes $\mathcal{F}_{\scriptscriptstyle\dqot}$ in the presence of semi-honest adversaries,
% (a) semi-honest receiver \re, honest sender \se, and honest servers $\p_{\st 1}$ and $\p_{\st 2}$, (b) semi-honest \se, honest \re, and honest $\p_{\st 1}$ and $\p_{\st 2}$, or (c) semi-honest $\p_{\st i}$ (where $i\in \{1, 2\}$), honest \se, and honest \se, 
w.r.t. Definition \ref{def::DQ-OT-sec-def}. 

\end{theorem}

Appendix \ref{sec::DQ-OT-proof} presents the proof of Theorem \ref{theo::DQ-OT-sec}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Correctness}

In this section, we discuss why the correctness of DQ-OT always holds. Recall, in the original OT of Naor and Pinkas \cite{Efficient-OT-Naor}, the random value $a$ (i.e., the discrete logarithm of random value $C$) is inserted by receiver \re into the query $\beta_{\st 1-s}$ whose index (i.e., $1-s$) is not interesting to \re while the other query $\beta_{\st s}$ is free from value $a$. As we will explain below, in our DQ-OT, the same applies to the final queries that are sent to \se.  
%
Briefly, in DQ-OT, when:

\begin{itemize}

\item[$\bullet$]  $s=s_{\st 1}\oplus s_{\st 2}=1$ (i.e., when $s_{\st 1}\neq s_{\st 2}$), then $a$ will always appear in $\beta_{\st 1-s}=\beta_{\st 0}$; however, $a$ will not appear in $\beta_{\st 1}$. 

\item[$\bullet$] $s=s_{\st 1}\oplus s_{\st 2} = 0$ (i.e., when $s_{\st 1}=s_{\st 2}$), then $a$ will always appear in $\beta_{\st 1-s}=\beta_{\st 1}$; but $a$ will not appear in $\beta_{\st 0}$.

\end{itemize}

This is evident in Table~\ref{tab:analysis} which shows what
$\delta_{\st i}$ and $\beta_{\st j}$ are for the different values of $s_{\st 1}$ and $s_{\st 2}$. Therefore, the query pair ($\beta_{\st 0}, \beta_{\st 1}$) has the same structure as it has in \cite{Efficient-OT-Naor}. 

\vspace{-1mm}

\begin{table}[h]
\vspace{-1mm}
\begin{center}
\scalebox{.76}{
  \begin{tabular}{|l||p{4.5cm}|p{4.5cm}|}
\hline
    &\multicolumn{1}{c|}{$s_{\st 2}=0$}&\multicolumn{1}{c|}{$s_{\st 2}=1$}\\
\hline
\hline
&\cellcolor{gray!20}$\delta_{\st 0} = g^{\st r_2}$, \hspace{3mm} $\delta_{\st 1} = g^{\st a-r_2}$&\cellcolor{gray!20} $\delta_{\st 0}=g^{\st a-r_2}$,\hspace{3mm} $\delta_{\st 1}=g^{\st r_2}$\\
\multirow{-2}{*}{$s_{\st 1}=0$}&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st r_2+r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st a-r_2-r_1}$&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st a-r_2+r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st r_2-r_1}$\\
\hline
&\cellcolor{gray!20}$\delta_{\st 0}=g^{\st r_2}$, \hspace{3mm} $\delta_{\st 1}=g^{\st a-r_2}$&\cellcolor{gray!20}$\delta_{\st 0}=g^{\st a-r_2}$, \hspace{3mm} $\delta_{\st 1}=g^{\st r_2}$\\
\multirow{-2}{*}{$s_{\st 1}=1$}&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st a-r_2-r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st r_2+r_1}$&\cellcolor{gray!20}$\beta_{\st 0}=g^{\st r_2-r_1}$, \hspace{3mm} $\beta_{\st 1}=g^{\st a-r_2+r_1}$\\
\hline
\end{tabular}
}
\end{center}
\caption{$\delta_{\st i}$ and $\beta_{\st j}$ are for the different values of $s_{\st 1}$ and $s_{\st 2}$.
We express each value as a power of $g$.}
\label{tab:analysis}
\vspace{-3mm}
\end{table}

Next, we show why, in DQ-OT, \re can extract the correct message, i.e., $m_s$. Given \se's reply pair $(e_{\st 0}, e_{\st 1})$ and its original index $s$, \re knows which element to pick from the response pair, i.e., it picks $e_{\st s}$.  


%\vspace{-1mm}
Moreover, given $g^{\st y_s}\in e_{\st s}$, \re can  recompute $\h(g^{\st y_s})^{\st x}$, as it knows the value of $s, s_{\st 1}$, and $s_{\st 2}$.  Specifically, as Table~\ref{tab:analysis} indicates, when: 

\begin{itemize}
\item[$\bullet$]  $\overbrace{(s= s_{\st 1}=s_{\st 2}=0)}^{\st \text{Case 
 1}}$ or $\overbrace{(s=s_{\st 1}=1 \wedge s_{\st 2}=0)}^{\st \text{Case 
 2}}$, then \re can set $x = r_{\st 2} + r_{\st 1}$.

\begin{itemize}

 \item In Case 1, it holds $\h((g^{\st y_0})^{\st x})= \h((g^{\st y_0})^{\st r_2 +r_1})=q$. Also, $e_{\st 0}=\h(\beta_{\st 0}^{\st y_0})\oplus m_{\st 0}=\h((g^{\st r_2+r_1})^{\st y_0})\oplus m_{\st 0}$. Thus, $q\oplus e_{\st 0}=m_{\st 0}$.
 
 \item In Case 2, it holds $\h((g^{\st y_1})^{\st x})= \h((g^{\st y_1})^{\st r_2 +r_1})=q$. Moreover, $e_{\st 1}=\h(\beta_{\st 1}^{\st y_1})\oplus m_{\st 1}=\h((g^{\st r_2+r_1})^{\st y_1})\oplus m_{\st 1}$. Hence, $q\oplus e_{\st 1}=m_{\st 1}$.

 
 \end{itemize}

 \vspace{.6mm} 
 
%
\item[$\bullet$]  $\overbrace{(s=0 \wedge s_{\st 1}=s_{\st 2}=1)}^{\st \text{Case 
 3}}$ or $\overbrace{(s=s_{\st 2}=1 \wedge s_{\st 1}=0)}^{\st \text{Case 
 4}}$, then \re can set $x = r_{\st 2} - r_{\st 1}$.
%

\begin{itemize}

 \item In Case 3, it holds $\h((g^{\st y_0})^{\st x})= \h((g^{\st y_0})^{\st r_2 - r_1})=q$. On the other hand, $e_{\st 0}=\h(\beta_{\st 0}^{\st y_0})\oplus m_{\st 0}=\h((g^{\st r_2 - r_1})^{\st y_0})\oplus m_{\st 0}$. Therefore, $q\oplus e_{\st 0}=m_{\st 0}$.
 
 \item In Case 4, it holds $\h((g^{\st y_1})^{\st x})= \h((g^{\st y_1})^{\st r_2 -r_1})=q$. Also, $e_{\st 1}=\h(\beta_{\st 1}^{\st y_1})\oplus m_{\st 1}=\h((g^{\st r_2-r_1})^{\st y_1})\oplus m_{\st 1}$. Hence, $q\oplus e_{\st 1}=m_{\st 1}$.
 
 \end{itemize}

%
\end{itemize}

We conclude that DQ-OT always allows honest \re to recover the message of its interest, i.e., $m_s$.   

\section{Delegated-Unknown-Query OT}\label{sec::DUQ-OT}

%The database $D$ will, similarly to Bellare-Micali, send $R$ the following:
%$\alpha_i=g^{y_i}$, where $y_i\in_R Z_q$ ($i\in {0,1}$)
%and $c_0=m_0\oplus \beta_0^{y_0}$ and $c_1=m_1\oplus \beta_1^{y_1}$, where
%$m_i$ is the plaintext in the database.
%
%When $P_i$ privately give $s_i,r_i$ ($i\in \{1,2\}$) to
%$R$, then $R$ can decrypt in a straightforward way.
%(Note that $s_i$ might have been chosen by $R$, in
%which case only $r_i$ is needed.)
%We now motivate an alternative approach to $R$ decrypting.

In certain cases, the receiver itself may not know the value of query $s$. Instead, the query is issued by a third-party query issuer (\tp). %An example in the context of banking is that customers \re do not know whether they are premium ones or not. %In that case only $r_2$ needs to be revealed to $R$; as we explain in Section \ref{sec:Alternative-decryption}.

In this section, we present a new variant of \dqot, called Delegated-Unknown-Query 1-out-of-2 OT (\duqot). It enables \tp to issue the query while (a) preserving the security of  \dqot and (b) preserving the privacy of query $s$ from \re.  


%
%\subsection{Motivation}\label{sec::elegated-Unknown-Query-OT-motivation}
%
%In the context of financial institutions, there exist specific details about customers that the financial institutions must not disclose to the customers. These details are generally related to security measures, proprietary systems, and certain operational aspects, such as (a) fraud prevention measures, including a binary flag that determines whether a certain customer is deemed suspicious \cite{arora2023privacy}, or (b) proprietary banking strategies, developed by banks for risk management, investment, and financial planning related to each client. 
%
%
%Therefore, in certain cases, the result that a client/receiver obtains for its request depends on the  private flag/query $s$ that a financial institution (as $\tp$) provides to its financial advisor who is directly dealing with the client, while the client itself is not aware of the value of $s$.  

\subsection{Security Definition}\label{sec::DUQ-OT-definition}

The functionality that \duqot computes takes as input (a) a pair of messages $(m_{\st 0}, m_{\st 1})$ from \se, (b) empty strings \empt from $\p_{\st 1}$, (c)  \empt from $\p_{\st 2}$, (d)   \empt from $\re$, and (e) the index $s$ (where $s\in \{0, 1\}$) from \tp. It outputs an empty string $\empt$ to  \se, \tp, $\p_{\st 1}$, and $\p_{\st 2}$, and outputs the message with index $s$, i.e., $m_{\st s}$, to \re. More formally, we define the functionality as: 
%
 $\mathcal{F}_{\scriptscriptstyle\duqot}:\big((m_{\st 0}, m_{\st 1}), \empt, \empt, \empt, s\big) \rightarrow (\empt, \empt, \empt, m_{\st s}, \empt)$. 
% 
Next, we present a formal definition of \duqot. 


\begin{definition}[\duqot]\label{def::DUQ-OT-sec-def} Let $\mathcal{F}_{\scriptscriptstyle\duqot}$ be the functionality defined above. We assert that protocol $\Gamma$ realizes $\mathcal{F}_{\scriptscriptstyle\duqot}$ in the presence of passive adversary \se, \re, $\p_{\st 1}$, or $\p_{\st 2}$, if for  every PPT adversary \adv
in the real model, there exists a non-uniform PPT simulator \simm  in
the ideal model, such that:
%
%{\small{
\begin{equation}\label{equ::DUQ-OT-sender-sim-}
\begin{split}
\Big\{\simm_{\st\se}\big((m_{\st 0}, m_{\st 1}), \empt\big)\Big\}_{\st m_{\st 0}, m_{\st 1}, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st \se}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, \empt, s\big) \Big\}_{\st m_{\st 0}, m_{\st 1}, s}
\end{split}
\end{equation}
%
\begin{equation}\label{equ::DUQ-OT-server-sim-}
\begin{split}
\Big\{\simm_{\st\p_i}(\empt, \empt)\Big\}_{\st m_{\st 0}, m_{\st 1}, s}\stackrel{c}{\equiv}\\ 
\Big\{\view_{\st\p_i}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, \empt, s\big) \Big\}_{\st m_0, m_1, s}
\end{split}
\end{equation}
%
\begin{equation}\label{equ::DUQ-OT-t-sim-}
\begin{split}
\Big\{\simm_{\st\tp}(s, \empt)\Big\}_{\st m_0, m_1, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\tp}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, \empt, s\big) \Big\}_{\st m_0, m_1, s}
\end{split}
\end{equation}
%
\begin{equation}\label{equ::DUQ-OT-reciever-sim-}
\begin{split}
\Big\{\simm_{\st\re}\Big(\empt, \mathcal{F}_{\scriptscriptstyle\duqot}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt,\empt, s\big)\Big)\Big\}_{\st m_0, m_1, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\re}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  \empt, \empt, s\big) \Big\}_{\st m_0, m_1, s}
\end{split}
\end{equation}



%}}
for all $i$,  $i\in \{1,2\}$. Since \duqot, is a variant of \dqot, it also supports efficiency and \spc, as discussed in Section \ref{sec::sec-def}.


%%
%%
\end{definition}




\subsection{Protocol}\label{sec::DUQ-OT-protocol}
In this section, we present DUQ-OT that realizes \duqot.  

\subsubsection{Main Challenge to Overcome} 
One of the primary differences between DUQ-OT and previous OTs in the literature (and DQ-OT) is that in DUQ-OT, \re does not know the secret index $s$. The knowledge of $s$ would help \re pick the suitable element from \se's response; for instance, in the DQ-OT, it picks  $e_s$ from $(e_{\st 0}, e_{\st 1})$. Then, it can extract the message from the chosen element. In DUQ-OT, to enable \re to extract the desirable message from \se's response without the knowledge of $s$, we rely on the following observation and technique. 

We know that (in any OT) after decrypting $e_{\st s-1}$, \re would obtain a value indistinguishable from a random value (otherwise, it would learn extra information about $m_{\st s-1}$). 
Therefore, if \se imposes a certain publicly known structure to messages $(m_{\st 0}, m_{\st 1})$, then after decrypting \se's response, only $m_{\st s}$ would preserve the same structure. 

In DUQ-OT, \se imposes a publicly known structure to $(m_{\st 0}, m_{\st 1})$  and then computes the response. Given the response, \re tries to decrypt \emph{every} message it received from \se and accepts only the result that has the structure.


\subsubsection{An Overview} 
Briefly, DUQ-OT operates as follows. First, \re picks two random values and sends each to a $\p_{\st i}$. Also, \tp splits the secret index $s$ into two shares and sends each share to a $\p_{\st i}$. Moreover, \tp selects a random value $r_{\st 3}$ and sends it to \re and \se. Given the messages received from \re and \tp, each $\p_{\st i}$ generates queries the same way they do in DQ-OT. 

Given the final query pair and $r_{\st 3}$,  \se first appends $r_{\st 3}$ to $m_{\st 0}$ and $m_{\st 1}$ and then computes the response the same way it does in DQ-OT, with the difference that it also randomly permutes the elements of the response pair.  Given the response pair and $r_{\st 3}$, \re decrypts each element in the pair and accepts the result that contains $r_{\st 3}$. 
%
Figure \ref{fig::DQ-OT-with-unknown-query} presents DUQ-OT in more detail. 
%%%%%%%%%%%%


\begin{figure}[!htbp]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=86mm, left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\begin{enumerate}[leftmargin=5.2mm]
%

\item \underline{\textit{$\se$-side Initialization:}} 
%
$\mathtt{Init}(1^{\st \lambda})\rightarrow pk$
%
\begin{enumerate}

\item chooses a sufficiently large prime number $p$.

\item selects random element
$C \stackrel{\st \$}\leftarrow \mathbb{Z}_p$ and generator $g$.
\item publish $pk=(C, p, g)$. 

\end{enumerate}




\item \underline{\textit{\re-side Delegation:}} $\mathtt{\re.Request}( pk)\hspace{-.6mm}\rightarrow\hspace{-.6mm} req=(req_{\st 1}, req_{\st 2})$
%
\begin{enumerate}


\item pick two uniformly random values: 
%
$r_{\st 1}, r_{\st 2} \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.

\item send $req_{\st 1}= r_{\st 1}$ to $\p_{\st 1}$ and $req_{\st 2}=r_{\st 2}$ to $\p_{\st 2}$.

\end{enumerate}

\item \underline{\textit{$\tp$-side Query Generation:}}
%
$\mathtt{\tp.Request}(1^{\st \lambda}, s, pk)\hspace{-.7mm}\rightarrow\hspace{-.7mm} (req'_{\st 1}, req'_{\st 2}, sp_{\st \se})$

\begin{enumerate}

\item split  the private index $s$ into two shares $(s_{\st 1}, s_{\st 2})$ by calling  $\ses(1^{\st\lambda}, s, 2, 2)\rightarrow (s_{\st 1}, s_{\st 2})$.

\item pick a uniformly random value: $r_{\st 3} \stackrel{\st\$}\leftarrow\{0,1\}^{\st\lambda}$.

\item send $req'_{\st 1} =s_{\st 1}$ to  $\p_{\st 1}$, $req'_{\st 2}=s_{\st 2}$ to  $\p_{\st 2}$. It also sends secret parameter $sp_{\st \se}=r_{\st 3}$ to \se and $sp_{\st \re} = (req'_{\st 2}, sp_{\st \se})$ to \re. 


\end{enumerate}

\item \underline{\textit{$\p_{\st 2}$-side Query Generation:}}
%
$\mathtt{\p_{\st 2}.GenQuery}(req_{\st 2}, req'_{\st 2}, pk)\rightarrow q_{\st 2}$
%

\begin{enumerate}

\item compute a pair of partial queries:
%
  $$\delta_{\st s_2}= g^{\st r_2},\ \  \delta_{\st 1-s_2} = \frac{C}{g^{\st r_2}}$$
  
\item send $q_{\st 2}=(\delta_{\st 0}, \delta_{\st 1})$ to  $\p_{\st 1}$. 

\end{enumerate}

\item\underline{\textit{$\p_{\st 1}$-side Query Generation:}}
%
$\mathtt{\p_{\st 1}.GenQuery}(req_{\st 1},req'_{\st 1}, q_{\st 2},pk)\rightarrow q_{\st 1}$

\begin{enumerate}

\item compute a pair of final queries as: 
%
$$\beta_{\st s_1}=\delta_{\st 0}\cdot g^{\st r_1},\ \ \beta_{\st 1-s_1}=\frac{\delta_{\st 1}} {g^{\st r_1}}$$

\item send $q_{\st 1} =(\beta_{\st 0}, \beta_{\st 1})$ to  $\se$.

\end{enumerate}

\item\underline{\textit{\se-side Response Generation:}} 
%
$\mathtt{GenRes}(m_{\st 0}, m_{\st 1}, pk, q_{\st 1}, sp_{\st \se})\rightarrow res$
%
%

\begin{enumerate}

\item abort if  $C \neq \beta_{\st 0}\cdot \beta_{\st 1}$.
    %
\item pick two uniformly random values: 
%
$y_{\st 0}, y_{\st 1}  \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p}$.
    
\item compute a response pair $(e_{\st 0}, e_{\st 1})$ as follows:
%
$$e_{\st 0} := (e_{\st 0,0}, e_{\st 0,1}) = (g^{\st y_0}, \g(\beta_{\st 0}^{\st y_0}) \oplus (m_{\st 0}||r_{\st 3}))$$
    %
$$e_{\st 1} := (e_{\st 1,0}, e_{\st 1,1}) = (g^{\st y_1}, \g(\beta_{\st 1}^{\st y_1}) \oplus (m_{\st 1}||r_{\st 3}))$$


\item randomly permute the elements of the pair $(e_{\st 0}, e_{\st 1})$ as follows: $\pi(e_{\st 0}, e_{\st 1})\rightarrow ({e}'_{\st 0}, {e}'_{\st 1})$.

 
\item send $res=(e'_{\st 0}, e'_{\st 1})$ to \re. 

\end{enumerate}

\item\underline{\textit{\re-side Message Extraction:}} 
%
$\mathtt{Retreive}(res, req, pk, sp_{\st \re})\hspace{-.6mm}\rightarrow\hspace{-.8mm} m_{\st s}$
%

\begin{enumerate}

\item set $x=r_{\st 2}+r_{\st 1}\cdot(-1)^{\st s_2}$. 

\item retrieve message $m_{\st s}$ as follows. 
%
 $\forall i, 0\leq i\leq1:$

\begin{enumerate}

\item set $y=\g(({e}'_{\st i, 0})^{\st x})\oplus {e}'_{\st i, 1}$.


\item  call $\parse(\gamma, y)\rightarrow (\ux, \uy)$.


\item set  $m_{\st s}=\ux$, if $\uy=r_{\st 3}$.


\end{enumerate}

\end{enumerate}

\end{enumerate}
%%%%%%%%%%%%%%%
\end{tcolorbox}
\end{center}
\vspace{-2.5mm}
    \caption{DUQ-OT: Our $1$-out-of-$2$ OT that supports query delegation while preserving the privacy of query from \re. In the protocol, $g$ is a generator, $C=g^{\st a}$ is a random public value, $\ses(.)$ is the share-generation algorithm (of a secret sharing), $\g(.)$ is a hash function, $\pi(.)$ is a random permutation, and $\$$ denotes picking a value uniformly at random.  
    }
    \label{fig::DQ-OT-with-unknown-query}
    \vspace{-3mm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{theo::DUQ-OT-sec}
%
Let $\mathcal{F}_{\scriptscriptstyle\duqot}$ be the functionality defined in Section \ref{sec::DUQ-OT-definition}. If  
DL, CDH, and RO assumptions hold and random permutation $\pi(.)$  is secure, then DUQ-OT (presented in Figure \ref{fig::DQ-OT-with-unknown-query}) securely computes $\mathcal{F}_{\scriptscriptstyle\duqot}$ in the presence of semi-honest adversaries, 
%
% (a) semi-honest receiver \re, honest  \se,  \tp, $\p_{\st 1}$, and $\p_{\st 2}$, (b) semi-honest \tp and  honest \re \se, $\p_{\st 1}$, and $\p_{\st 2}$, (c) semi-honest \se, honest \tp, \re, $\p_{\st 1}$, and $\p_{\st 2}$, or (d) semi-honest $\p_{\st i}$ (where $i\in \{1, 2\}$), honest \se, \tp, and \re, 
%
w.r.t. Definition \ref{def::DUQ-OT-sec-def}. 

\end{theorem}



We refer readers to Appendix \ref{sec::DUQ-OT-Security-Proof} for the proof of Theorem \ref{theo::DUQ-OT-sec}. 

%
%%%%%%%%%%%%% Old version %%%%%%%%%%%%%%%%
%\begin{figure*}[!htp]
%%\begin{center}
%    \begin{tcolorbox}[enhanced,width=6.8in, height=148mm, left=1mm,top=1mm,
%    drop fuzzy shadow southwest,
%    colframe=black,colback=white]
%%
% \procedure{}{%
%%
%\hspace{10mm}\underline{\textbf{  $\se$  }} \hsort \underline{\textbf{ $\p_1$ }} \hsort  \hspace{-6mm}\underline{\textbf{ $\p_2$ }}\hs \underline{\textbf{ \tp }} \hs\hspace{-16mm} \underline{\textbf{ $\re$ }} \\
%%
%\shs   \pcln  \hs \hs \hspace{49mm}  r_1, r_2 \stackrel{\$}\leftarrow\mathbb{Z}_{p-1}  \\
% %
% \shs  \pcln  \hs  \hspace{23mm} \xleftarrow{\makebox[7.7cm]{$r_2$}}\\
%%
%  \shs  \pcln  \hs \xleftarrow{\makebox[10cm]{$r_1$}}\\
% %
% \shs \pcln  \hs \hs \hspace{18mm} \ses(1^{\lambda}, s, 2, 2)\rightarrow (s_1, s_2) \\
%  %
%  \shs   \pcln  \hs \hs\hspace{18mm}  r_3 \stackrel{\$}\leftarrow\{0,1\}^{\gamma}  \\
%  %
%  \shs  \pcln  \hs \hs\hspace{24mm} \xrightarrow{\makebox[2.96cm]{$(s_2, r_3)$}}\\
% %
%  \shs  \pcln  \hs \hspace{23mm} \xleftarrow{\makebox[4.5cm]{$s_2$}}\\
% %
% \shs  \pcln  \hs  \xleftarrow{\makebox[6.8cm]{$s_1$}}\\
%   %
% \shs  \pcln  \hspace{6mm}  \xleftarrow{\makebox[10.7cm]{$r_3$}}\\
%  %
%\shs  \pcln   \hs \hsort\hspace{-12mm}   \delta_{s_2}= g^{r_2};\ \delta_{1-s_2} = \frac{C}{g^{r_2}} \\
%  %%
%%\shs  \pcln   \hs \hs \delta_{1-s_2} = \frac{C}{g^{r_2}}  \\
%  %
%\shs    \pcln   \hs \xleftarrow{\makebox[2.2cm]{$(\delta_0, \delta_1)$}} \\
%  %
%\shs  \pcln  \hsort \beta_{s_1}=\delta_{0}\cdot g^{r_1};\ \beta_{1-s_1}=\frac{\delta_{1}} {g^{r_1}}\\
%  %
%\shs    \pcln  \hspace{6mm}\xleftarrow{\makebox[3.35cm]{$(\beta_0, \beta_1)$}} \\
%    %
% \shs   \pcln \hspace{-1mm}  \text{abort if } C \neq \beta_0\cdot \beta_1 \\
%    %
% \shs   \pcln \hspace{-1mm}  y_0, y_1  \stackrel{\$}\leftarrow\mathbb{Z}_{p-1}\\
%    %
%\shs\pcln \hspace{-1mm}  e_0 := (e_{0,0}, e_{0,1}) = (g^{y_0}, \g(\beta_{0}^{y_0}) \oplus (m_0||r_3)) \\
%    %
%\shs\pcln \hspace{-1mm}  e_1 := (e_{1,0}, e_{1,1}) = (g^{y_1}, \g(\beta_{1}^{y_1}) \oplus (m_1||r_3)) \\
%%
%\shs\pcln \hspace{-1mm}  \pi(e_0, e_1)\rightarrow ({e}'_{0}, {e}'_{1}) \\
%    %  
%\shs  \pcln  \hspace{6mm}\xrightarrow{\makebox[14.32cm]{$({e}'_{0}, {e}'_{1})$}} \\
%%
%\shs \pcln \hs \hs\hspace{46mm} 
%x=r_2+r_1\cdot(-1)^{s_2}\\%
%\shs \pcln \hs \hs\hspace{46mm} \forall i, 0\leq i\leq1:
%\\
%%
%\shs\pcln  
%\hs \hs \hspace{49mm} y=\g(({e}'_{i, 0})^{x})\oplus {e}'_{i, 1}\\
%%
%\shs\pcln  
%\hs \hs \hspace{49mm} \parse(\gamma, y)\rightarrow (a, b)\\
%%
%\shs\pcln  
%\hs \hs \hspace{49mm} \text{if } b=r_3, \text{ set } m_s=a\\
%\shs\pcln \hs \hs \hspace{48mm} \text{ return } m_s
% }
%%}}
%\end{tcolorbox}
%%\end{center}
%    \caption{DUQ-OT: Our $1$-out-of-$2$ OT that supports query delegation while preserving the privacy of query from \re. In the protocol, $C=g^{a}$ is a random public value, $\ses(.)$ is the share-generation algorithm (of a secret sharing), $\g(.)$ is a hash function, $\pi(.)$ is a random permutation, and $\$$ denotes picking a value uniformly at random.  
%    }
%    \label{fig::DQ-OT-with-unknown-query-x}
%\end{figure*}
%%%%%%%%%%%%% Old version %%%%%%%%%%%%%%%%
%


%
%
%%
%\subsection{Alternative decryption}\label{sec:Alternative-decryption}
%In our alternative approach, in order to maintain the security,
%$P_2$ will encrypt the $\delta_i$ in a way only $P_1$ can decrypt
%these.
%
%We now reflect on Table~\ref{tab:analysis}.
%When considering $\beta_i$ in this table, and comparing the case
%$s_1=0$ with the case $s_1=1$, we see that the role of $r_1$ and $-r_1$
%interchanged. So, if $P_1$ provides $r_1$ to $D$ in the case $s_1=0$
%and $-r_1$ to $D$ in the other case, then $D$ can remove this $r_1$ from
%$\beta_i$ without being told the value of $s_1$. For all practical
%purposes $D$ then learned the $\delta$'s, but without knowing whether
%these were permuted or not. $D$ can then use these obtained $\delta$'s
%instead of $\beta_i$ when constructing $c_0$ and $c_1$.
%$R$ having received $r_1$ from $P_1$ can then decrypt and obtain
%one of the two plaintexts.
%
%
%\subsection{Security proof}
%The security proof is rather straightforward. %(Note that Bellare-Micali~\cite{bellare1989non} did not even bother giving one.) 
%%
%First of all it is trivial to see that due to the property of the one-time
%pad, as proven by Shannon~\cite{Shannon49}, $\beta_2$ is independent of $s_2$,
%and so $s_2$ is not leaked to $P_1$. (Note that choosing $-r_1$ is indistinguishable
%from $r_1$.)
%
%When wondering whether $P_1$ learn $s_1$, note that $P_1$ is in the same
%situation as $D$ in Bellare-Micali.
%
%
%\subsection{Generalizations}
%It is well known how to convert a 1-out-of-2 OT into a 1-out-of-$n$ OT (see~\cite{OT-Survey} for various variants of 1-out-of-$n$ OT).
%It is trivial to adapt our protocol to that setting. In the 1-out-of-$n$ OT
%the database has $n$ records/plaintexts, while the case we considered
%the database has only 2 records/plaintexts.
%
%Moreover, our distributed request can be generalized to some variants of Bellare-Micali,
%as can easily be verified. For more details see the final paper. 
%
%\subsection{Recipient without the knowledge of $s_i$}
%There are cases where the recipient/customer does/must not know the index $s_i$; for instance, when $P_1$ and $P_2$ need to make a decision based on whether the customer is a premium member, without telling the customer whether it is not a premium member that might annoy it.
%
%In this case, $s_i$ can be the output of a secure Muti-Party Computation or a third-party secret shares it and sends a share to $P_1$ and $P_2$.  
%




\vspace{-2mm}


\section{Delegated-Query Multi-Receiver Oblivious Transfers}\label{sec::Multi-Receiver-OT}


In this section, we present two new variants of \dqot; namely, (1) Delegated-Query Multi-Receiver OT (\dqothf) and\\ (2) Delegated-Unknown-Query Multi-Receiver OT (\duqothf). They are suitable for the \emph{multi-receiver} setting in which the sender maintains a (large) database containing $z$ pairs of messages $\bm m=[(m_{\st 0, 0},m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})]$. 

In this setting, each pair, say $v$-th pair $(m_{\st 0, v},$ $m_{\st 1, v})\in \bm m$ is related to  a receiver,  $\re_{\st j}$, where $0\leq v\leq z-1$. Both variants (in addition to offering the efficiency, \spc, and security guarantee of \dqot) ensure that (i) a receiver learns nothing about the total number of receivers/pairs (i.e., $z$) and (ii) the sender learns nothing about which receiver is sending the query, i.e., a message pair's index for which a query was generated.  In the remainder of this section, we discuss these new variants.  


%We call the multi-receiver OT variant(s), OT \textit{with hidden field}, for the following reason. In a non-private   database comprising of numerous records and several users, for each user, there is a field  associated with the record that specifies whether the user should be able to access it. This field itself should remain hidden from the user. 


%\subsection{Motivation}\label{sec:Delegated-Query-OT-w-HF}
%
%
%
%
%
%
%
%
%The adoption of cloud computing has been accelerating. The ``PwC’s 2023 Cloud Business Survey'' suggests that 78\% of executives participating in the survey have mentioned that their companies had adopted cloud in most or  all parts of the business \cite{PwC2023}. As a result, multiple (sensitive) databases belonging to independent individuals and organisations have been merged and hosted by a single cloud provider.  To enable their staff members to access the organisation's remote database in a privacy-preserving manner, each organisation might be tempted to use one of the following approaches.
%
%\begin{itemize}[leftmargin=4mm]
%
%\item  \underline{\textit{Using an existing single-receiver OT, e.g., in \cite{IshaiKNP03}}}. However, this approach suffers from information leakage. It allows the server to learn not only which organisation is accessing the data but potentially even which specific staff member is utilising a particular portion of the data. 
%
%\item \underline{\textit{Using an existing multi-receiver OT, e.g., in \cite{CamenischDN09}}}. Nevertheless, this will also come with a privacy cost. The existing multi-receiver OTs reveal the size of the entire database to each receiver. In this scenario, a receiver can learn the number of private records other companies have in the same database. This type of leakage is particularly significant, especially when coupled with specific auxiliary information. For instance, the recent cyber attack revealed that data belonging to British Airways, Boots, BBC, and Aer Lingus was kept by the same cloud  \cite{BBB-hack}. 
%
%\end{itemize}
%
%Hence, a fully-private multi-receiver OT is necessary to ensure user privacy in real-world cloud settings. 

\vspace{-2mm}
\subsection{Delegated-Query Multi-Receiver OT}\label{sec::DQ-OT-HF}
The first variant \dqothf considers the setting where server $\p_{\st 1}$ or $\p_{\st 2}$ knows a client's related pair's index in the sender's database. 


%%%%%%%%%%%%


 \subsubsection{Security Definition}\label{sec::DQOT-HF}

The functionality that \dqothf computes takes as input (i)  a vector of messages $\bm{m}=[(m_{\st 0, 0},m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})]$ from \se, (ii) an index $v$ of a pair in $\bm{m}$ from $\p_{\st 1}$, (iii)  empty string  \empt from $\p_{\st 2}$, and (iv) the index $s$ (where $s\in \{0, 1\}$) from \re. It outputs an empty string $\empt$ to  \se, $z$ to $\p_{\st 1}$, $\empt$ to $\p_{\st 2}$, and outputs to \re $s$-th message from $v$-th pair in the vector, i.e., $m_{\st s, v}$. Formally, we define the functionality as: 
%
 $\mathcal{F}_{\scriptscriptstyle\dqothf}:\big([(m_{\st 0, 0},m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})], v, \empt, s\big) \rightarrow (\empt, z, \empt, m_{\st s, v})$, where $v\in\{0,..., z-1\}$. Next, we present a formal definition of \dqothf, in Definition \ref{def::DQ-OT-HF-sec-def}.  


\begin{definition}[\dqothf]\label{def::DQ-OT-HF-sec-def} Let $\mathcal{F}_{\scriptscriptstyle\dqothf}$ be the functionality defined above. We say that protocol $\Gamma$ realizes $\mathcal{F}_{\scriptscriptstyle\dqothf}$ in the presence of passive adversary \se, \re, $\p_{\st 1}$, or $\p_{\st 2}$, if for  every non-uniform PPT adversary \adv
in the real model, there exists a non-uniform PPT simulator \simm  in
the ideal model, such that:
%
%{\small{
\begin{equation}\label{equ::sender-sim-DQ-OT-HF}
\Big\{\simm_{\st\se}\big(\bm{m}, \empt\big)\Big\}_{\st \bm{m}, v, s}\stackrel{c}{\equiv} \Big\{\view_{\st\se}^{\st \Gamma}\big(\bm{m}, v,  \empt, s\big) \Big\}_{\st \bm{m}, v, s}
\end{equation}
%
\begin{equation}\label{equ::server1-sim-DQ-OT-HF}
\Big\{\simm_{\st\p_1}(v, z)\Big\}_{\st \bm{m}, v, s}\stackrel{c}{\equiv} \Big\{\view_{\st\p_1}^{\st \Gamma}\big(\bm{m}, v,  \empt, s\big) \Big\}_{\st \bm{m}, v, s}
\end{equation}
%
\begin{equation}\label{equ::server2-sim-DQ-OT-HF}
\Big\{\simm_{\st\p_2}(\empt, \empt)\Big\}_{\st \bm{m}, v, s}\stackrel{c}{\equiv} \Big\{\view_{\st\p_2}^{ \st\Gamma}\big(\bm{m}, v,  \empt, s\big) \Big\}_{\st \bm{m}, v, s}
\end{equation}
%
\begin{equation}\label{equ::reciever-sim-DQ-OT-HF}
\begin{split}
\Big\{\simm_{\st\re}\Big(s, \mathcal{F}_{\scriptscriptstyle\dqothf}\big(\bm{m}, v,  \empt, s\big)\Big)\Big\}_{\st \bm{m}, v,  s}\stackrel{c}{\equiv} \\   \Big\{\view_{\st\re}^{ \st\Gamma}\big(\bm{m}, v,  \empt, s\big) \Big\}_{\st \bm{m}, v, s}
\end{split}
\end{equation}
%}}
where $\bm{m}=[(m_{\st 0, 0},m_{\st 1, 0}),..., (m_{\st 0, z-1}, m_{\st 1, z-1})]$.


%%
%%
\end{definition}

%%%%%%%%%%%%

\subsubsection{Strawman Approaches}\label{sec::OT-HFstrawman-aprroach}

One may consider using one of the following ideas in the multi-receiver setting: 

\begin{enumerate}%[leftmargin=5.2mm]
    \item \underline{\textit{Using an existing single-receiver OT, e.g., in \cite{IshaiKNP03}}}, employing one of the following approaches:

    \begin{itemize}
        \item \textit{Approach 1}: receiver $\re_{\st j}$ sends a standard OT query to \se which computes the response for all $z$ pairs of messages. Subsequently, \se sends $z$ pair of responses to receiver $\re_{\st j}$ which discards all pairs from the response except for $v$-th pair. $\re_{\st j}$ extracts its message $m_{\st v}$ from the selected pair, similar to a regular $1$-out-of-$2$ OT.  However, this approach results in the leakage of the entire database size to $\re_{\st j}$.

        \item \textit{Approach 2}: $\re_{\st j}$ sends a standard OT query to \se, along with the index $v$ of its record.  This can be perceived as if \se holds a single record/pair. Accordingly, \se generates a response in the same manner as it does in regular $1$-out-of-$2$ OT. Nevertheless, Approach 2 leaks to $\se$ the index $v$ of the record that $\re_{\st j}$ is interested.
    \end{itemize}
    \item \underline{\textit{Using an existing multi-receiver OT, e.g., in \cite{CamenischDN09}}}. This will also come with a privacy cost. The existing multi-receiver OTs reveal the entire database's size to each receiver (as discussed in Section \ref{sec::multi-rec-ot}). In this scenario, a receiver can learn the number of private records other companies have in the same database. This type of leakage is particularly significant, especially when coupled with specific auxiliary information. 
\end{enumerate}
 Hence, a fully private multi-receiver OT is necessary to ensure user privacy in real-world cloud settings. 

 



\subsubsection{Protocol}\label{sec::rdqothf}
%
We present \rdqothf that realizes \dqothf. We build \rdqothf upon DQ-OT (presented in Figure \ref{fig::DQ-OT}). \rdqothf relies on our observation that in DQ-OT, given the response of \se, $\p_{\st 1}$ cannot learn anything, e.g., about the plaintext messages $m_{\st i}$ of  \se. Below, we formally state it.


\begin{lemma}\label{lemma::two-pairs-indis-}
Let $g$ be a generator of a group $\mathbb{G}$ (defined in Section \ref{sec::dh-assumption}) whose order is a prime number $p$ and $\log_{\st 2}(p)=\lambda$ is a security parameter. Also, let $(r_{\st 1}, r_{\st 2}, y_{\st 1}, y_{\st 2})$ be elements of $\mathbb{G}$ picked uniformly at random, $C=g^{\st a}$ be a random public value whose discrete logarithm is unknown, $(m_{\st 0}, m_{\st 1})$ be two arbitrary messages, and $\h$ be a hash function modelled as a RO (as defined in Section \ref{sec::notations}), where its output size is $\delta$-bit.  Let $\gamma=\stackrel{\st+}-r_{\st 1} \stackrel{\st+}-r_{\st 2}$, $\beta_{\st 0}=g^{\st a+\gamma}$, and $\beta_{\st 1}=g^{\st a-\gamma}$.  If DL, RO, and CDH assumptions hold, then given $r_{\st 1}, C, g^{\st r_2}$, and $\frac{C}{g^{\st r_2}}$, a PPT distinguisher cannot distinguish (i) $g^{\st y_0}$ and $g^{\st y_1}$ form  random elements of $\mathbb{G}$ and (ii) $ \h(\beta_{\st 0}^{\st y_0}) \oplus m_{\st 0}$ and $ \h(\beta_{\st 1}^{\st y_1}) \oplus m_{\st 1}$  from random elements from $\{0, 1\}^{\st\sigma}$, except for a negligible probability  $\mu(\lambda)$.



% the first elements of pairs $(g^{\st y_0}, \h(\beta_{\st 0}^{\st y_0}) \oplus m_{\st 0})$ and $(g^{\st y_1}, \h(\beta_{\st 1}^{\st y_1}) \oplus m_{\st 1})$  from random elements of $\mathbb{G}$, except for a negligible probability, $\mu(\lambda)$ and the second elements of the pairs from 

% from random elements of 



\end{lemma}

Appendix \ref{sec::proof-of-thorem} presents the proof of Lemma \ref{lemma::two-pairs-indis-}. 
%
The main idea behind the design of \rdqothf is as follows. Given a message pair from $\p_{\st 1}$,  \se needs to compute the response for all of the receivers and sends the result to  $\p_{\st 1}$, which picks and sends only one pair in the response to the specific receiver who sent the query and discards the rest of the pairs it received from \se. Therefore, \re receives a single pair (so it cannot learn the total number of receivers or the database size), and the server cannot know which receiver sent the query as it generates the response for all of them. As we will prove, $\p_{\st 1}$ itself cannot learn the actual query of \re, too. 



Consider the case where one of the receivers, say  $\re_{\st j}$, wants to send a query. In this case, within \rdqothf, messages $(s_{\st 1}, r_{\st 1})$, $(s_{\st 2}, r_{\st 2})$ and $(\beta_{\st 0}, \beta_{\st 1})$ are generated the same way as they are computed in DQ-OT.  However, given $(\beta_{\st 0}, \beta_{\st 1})$, \se generates $z$ pairs and sends them to $\p_{\st 1}$ who forwards only $v$-th pair to $\re_{\st j}$ and discards the rest.  Given the pair, $\re_{\st j}$ computes the result the same way a receiver does in DQ-OT. Figure \ref{fig::DQHT-OT} in Appendix \ref{sec::DQ-HF-OT-detailed-protocol} presents \rdqothf in detail. 



\vspace{-2mm}


\subsection{Delegated-Unknown-Query Multi-Receiver OT}\label{sec::Delegated-Unknown-Query-OT-HF}


The second variant    \duqothf can be considered as a variant of  \duqot. It is suitable for the setting where servers $\p_{\st 1}$ and $\p_{\st 2}$ do not (and must not) know a client's related index in the sender's database (as well as the index $s$ of the message that the client is interested in).% and only an external party, say \tp, knows the index. 





\subsubsection{Security Definition}\label{sec::DUQOT-HD-def}

The functionality that \duqothf computes takes as input (i)  a vector of messages $\bm{m}=[(m_{\st 0, 0},m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})]$ from \se, (ii) an index $v$ of a pair in $\bm{m}$ from $\tp$, (iii) the index $s$ of a message in a pair (where $s\in \{0, 1\}$) from \tp, (iv) the total number $z$ of message pairs from $\tp$, (v)  empty string  \empt from $\p_{\st 1}$, (vi)   \empt from $\p_{\st 2}$, and (vii)  \empt from $\re$. It outputs an empty string $\empt$ to  \se and $\tp$, $z$ to $\p_{\st 1}$, $\empt$ to $\p_{\st 2}$, and outputs to \re $s$-th message from $v$-th pair in $\bm{m}$, i.e., $m_{\st s, v}$. Formally, we define the functionality as: $\mathcal{F}_{\scriptscriptstyle\duqothf}:\big([(m_{\st 0, 0},m_{\st 1, 0}),...,$ $ (m_{\st 0, z-1},$ $m_{\st 1, z-1})], (v, s, z), \empt, \empt, \empt\big) \rightarrow ( \empt, \empt, z, \empt, m_{\st s, v})$, where $v\in\{0,..., z-1\}$. Next, we present a formal definition of \duqothf. 


\vspace{-2mm}

\begin{definition}[\duqothf]\label{def::DUQ-OT-HF-sec-def} Let $\mathcal{F}_{\scriptscriptstyle\duqothf}$ be the functionality defined above. We assert that protocol $\Gamma$ realizes $\mathcal{F}_{\scriptscriptstyle\duqothf}$ in the presence of passive adversary \se, \re, \tp, $\p_{\st 1}$, or $\p_{\st 2}$, if for  every non-uniform PPT adversary \adv
in the real model, there exists a non-uniform PPT simulator \simm  in
the ideal model, such that:
%
\begin{equation}\label{equ::DUQ-OT-HF-sender-sim-}
\begin{split}
\Big\{\simm_{\st\se}\big(\bm{m}, \empt\big)\Big\}_{\st \bm{m}, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\se}^{\st \Gamma}\big(\bm{m}, (v, s, z), \empt,  \empt, \empt \big) \Big\}_{\st \bm{m}, s}
\end{split}
\end{equation}

\vspace{-2mm}

\begin{equation}\label{equ::DUQ-OT-HF-server-sim-}
\begin{split}
\Big\{\simm_{\st\p_i}(\empt, out_{\st i})\Big\}_{\st \bm{m}, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\p_i}^{ \st\Gamma}\big(\bm{m}, (v, s, z), \empt,  \empt, \empt \big) \Big\}_{\st \bm{m}, s}
\end{split}
\end{equation}

\begin{equation}\label{equ::DUQ-OT-HF-t-sim-}
\begin{split}
\Big\{\simm_{\st\tp}\big((v, s, z), \empt\big)\Big\}_{\st \bm{m}, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\tp}^{ \st\Gamma}\big(\bm{m}, (v, s, z), \empt,  \empt, \empt \big) \Big\}_{\st \bm{m}, s}
\end{split}
\end{equation}

\begin{equation}\label{equ::DUQ-OT-HF-reciever-sim-}
\begin{split}
\Big\{\simm_{\st\re}\Big(\empt, \mathcal{F}_{\scriptscriptstyle\duqothf}\big(\bm{m}, (v, s, z), \empt,  \empt, \empt \big)\big)\Big)\Big\}_{\st \bm{m}, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\re}^{ \st\Gamma}\big(\bm{m}, (v, s, z), \empt,  \empt, \empt \big) \Big\}_{\st \bm{m}, s}
\end{split}
\end{equation}
%}}
where $\bm{m}=[(m_{\st 0, 0},m_{\st 1, 0}),..., (m_{\st 0, z-1}, m_{\st 1, z-1})]$, $out_{\st 1}=z$, $out_{\st 2}=\empt$, and $\forall i$,  $i\in \{1,2\}$. 
%
\end{definition}


\subsubsection{Protocol}\label{sec::DUQ-OT-HF} We proceed to present \rduqothf that realizes \duqothf. We build \rdqothf upon protocol DUQ-OT (presented in Figure \ref{fig::DQ-OT-with-unknown-query}). \rduqothf mainly relies on Lemma \ref{lemma::two-pairs-indis-} and the following technique. 


%To securely fetch $v$-th element $m_v$ from a database of the form   
%$A=
%\begin{bmatrix}
%m_0\\
%m_1\\
%...\\
%m_z\\
%\end{bmatrix}
%$ with a constant size response, it would suffice for to: (1) construct a vector $B=[b_1,...,b_z]$, where all $b_i$ are set to zero except $b_v$ which is set to $1$, (2) send $B$ to the database holder, and (2) compute $B\times A$ which results is $m_v$. 


To fetch a record $m_{\st v}$ ``securely'' from a semi-honest \se that holds a database of the form $\bm{a}=[m_{\st 0}, m_{\st 1}, ..., m_{\st z-1}]^{\st T}$ where $T$ denotes transpose, 
%
%$A=
%\begin{bmatrix}
%m_0\\
%m_1\\
%...\\
%m_z\\
%\end{bmatrix}
%$
% 
without revealing which plaintext record we want to fetch, we can perform as follows: 

\begin{enumerate}%[label=$\roman$]
\item construct vector $\bm{b}=[b_{\st 0},..., b_{\st z-1}]$, where all $b_{\st i}$s are set to zero except for $v$-th element $b_{\st v}$ which is set to $1$.

\item encrypt each element of $\bm{b}$ using additively homomorphic encryption, e.g., Paillier encryption. Let $\bm{b}'$ be the vector of the encrypted elements. 

 \item send $\bm{b}'$ to the database holder which performs $\bm{b}'\times \bm{a}$ homomorphically, and sends us the single result $res$.
 
 \item decrypt $res$ to discover $m_{\st v}$.\footnote{Such a technique was previously used by Devet \textit{et al.} \cite{DevetGH12} in the ``private information retrieval'' research line.} 
 \end{enumerate}
 
 
 
 In our \rduqothf,  $\bm{b}'$ is not sent for each query to  \se. Instead,  $\bm{b}'$ is stored once in one of the servers, for example, $\p_{\st 1}$. Any time \se computes a vector of responses, say $\bm{a}$, to an OT query, it sends $\bm{a}$ to  $\p_{\st 1}$ which computes $\bm{b}'\times \bm{a}$ homomorphically and sends the result to \re.  Subsequently, \re can decrypt it and find the message it was interested.   Thus, $\p_{\st 1}$ \emph{obliviously filters out} all other records of field elements that do not belong to $\re_j$ and sends to $\re_{\st j}$ only the messages that $\re_{\st j}$ is allowed to fetch. 
 %
 Figure  \ref{fig::DQ-OT-with-unknown-query-and-HF-first-sevene-phases}  presents \rduqothf in detail. 


\input{DUQ-MR-OT-Protocol}

%%%%%%%%% Start of 1st table %%%%%%%%%
%
% \begin{figure}[!htbp]
% \setlength{\fboxsep}{.9pt}
% \begin{center}
%     \begin{tcolorbox}[enhanced,width=86mm, height=113mm, left=0mm,
%     drop fuzzy shadow southwest,
%     colframe=black,colback=white]
% %%%%%%%%%%%%
% \vspace{-2.2mm}

% \begin{enumerate}[leftmargin=5.2mm]
% %
% \item\label{DUQOT-HT::gen-key} \underline{\textit{$\re_{\st j}$-side One-off Setup:}}
% %
% \begin{enumerate}

% \item generate a key pair for additive homomorphic encryption, by calling $\keygen(1^{\st\lambda})\rightarrow(sk, pk)$.

% \item send $pk$  to \tp and $\se$.

% \end{enumerate}



% \item \underline{\textit{\tp-side One-off Setup:}}

% \begin{enumerate}

% \item initialise an empty vector $\bm{w}_{\st j}=[]$ of size $z$.

% \item create a compressing vector, by setting $v$-th position of $\bm{w}_{\st j}$ to encrypted $1$ and setting the rest of $z-1$ positions to encrypted $0$. $ \forall t, 0\leq t\leq z-1:$
% %

% \begin{enumerate}

% \item  set  $d=1$, if $t=v$; set $d=0$, otherwise.

% \item  append $\enc(pk, d)$ to  $\bm{w}_{\st j}$.

% \end{enumerate}

% \item send $\bm{w}_{\st j}$ to $\p_{\st 1}$.

% \end{enumerate}

% \item \underline{\textit{$\re_{\st j}$-side Delegation:}}

% \begin{enumerate} 

% \item pick random values: $r_{\st 1}, r_{\st 2} \stackrel{\st\$}\leftarrow\mathbb{Z}_{\st p-1}$.

% \item send $r_{\st 1}$ to $\p_{\st 1}$ and $r_{\st 2}$ to $\p_{\st 2}$.

% \end{enumerate}

% \item \underline{\textit{$\tp$-side Query Generation:}}

% \begin{enumerate}

% \item split  the private index $s$ into two shares $(s_{\st 1}, s_{\st 2})$ by calling  $\ses(1^{\st \lambda}, s, 2, 2)\rightarrow (s_{\st 1}, s_{\st 2})$.

% \item pick a uniformly random value: $r_{\st 3} \stackrel{\st\$}\leftarrow\{0,1\}^{\st\lambda}$.

% \item send $(s_{\st 2}, r_{\st 3})$ to $\re_{\st j}$, $s_{\st 1}$ to  $\p_{\st 1}$, $s_{\st 2}$ to  $\p_{\st 2}$,  $r_{\st 3}$ to \se. 

% \end{enumerate}
% \item \underline{\textit{$\p_{\st 2}$-side Query Generation:}}

% \begin{enumerate}

% \item compute queries:
% %
%   $\delta_{\st s_2}= g^{\st r_2},\ \  \delta_{\st 1-s_2} = \frac{C}{g^{\st r_{\st 2}}}$.
%   %
% \item send $(\delta_{\st 0}, \delta_{\st 1})$ to  $\p_{\st 1}$. 

% \end{enumerate}

% \item\label{DUQOT-HT::gen-P1-side-q-gen}\underline{\textit{$\p_{\st 1}$-side Query Generation:}}

% \begin{enumerate}

% \item compute final queries as: 

% $\beta_{\st s_{\st 1}}=\delta_{\st 0}\cdot g^{\st r_1},\ \ \beta_{\st 1-s_1}=\frac{\delta_{\st 1}} {g^{\st r_1}}$. 

% \item send $(\beta_{\st 0}, \beta_{\st 1})$ to  $\se$.

% \end{enumerate}

% \end{enumerate}
% \vspace{-3mm}
% \end{tcolorbox}
% \end{center}
% \vspace{-5mm}
%     \caption{Phases \ref{DUQOT-HT::gen-key}--\ref{DUQOT-HT::gen-P1-side-q-gen} of \rduqothf.    
%     }
%     \label{fig::DQ-OT-with-unknown-query-and-HF-first-sevene-phases}
%     \vspace{-3mm}
% \end{figure}
% %%%%%%%%%%% end of 1st table%%%%%%%%%%%%%%



% %%%%%%%%%%%start of 2nd table%%%%%%%%%%%%%%
% \begin{figure}[!htbp]
% \setlength{\fboxsep}{.9pt}
% \begin{center}
%     \begin{tcolorbox}[enhanced,width=86mm, height=93mm, left=0mm,
%     drop fuzzy shadow southwest,
%     colframe=black,colback=white]
% %%%%%%%%%%%%
% \vspace{-2.4mm}

% \begin{enumerate}[leftmargin=5.2mm]
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \setcounter{enumi}{6}
% %XXXXXXXX


% \item\label{DUQOT-HT::gen-res}\underline{\textit{\se-side Response Generation:}} 

% \begin{enumerate}

% \item abort if  $C \neq \beta_{\st 0}\cdot \beta_{\st 1}$.

% \item compute a response as follows. $\forall t, 0\leq t \leq z-1:$
% %
% \begin{enumerate}[leftmargin=1.2mm]
% \item   pick two random values $y_{\st 0, t}, y_{\st 1, t}  \stackrel{\$}\leftarrow\mathbb{Z}_{\st p-1}$.
  
% \item  compute  response:

%  $ e_{\st 0, t} := (e_{\st 0, 0, t}, e_{\st 0, 1, t}) = (g^{\st y_{\st 0, t}}, \g(\beta_{\st 0}^{\st y_{0, t}}) \oplus (m_{\st 0, t}||r_{\st 3}))$
      
% $e_{\st 1, t} := (e_{\st 1, 0, t}, e_{\st 1, 1, t}) = (g^{\st y_{1, t}}, \g(\beta_{\st 1}^{\st y_{\st 1, t}}) \oplus (m_{\st 1, t}||r_{\st 3})) $ 
   
% \item   randomly permute the elements of each pair $(e_{\st 0, t}, e_{\st 1, t})$ as $\pi(e_{\st 0, t}, e_{\st 1, t})\rightarrow ({e}'_{\st 0, t}, {e}'_{\st 1, t})$.
   
% \end{enumerate}

% \item     send $(e'_{\st 0, 0}, e'_{\st 1, 0}),..., (e'_{\st 0, z-1}, e'_{\st 1, z-1}) \text{ to } \p_{\st 1}$.
% \end{enumerate}


% %XXXXXXXXXXXXXXX
% \item\label{DUQOT-HT::oblivius-filter}\underline{\textit{$\p_{\st 1}$-side Oblivious Filtering:}} 


% \begin{enumerate}

% \item compresses the \se's response using vector  $\bm{w}_{\st j}$ as follows. $\forall i,i', 0\leq i,i'\leq 1:$
    
% $o_{\st i, i'}= (e'_{\st i, i',0}\hmul \bm{w}_{\st j}[0])\hadd...\hadd  (e'_{\st i,i', z-1}\hmul \bm{w}_{\st j}[z-1])$
 
% \item  send $(o_{\st 0, 0}, o_{\st 0, 1}), (o_{\st 1, 0}, o_{\st 1, 1}) \text{ to } \re_{\st j}$

% \end{enumerate}



% \item\label{DUQOT-HT::message-ext}\underline{\textit{\re-side Message Extraction:}} 

% \begin{enumerate}


% \item decrypt the response from $\p_{\st 1}$ as follows: 

%  $\forall i,i', 0\leq i,i'\leq 1:$
% %
% $ \dec(sk, o_{\st i,i'})\rightarrow o'_{\st i,i'}$. 



% \item set $x=r_{\st 2}+r_{\st 1}\cdot(-1)^{\st s_2}$.

% \item retrieve message $m_{\st s, v}$ as follows. 
% %
%  $\forall i, 0\leq i\leq1:$

% \begin{enumerate}

% \item set $y=\g(({o}'_{\st i, 0})^{\st x})\oplus {o}'_{\st i, 1}$.

% \item call $\parse(\gamma, y)\rightarrow (a, b)$.

% \item  set $m_{\st s, v}=a$, if $b=r_{\st 3}$.

% \end{enumerate}

% \end{enumerate}

% \end{enumerate}
% %%%%%%%%%%%%%%%
% \end{tcolorbox}
% \end{center}
% \vspace{-5mm}
%     \caption{Phases \ref{DUQOT-HT::gen-res}--\ref{DUQOT-HT::message-ext} of \rduqothf.   
%     }
%     \label{fig::DQ-OT-with-unknown-query-and-HF}
% \end{figure}
% %%%%%%%%%%%%%%%end of 2nd table %%%%%%%%%%%%%%


In both \rdqothf and \rduqothf, \se sends to $\p_{\st 1}$ a number of messages linear with the database size.  

% future work (for us): we can make a tradeoff between security and  efficiency-- by using OT to hide only that there's a hidden field.  

% For these protocols to be practical, $\p_1$ needs to be in close proximity to \se. In fact, $\p_1$ can be a secure hardware/chipset, such as Intel SGX with very limited storage space, hosted by \se itself. In this case,  $\p_1$ can receive the messages sequentially (i.e., element by element) and perform computations on each element as it is received. 



\begin{theorem}\label{theo::DUQ-OTHF-2-sec}
%
Let $\mathcal{F}_{\scriptscriptstyle\duqothf}$ be the functionality defined in Section \ref{sec::DUQOT-HD-def}. If  
DL, CDH, and RO assumptions hold and additive homomorphic encryption satisfies IND-CPA, then \rduqothf (presented in Figure \ref{fig::DQ-OT-with-unknown-query-and-HF-first-sevene-phases}) securely computes $\mathcal{F}_{\scriptscriptstyle\duqothf}$ in the presence of semi-honest adversaries, 
%
% (a) semi-honest receiver \re, honest  \se, \tp,  $\p_{\st 1}$, and $\p_{\st 2}$, (b)  semi-honest \se, honest \re, \tp, $\p_{\st 1}$, and $\p_{\st 2}$, (c) semi-honest \tp and honest \se, $\p_{\st i}$, and \re, or (d) semi-honest $\p_i$ (where $i\in \{1, 2\}$), honest \se, \tp, and \re,
%
w.r.t. Definition \ref{def::DUQ-OT-HF-sec-def}. 
%
\end{theorem}
We refer readers to Appendix \ref{sec::proof-of-DUQ-OT-HF} for Theorem \ref{theo::DUQ-OTHF-2-sec}'s proof.

\vspace{-2mm}
\section{A Compiler for Generic OT with Constant Size Response}\label{sec::the-compiler}

In this section, we present a compiler that transforms  \emph{any} $1$-out-of-$n$ OT that requires \re to receive $n$ messages (as a response) into a $1$-out-of-$n$ OT that enables \re to receive only a \emph{constant} number of messages. 


 The main technique we rely on is the encrypted binary vector that we used in Section \ref{sec::Delegated-Unknown-Query-OT-HF}.  The high-level idea is as follows.  During query computation, \re (along with its vector that encodes its index $s\in\{0, n-1\}$) computes a binary vector of size $n$, where all elements of the vector are set to $0$ except for $s$-th element which is set to $1$. \re encrypts each element of the vector and sends the result as well as its query to \se. Subsequently, \se computes a response vector (the same manner it does in regular OT), homomorphically multiplies each element of the response by the element of the encrypted vector (component-wise), and then homomorphically sums all the products. It sends the result (which is now constant with regard to $n$) to \re. Next, \re decrypts the response and retrieves the result $m_{\st s}$. 
 
 In the remainder of this section, we will present a generic OT's syntax, and then introduce the generic compiler using this syntax. 
 
\vspace{-2mm}

\subsection{Syntax of a Conventional OT}\label{sec::OT-syntax}

\vspace{-1mm}

Since we would like to treat any  OT in a block-box manner, we first present the syntax of an OT. A conventional (or non-delegated) $1$-out-of-$n$ OT (\onenot) have the following algorithms: 


\begin{itemize}[leftmargin=4.5mm]



\item[$\bullet$] $\mathtt{\se.Init}(1^{\st\lambda})\rightarrow pk$: a probabilistic algorithm run by \se. It takes as input security parameter $1^{\st\lambda}$ and returns a public key $pk$. 

% =======\\

% \item[$\bullet$] $\mathtt{Setup}(1^{\st\lambda})\rightarrow (sk, pk)$: a probabilistic algorithm run by \re. It takes as input security parameter $1^{\st\lambda}$ and returns a pair of private and public keys $(sk, pk)$. 

% =====\\

\item[$\bullet$] $\mathtt{\re.GenQuery}(pk, n, s)\rightarrow (q, sp)$: a probabilistic algorithm run by \re. It takes as input $pk$, the total number of messages $n$, and a secret index $s$. It returns a query (vector) $q$ and a secret parameter $sp$.  

 \item[$\bullet$] $\mathtt{\se.GenRes}(m_{\st 0},\ldots,m_{\st n-1}, pk, q)\rightarrow res$: a probabilistic algorithm run by \se. It takes as input $pk$ and $q$. It generates an encoded response (vector) $res$. 
 
 
  \item[$\bullet$] $\mathtt{\re.Retreive}(res, q, sp, pk, s)\rightarrow m_{\st s}$: a deterministic algorithm run by \se. It takes as input $res$,  $q$, $sp$,  $pk$, and $s$. It returns message $m_{\st s}$. 
 
\end{itemize} 



% \begin{itemize}



% \item[$\bullet$] $\mathtt{Init}(1^{\st\lambda})\rightarrow pk$: a probabilistic algorithm run by \se. It takes as input security parameter $1^{\st\lambda}$ and returns a public key $pk$. 

% =======\\

% \item[$\bullet$] $\mathtt{Setup}(1^{\st\lambda})\rightarrow (sk, pk)$: a probabilistic algorithm run by \re. It takes as input security parameter $1^{\st\lambda}$ and returns a pair of private and public keys $(sk, pk)$. 

% =====\\

% \item[$\bullet$] $\mathtt{GenQuery}(sk,pk, s)\rightarrow q$: a probabilistic algorithm run by \re. It takes as input $sk$,  $pk$, and an index $s$. It returns a query (vector) $q$.  

%  \item[$\bullet$] $\mathtt{GenRes}(pk, q)\rightarrow res$: a probabilistic algorithm run by \se. It takes as input $pk$ and $q$. It generates an encoded response (vector) $res$. 
 
 
%   \item[$\bullet$] $\mathtt{Retreive}(res, q, sk, pk, s)\rightarrow m_{\st s}$: a deterministic algorithm run by \se. It takes as input $res$,  $q$, $sk$,  $pk$, and $s$. It returns message $m_{\st s}$. 
 
% \end{itemize} 


The functionality that a $1$-out-of-$n$ OT  computes can be defined as: 
%
 $\mathcal{F}_{\scriptscriptstyle\onenot}:\big((m_{\st 0}, ..., m_{\st n-1}), s\big) \rightarrow (\empt, m_{\st s})$. Informally, the security of $1$-out-of-$n$ OT states that (1) \re's view can be simulated given its input query $s$ and output message $m_{\st s}$ and (2) \se's view can be simulated given its input messages $(m_{\st 0}, ..., m_{\st n-1})$. We refer readers to \cite{DBLP:books/cu/Goldreich2004} for further discussion on $1$-out-of-$n$ OT. 


\subsection{The Compiler}\label{sec::compiler}
We present the compiler in detail in Figure \ref{fig::generic-short-res-HE}.  We highlight that in the case where each $e_i \in res$ contains more than one value, e.g., $e_{\st i}=[e_{\st 0,i},..., e_{\st w-1,i}]$ (due to a certain protocol design), then each element of $e_i$ is separately multiplied and added by the element of vector $\bm{b}'$, e.g., the $j$-st element of the response is $e_{\st j, 0}\hmul \bm{b}'[0]\hadd...\hadd e_{\st j, n-1}\hmul \bm{b}'[n-1]$, for all $j$, $0\leq j\leq w-1$. In this case, only $w$ elements are sent to \re. 


%%%%%%%%%%%%%%
\begin{figure}[!htbp]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=81mm,  left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\vspace{-2mm}
\begin{enumerate}[leftmargin=5.2mm]
%
\item\underline{\textit{$\se$-side Initialization:}}
%
$\mathtt{Init}(1^{\st\lambda})\rightarrow pk$



This phase involves \se. 
\begin{enumerate}
    \item call $\mathtt{\se.Init}(1^{\st\lambda})\rightarrow pk$. 
    \item publish $pk$.
\end{enumerate}


\item\underline{\re-side Setup:} 
%
$\mathtt{Setup}(1^{\st\lambda})\rightarrow (sk_{\st \re}, pk_{\st \re})$ 

This phase involves \re. 
%
\begin{enumerate}
%
 \item call 
 $\keygen(1^{\st\lambda})\rightarrow(sk_{\st \re}, pk_{\st \re})$. 

% $\mathtt{Setup}(1^{\st\lambda})\rightarrow (sk, pk)$.
%
\item publish $pk_{\st \re}$.
 %
 \end{enumerate}
\item\underline{\re-side Query Generation:} 
%
$\mathtt{GenQuery}(pk_{\st \re}, n, s)\rightarrow (q, sp, \bm{b}')$

This phase involves \re. 
\begin{enumerate}
\item call $\mathtt{\re.GenQuery}(pk,n, s)\rightarrow (q, sp)$. 
%
\item construct a vector $\bm{b}=[b_{\st 0},...,b_{\st n-1}]$, as: 
%

\begin{enumerate}
%
\item set every element $b_{\st i}$ to zero except for $s$-th element $b_{\st s}$ which is set to $1$.
%
\item encrypt each element of $\bm{b}$ using additive homomorphic encryption, $\forall 0\leq i\leq n-1: b'_{\st i}=\enc(pk_{\st \re}, b_{\st i})$. 
%
Let $\bm{b}'$ be the vector of the encrypted elements. 
%
\end{enumerate}
%
 \item send $q$ and $\bm{b}'$ to \se and locally store $sp$. 
\end{enumerate}
\item\underline{\se-side Response Generation:}
%
$\mathtt{GenRes}(m_{\st 0},\ldots,m_{\st n-1}, pk, pk_{\st \re}, q, \bm{b}')\rightarrow res$

This phase involves \se. 
%
\begin{enumerate}
%
\item call $\mathtt{\se.GenRes}(m_{\st 0},\ldots,m_{\st n-1}, pk, q)\rightarrow res$. Let $res=[e_{\st 0},..., e_{\st n-1}]$. 
%
\item compress the response using vector  $\bm{b}'$ as follows. $\forall i, 0\leq i\leq n-1:$ 
    %  
    \vspace{-1.6mm}
$$e= (e_{0}\hmul \bm{b}'[0])\hadd...\hadd  (e_{\st n-1}\hmul \bm{b}'[n-1])$$
 
\item  send $res=e$  to \re.
%
\end{enumerate}

\item\underline{\re-side Message Extraction.} 
%
$\mathtt{Retreive}(res, q, sp, pk,sk_{\st \re}, s)\rightarrow m_{\st s}$



This phase involves \re. 

\begin{itemize}
%

\item call $\dec(sk_{\st \re}, res)\rightarrow res'$. 


\item[$\bullet$] call $\mathtt{\re.Retreive}(res', q, sp, pk, s)\rightarrow m_{\st s}$. 
%
\end{itemize}
\end{enumerate}
%%%%%%%%%%%%%%%
\end{tcolorbox}
\end{center}
\vspace{-4mm}
    \caption{A compiler that turns a $1$-out-of-$n$ OT with response size $O(n)$ to  a $1$-out-of-$n$ OT with response size $O(1)$.}
    \label{fig::generic-short-res-HE}
    \vspace{-4mm}
\end{figure}




\begin{theorem}\label{theo::one-out-of-n-OT}
%
Let $\mathcal{F}_{\scriptscriptstyle\onenot}$ be the functionality defined above. If  
\onenot is secure and additive homomorphic encryption satisfies IND-CPA property, then generic OT with constant size response (presented in Figure \ref{fig::generic-short-res-HE}) (i) securely computes $\mathcal{F}_{\scriptscriptstyle\onenot}$ in the presence of semi-honest receiver \re or semi-honest \se and (ii) offers $O(1)$ response size, w.r.t. the total number of messages $n$. 
%
\end{theorem}


Appendix \ref{theo::compiler-sec--} presents the proof of Theorem \ref{theo::one-out-of-n-OT}.


\vspace{-1mm}
\section{Supersonic OT}\label{sec::supersonice-OT}

%\vspace{-1mm}

%In this section, we propose a $1$-out-of-$2$ OT, called ``Supersonic OT'',  that (i) is highly fast as it does not require any public-key-based cryptography, (ii) has $O(1)$ size response that \re receives,  (iii) is information-theoretic secure; thus, it is post-quantum secure too, and (iv) it simple; so it is easy to analyse its security and to implement it.  


In this section, we introduce a $1$-out-of-$2$ OT, called ``Supersonic OT'',  which (i)
operates at high speed by eliminating the need for public-key-based cryptography, (ii) delivers a response of size $O(1)$ to the recipient, \re, (iii) ensures information-theoretic security, making it post-quantum secure, and (iv) is simple (but elegant), thus facilitating a simple analysis of its security and implementation.


\vspace{-1mm}
\subsection{Security Definition}\label{sec::Ultra-OT-definition}
%\vspace{-1mm}

Supersonic OT involves three types of entities, a sender \se, a receiver \re, and a server \p. We assume each party can be corrupted by a passive non-colluding adversary. The functionality $\mathcal{F}_{\scriptscriptstyle\ot}$ that Supersonic OT will compute is similar to that of conventional OT with the difference that now an additional party $\p$ is introduced, having no input and receiving no output. Thus, we define the functionality as   $\mathcal{F}_{\scriptscriptstyle\ot}:\big((m_{\st 0}, m_{\st 1}), \empt, s\big) \rightarrow (\empt, \empt, m_{\st s})$. 
%
 Next, we present a formal definition of \ot. 


\begin{definition}[\ot]\label{def::ultra-OT-sec-def} Let $\mathcal{F}_{\scriptscriptstyle\ot}$ be the   OT functionality defined above. We assert that protocol $\Gamma$ realizes $\mathcal{F}_{\scriptscriptstyle\ot}$ in the presence of passive adversary \se, \re, or $\p$, if for  every non-uniform PPT adversary \adv
in the real model, there is a non-uniform PPT  simulator \simm  in
the ideal model, where:
%
%{\small{
\begin{equation}\label{equ::ultra-ot-sender-sim-}
\begin{split}
\Big\{\simm_{\st\se}\big((m_{\st 0}, m_{\st 1}), \empt\big)\Big\}_{\st m_{0}, m_{1}, s}\stackrel{c}{\equiv}\\ \Big\{\view_{\st\se}^{ \st\Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,  s\big) \Big\}_{\st m_0, m_1, s}
\end{split}
\end{equation}

\begin{equation}\label{equ::ultra-ot-server-sim-}
\begin{split}
\Big\{\simm_{\st\p}(\empt, \empt)\Big\}_{\st m_0, m_1, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\p}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt, s\big) \Big\}_{\st m_0, m_1, s}
\end{split}
\end{equation}

\begin{equation}\label{equ::ultra-ot-reciever-sim-}
\begin{split}
\Big\{\simm_{\st\re}\Big(s, \mathcal{F}_{\scriptscriptstyle\ot}\big((m_{\st 0}, m_{\st 1}), \empt,  s\big)\Big)\Big\}_{\st m_0, m_1, s}\stackrel{c}{\equiv}\\  \Big\{\view_{\st\re}^{\st \Gamma}\big((m_{\st 0}, m_{\st 1}), \empt,   s\big) \Big\}_{\st m_0, m_1, s}
\end{split}
\end{equation}
%}}



%%
%%
\end{definition}



 


\vspace{-2mm}
\subsection{The Protocol}
\vspace{-.4mm}


At a high level, the protocol works as follows. Initially, \re and \se agree on a pair of keys. In the query generation phase, \re splits its private index into two binary shares. It sends one share to \se and the other to \p. Given the share/query, \se encrypts every message $m_{\st i}$ (using a one-time pad) under one of the keys it agreed with \re.  

Then, \se permutes the encrypted messages using  $\cper$ and its share. It sends the resulting pair to \p which permutes the received pair using  $\cper$ and its share. \p sends only the first element of the resulting pair (which is a ciphertext) to \re and discards the second element of the pair. Next, \re decrypts the ciphertext and learns the message it was interested in. Figure \ref{fig::Ultrasonic-OT} presents Supersonic OT in detail. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-1mm}
\begin{figure}[!h]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=85mm, height=89mm, left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%%%%%
\vspace{-2mm}
\begin{enumerate}[leftmargin=5mm]

\item \underline{\textit{\re-side Setup:}}
%
$\mathtt{Setup}(1^{\st\lambda})\rightarrow (k_{\st 0}, k_{\st 1})$ 

\begin{itemize}

%\item  \re and \se jointly run a coin tossing protocol to agree on two random keys $(k_0, k_1) \in\{0, 1\}^{\sigma}$. 

\item  \re picks two random keys $(k_{\st 0}, k_{\st 1}) \stackrel{\st\$}\leftarrow\{0, 1\}^{\st\sigma}$ and sends them to \se.

\end{itemize}

\item \underline{\textit{$\re$-side Query Generation:}} 
%
$\mathtt{GenQuery}(1^{\st \lambda}, s)\rightarrow q=(q_{\st 1}, q_{\st 2})$

\begin{enumerate}

\item split  the private index $s$ into two shares $(s_{\st 1}, s_{\st 2})$ by calling  $\ses(1^{\st \lambda}, s, 2, 2)\rightarrow (s_{\st 1}, s_{\st 2})$. 

\item send $q_{\st 1}=s_{\st 1}$ to \se and $q_{\st 2}=s_{\st 2}$ to $\p$. 

\end{enumerate}

\item \underline{\textit{$\se$-side Response Generation:}} 
%
$\mathtt{GenRes}(m_{\st 0}, m_{\st 1}, k_{\st 1},k_{\st 2}, q_{\st 1})\rightarrow res$

\begin{enumerate}

\item encrypt each message as follows. 
%
\vspace{-2mm}
$$\forall i, 0\leq i\leq 1: m'_{\st i}=m_{\st i}\oplus k_{\st i}$$


Let $e=(m'_{\st 0}, m'_{\st 1})$ contain the encrypted messages. 

\item permute the elements of $e$ as follows: $\cper(s_{\st 1}, e)\rightarrow e'$.

\item send $res=e'$ to $\p$. 

\end{enumerate}

\item \underline{\textit{$\p$-side Oblivious Filtering:}} 
%
$\mathtt{OblFilter}(res, q_{\st 2})\rightarrow res'$

\begin{enumerate}

\item permute the elements of $e'$ as: $\cper(s_{\st 2}, e')\rightarrow e''$.

\item\label{ultra-ot::e-double-prime} send (always) the first element in $e''$, say $res'=e''_{\st 0}$, to \re and discard the second element in $e''$. 

\end{enumerate}

\item\underline{\textit{\re-side Message Extraction:}} 
%
$\mathtt{Retreive}(res',  k_{\st s})\rightarrow m_{\st s}$

\begin{itemize}
\item retrieve the final related message $m_{\st s}$ by decrypting $e''_{\st 0}$ as: $m_{\st s}=e''_{\st 0}\oplus k_{\st s}$.
\end{itemize}

\end{enumerate}
%%%%%%%%%%%%%%%
\end{tcolorbox}
\end{center}
\vspace{-5.3mm}
\caption{Supersonic OT.} 
\vspace{-1mm}
\label{fig::Ultrasonic-OT}
\end{figure}

% At a high level, the protocol works as follows. Initially, \re and \se agree on a pair of keys. In the query generation phase, \re splits its private index into two binary shares. It sends one share to \se and the other to \p. Given the share/query, \se encrypts every message $m_{\st i}$ (using a one-time pad) under one of the keys it initially agreed with \re.  Then, \se permutes the encrypted messages using  $\cper$ and its share. It sends the resulting pair to \p. Accordingly, \p permutes the received pair using  $\cper$ and its share. \p sends only the first element of the resulting pair (which is a ciphertext) to \re and discards the second element of the pair. Subsequently, \re decrypts the ciphertext and learns the message it was interested in. 


%Figure \ref{fig::Ultrasonic-OT} presents the protocol in detail. 



\begin{theorem}\label{theo::ultra-OT}
%
Let $\mathcal{F}_{\scriptscriptstyle\ot}$ be the functionality defined in Section \ref{sec::Ultra-OT-definition}.  Then, Supersonic OT (presented in Figure \ref{fig::Ultrasonic-OT}) securely computes $\mathcal{F}_{\scriptscriptstyle\ot}$ in the presence of semi-honest adversaries, 
%
% (a) semi-honest receiver \re, honest  \se, and \p, (b)  semi-honest \se, honest \re and \p, or (c) semi-honest \p and honest \se and \re, 
%
w.r.t. Definition \ref{def::ultra-OT-sec-def}. 
%
\end{theorem}

\vspace{-1mm}
We refer readers to Appendix \ref{sec::ultrasonic-ot-proof} for proof of Theorem \ref{theo::ultra-OT}. 









\vspace{-2mm}
\subsection{Proof of Correctness}\label{sec::Ultra-OT-Proof-of-Correctness}

%\vspace{-1mm}

In this section, we demonstrate that \re always receives the message $m_{\st s}$ corresponding to its query $s$. To accomplish this, we will show that (in step \ref{ultra-ot::e-double-prime}) the first element of pair $e''$ always equals the encryption of $m_s$. This outcome is guaranteed by the following two facts: (a) $s=s_{\st 1}\oplus s_{\st 2}$ and (b)  \se and \tp permute their pairs based on the value of their share, i.e., $s_{\st 1}$ and $s_{\st 2}$ respectively. 

%%%%%

\begin{table}[!htb]
\vspace{-3mm}
\begin{center}
\scalebox{.8}{
  \begin{tabular}{|c|c|c|c|c|}   
\hline
    $s$&$s_{\st 1}$&$s_{\st 2}$\\   
\hline

\hline
&\cellcolor{gray!20}1&\cellcolor{gray!20} 1\\

\cline{2-3}

\multirow{-2}{*}{$0$}&\cellcolor{gray!20}0&\cellcolor{gray!20}0\\

\hline

&\cellcolor{gray!20}1&\cellcolor{gray!20}0\\

\cline{2-3}

\multirow{-2}{*}{$1$}&\cellcolor{gray!20}0&\cellcolor{gray!20}1\\

\hline

\end{tabular}
}
\end{center}
\caption{Relation between query $s$ and behaviour of permutation $\cper$ from the perspective of $\se$ and $\p$. When $s_{\st i}=1$, $\cper$ swaps the elements of its input pairs and when $s_{\st i}=0$, $\cper$ does not swap the elements of the input pairs.}
\label{tab:ultra-ot-correctness}
\vspace{-6mm}
\end{table}


%%%%%%



As Table \ref{tab:ultra-ot-correctness} indicates, when $s=0$, then (i) either both $\se$ and \p permute their pairs or (ii) neither does. In the former case, since both swap the elements of their pair, then the final permuted pair $e''$ will have the same order as the original pair $e$ (before it was permuted). In the latter case, again $e''$ will have the same order as the original pair $e$ because neither party has permuted it. Thus, in both of the above cases (when $s=0$), the first element of $e''$ will be the encryption of $m_{\st 0}$. 
%
Moreover, as Table \ref{tab:ultra-ot-correctness} indicates, when $s=1$, then only one of the parties \se and \p will permute their input pair. This means that the first element of the final permuted pair $e''$  will always equal the encryption of $m_{\st 1}$. 
%

\vspace{-2mm}
\subsection{Evaluation}\label{sec::supersonic-OT}

We have implemented Supersonic OT in C++ and evaluated its concrete runtime. The source code for the implementation is publicly available in \cite{supersonic-code}. For the experiment, we utilized a MacBook Pro laptop equipped with a quad-core Intel Core i5, 2 GHz CPU, and 16 GB RAM. Given the low number and small size of exchanged messages in our protocol, implementing it in a network setting will yield negligible network overhead.  
%
Despite our protocol being highly parallelizable, we did not leverage parallelization or any other optimization. The experiment was run an average of 50 times. The implementation utilizes GMP library\footnote{
https://gmplib.org} for big-integer arithmetic. 


We analyzed the runtime of various phases of Supersonic OT across different invocation frequencies ($1, 10, 10^{\st 3}, 10^{\st 5}$, and $10^{\st 7}$ times). Table \ref{fig::supersonic-cost-breakdown-by-phases} shows the high-speed performance of Supersonic OT, requiring only $0.35$ milliseconds for a single invocation. Notably, Phase 1 incurs the highest computation cost when the number of invocations is $1, 10$, and $10^{\st 3}$, while Phase 3 imposes the highest computation cost when the number of invocations is $10^{\st5}$ and $10^{\st7}$. Overall, Phase 2 has the lowest computation cost.





\input{Supersonic-OT-runtime-breakdown-by-phase}

\input{base-OTs-performance}






%\vspace{-4mm}
\subsubsection{Runtime}



% To date, the most efficient OTs belong to the class of OT extension, such as the ones described in \cite{IshaiKNP03,Efficient-OT-Naor,AsharovL0Z13}. 


\vspace{-1mm}
\noindent\underline{\textit{Supersonic Versus Base OTs.}} Initially, we compare the runtime of Supersonic OT with that of \textit{base} OTs proposed in \cite{AsharovL0Z13,Efficient-OT-Naor}. These base OTs, known for their generality, efficiency, and widespread usage in literature, serve as efficient foundations in OT extensions. 
%
Table \ref{fig::supersonic-vs-base-OTs} 
provides a summary of this comparison. The runtime data for OTs in \cite{AsharovL0Z13,Efficient-OT-Naor} is derived from the figures reported in \cite{AsharovL0Z13}, specifically from Table 3, where the GMP library was employed. \footnote{The implementation in \cite{AsharovL0Z13} used smaller RAM size (4-GB) compared to our usage of 16-GB. Their reported performance also accounts for LAN delay. However, it is important to note that doubling the RAM size doesn't necessarily equate to doubling the runtime. Moreover, the impact of LAN delay is negligible, particularly for our OT, which incurs a very low communication cost.}
%
Table \ref{fig::supersonic-vs-base-OTs} highlights that Supersonic OT demonstrates a speed advantage, being approximately $10^{\st 3}$ times faster than the OT in \cite{AsharovL0Z13} and up to around $2\times 10^{\st 3}$ times faster than the OT in \cite{Efficient-OT-Naor}.%\footnote{}

\input{OT-extension-performance}


Note that Supersonic OT maintains a consistent runtime across different security parameters, whether lower (e.g., 80-bit) or higher (e.g., 256-bit) than 128-bit. In contrast, the runtime of the schemes in \cite{AsharovL0Z13,Efficient-OT-Naor} would vary, fluctuating by at least a factor of 2.5 with changes in the security parameter.



\noindent\underline{\textit{Supersonic Versus OT Extensions.}} We proceed to compare the runtime of Supersonic OT with the runtime of efficient OT extensions presented in \cite{AsharovL0Z13,SchneiderZ13}. Given that OT extensions are designed for scenarios involving frequent executions, we evaluate the runtime of these three OTs when invoked $10^{\st 7}$ times. 
%
The runtime data for OTs in \cite{AsharovL0Z13,SchneiderZ13} is extracted from the figures reported in \cite{AsharovL0Z13}, specifically from Tables 3 and 4 in \cite{AsharovL0Z13}, where the GMP library was utilized.\footnote{Note that Table 4 in \cite{AsharovL0Z13} excludes the runtime of base OTs. Thus, the corresponding runtime of the base OT in Table 3 in \cite{AsharovL0Z13} must be added to each figure reported in Table 4. For instance, for G-OT (in LAN setting) we would have $13.92\times 1000+ 352=14,272$.} Table \ref{fig::supersonic-vs-extension-OTs} presents the outcome of this comparison. 

Table \ref{fig::supersonic-vs-extension-OTs} indicates that invoking  Supersonic OT $10^{\st 7}$ times takes approximately 6,610 milliseconds with a 128-bit security parameter. 
%
Supersonic OT outperforms the OT in \cite{AsharovL0Z13} by a factor of 2 and \cite{SchneiderZ13} by a factor of 3. Despite the higher 128-bit security parameter in Supersonic OT compared to the 80-bit parameter in the other two schemes, its runtime is still lower. We expect that increasing the security parameter in schemes in \cite{AsharovL0Z13,SchneiderZ13} would result in higher runtimes, given that the base OT's runtime increases accordingly.




 
%\vspace{-1mm}

\subsubsection{Features} 

For the base OTs and OT extensions in \cite{AsharovL0Z13,Efficient-OT-Naor,SchneiderZ13} to achieve unconditional security, as discussed in Section \ref{sec::uncon-sec-OT}, they typically require multiple replicas of the database, a noisy channel, or the involvement of a trusted initializer, all of which contribute to increased deployment costs. In contrast, Supersonic OT attains unconditional security without relying on database replications, noisy channels, or a fully trusted party. Although Supersonic OT involves an additional party, unlike base OTs or OT extensions that typically only involve the sender and receiver, it maintains its security even when this party is semi-honest.




\vspace{-1mm}
\section{Conclusion and Future Work}


OT is a crucial privacy-preserving technology.  OTs have found extensive applications in designing secure Multi-Party Computation (MPC) protocols \cite{Yao82b,AsharovL0Z13,HarnikIK07}, Federated (Machine) Learning (FL) \cite{YangLCT19,RenYC22,XuLZXND22}, and in accessing sensitive field elements of remote private databases while preserving privacy \cite{CamenischDN09,AielloIR01,libert2021adaptive}. In this work, we have identified various gaps both in the privacy of databases and in the OT research. We proposed several novel OTs to address these gaps. Specifically, we have proposed the following:

\begin{itemize}[leftmargin=4.5mm]
\item [i.]  Delegated-Query OT (and its variant), which enables the receiver to delegate query computation to potentially semi-honest parties while ensuring the privacy of the sender and receiver.

\item [ii.] Delegated-Query Multi-Receiver OT (and its variant), that ensures each receiver remains unaware of the total number of records and their field elements while preventing the sender from learning which query corresponds to which record.


\item[iii.]  a compiler that transforms any $1$-out-of-$n$ OT that requires the receiver to receive $n$ messages into a $1$-out-of-$n$ OT enabling a receiver to receive only a constant number of messages and have constant storage space.

\item[iv.] Supersonic OT, a $1$-out-of-$2$ OT that does not rely on database replications, noisy channels, or the involvement of a trusted initializer. It enables the receiver to receive a constant-size response and offers post-quantum security. We have implemented Supersonic OT and evaluated its overhead. Our evaluation exhibits that Supersonic OT is the fastest OT to date. 
\end{itemize}

We have presented several real-world applications of the proposed OTs, while also formally defining and proving their security within the simulation-based model. 


As a future research direction, exploring how the exceptional efficiency of Supersonic OT can enhance the performance of protocols (such as generic MPC or Private Set Intersection) that heavily rely on OTs would be intriguing. Furthermore, it would be interesting to generalize  Supersonic OT to support $1$-out-of-$n$ OT.

%As a future research direction, it would be interesting to see how the exceptional efficiency of Supersonic OT can improve the performance of those (generic MPC or Private Set Intersection) protocols that heavily rely on OT protocols. 


 




%In the cryptographic community, one of the main applications of OT is used in the context of secure multi-party computation. This paper was mainly inspired by several real-world database security problems. In particular, we focused on: (i) users who use an untrusted proxy to query a database to which they do not have direct access. 
%(i) databases with hidden fields/records, (ii) databases that were inappropriately merged 




%\section{Conclusions and Open Problems}
%We presented the first distributed request in OT. Note that the use of a distributed
%database in OT was addressed earlier~\cite{NaorP00}.
%
%There are several open problems which we now pose. First the distributed
%request is sequential. Can this be made parallel? Secondly,
%how to generalize this to a $t$-out-of-$n$ distributed request in which
%$t\neq n$?
%
%In this work, we have highlighted serious security/privacy issues in the
%banking sector. However, these issues have been overlooked by the
%information security and the cryptography research community so far. We hope this paper
%initiates future discussion and research to tackle such issues at their
%roots. 



%\begin{thebibliography}{10}
%
%%\bibitem{AbadiM22}
%%Abadi, A., Murdoch, S.~J.: Payment with dispute resolution: {A} protocol for
%%  reimbursing frauds' victims.
%%\newblock {IACR} Cryptol. ePrint Arch. (2022).
%
%%\bibitem{bellare1989non}
%%Bellare, M., Micali, S.:.
%%\newblock Non-interactive oblivious transfer and applications.
%%\newblock In Conference on the Theory and Application of Cryptology (1989)
%%  Springer.
%
%%\bibitem{Blakley-ACISP05}
%%Blakley, B., Blakley, G.~R.:.
%%\newblock All sail, no anchor {III:} risk aggregation and time's arrow.
%%\newblock In Information Security and Privacy, 10th Australasian Conference,
%%  {ACISP} 2005, Brisbane, Australia, July 4-6, 2005, Proceedings (2005)
%%  Springer.
%
%%\bibitem{Blakley79}
%%Blakley, G.~R.:.
%%\newblock Safeguarding cryptographic keys.
%%\newblock In Proc. Nat. Computer Conf. {AFIPS} Conf. Proc. (1979) pp.~313--317.
%
%%\bibitem{Chaum81}
%%Chaum, D.: Untraceable electronic mail, return addresses, and digital
%%  pseudonyms.
%%\newblock Commun. ACM {\bf 24} (1981) 84--88.
%
%%\bibitem{ChenHY04}
%%Chen, L., Huang, X., You, J.:.
%%\newblock Fair tracing without trustees for multiple banks.
%%\newblock In Computational and Information Science, First International
%%  Symposium, {CIS} 2004, Shanghai, China, December 16-18, 2004, Proceedings
%%  (2004).
%
%%\bibitem{ChouO15}
%%Chou, T., Orlandi, C.:.
%%\newblock The simplest protocol for oblivious transfer.
%%\newblock In Progress in Cryptology - {LATINCRYPT} 2015 - 4th International
%%  Conference on Cryptology and Information Security in Latin America,
%%  Guadalajara, Mexico, August 23-26, 2015, Proceedings (2015).
%
%\bibitem{darbha2020privacy}
%Darbha, S., Arora, R.:.
%\newblock Privacy in {CBDC} technology.
%\newblock Tech. rep. Bank of Canada 2020.
%
%\bibitem{bitcoin-hack-1}
%{Department of Justice}:.
%\newblock Two arrested for alleged conspiracy to launder \$4.5 billion in
%  stolen cryptocurrency 2022.
%\newblock
%  \url{https://www.justice.gov/opa/pr/two-arrested-alleged-conspiracy-launder-45-billion-stolen-cryptocurrency}.
%
%\bibitem{JPMorgan}
%{Department of Justice--U.S. Attorney's Office}:.
%\newblock Former {JP Morgan Chase Bank} employee sentenced to four years in
%  prison for selling customer account information 2018.
%\newblock
%  \url{https://www.justice.gov/usao-edny/pr/former-jp-morgan-chase-bank-employee-sentenced-four-years-prison-selling-customer}.
%
%\bibitem{Desjardins-settelment}
%{Desjardins Group}:.
%\newblock Privacy breach: Class action settlement {agreement} submitted to the
%  {Superior Court} of {Quebec} for approval 2022.\\
%\newblock
%  \url{https://www.desjardins.com/qc/en/news/desjardins-settlement-agreement.html}.
%
%\bibitem{egress-survey}
%egress:.
%\newblock Insider data breach survey 2021.\\
%\newblock
%  \url{https://www.egress.com/media/4kqhlafh/egress-insider-data-breach-survey-2021.pdf}.
%
%\bibitem{hegde2008secure}
%Hegde, C., Manu, S., Shenoy, P.~D., Venugopal, K., Patnaik, L.:.
%\newblock Secure authentication using image processing and visual cryptography
%  for banking applications.
%\newblock In 2008 16th International Conference on Advanced Computing and
%  Communications (2008) IEEE.
%
%\bibitem{bitcoin-hack-2}
%Hern, A.:.
%\newblock A history of bitcoin hacks 2014.\\
%\newblock
%  \url{https://www.theguardian.com/technology/2014/mar/18/history-of-bitcoin-hacks-alternative-currency}.
%
%\bibitem{IshaiKNP03}
%Ishai, Y., Kilian, J., Nissim, K., Petrank, E.:.
%\newblock Extending oblivious transfers efficiently.
%\newblock In Advances in Cryptology - {CRYPTO} 2003, 23rd Annual International
%  Cryptology Conference, Santa Barbara, California, USA, August 17-21, 2003,
%  Proceedings (2003) Springer.
%
%\bibitem{kenney2007regional}
%Kenney, S.: Regional shortcomings and global solutions: Kidnap, ransom and
%  insurance in {Latin America}.
%\newblock Conn. Ins. LJ {\bf 14} (2007) 557.
%
%\bibitem{Optus}
%Kurmelovs, R.:.
%\newblock Optus cyber-attack leaves customers feeling powerless over risk of
%  identity theft 2022.
%\newblock
%  \url{https://www.theguardian.com/australia-news/2022/sep/23/optus-cyber-attack-leaves-customers-feeling-powerless-over-risk-of-identity-theft}.
%
%\bibitem{leigh2015hsbc}
%Leigh, D., Ball, J., Garside, J., Pegg, D.: {HSBC} files timeline: From {Swiss}
%  bank leak to fallout.
%\newblock The Guardian {\bf 12} (2015).
%
%\bibitem{NYT-facial-rec}
%Murphy, H.:.
%\newblock Whatever happened to those self-service passport kiosks at airports?
%  2022.
%\newblock
%  \url{https://www.nytimes.com/2022/10/05/travel/customs-kiosks-facial-recognition.html}.
%
%\bibitem{NaorP00}
%Naor, M., Pinkas, B.:.
%\newblock Distributed oblivious transfer.
%\newblock In Advances in Cryptology - {ASIACRYPT} 2000, 6th International
%  Conference on the Theory and Application of Cryptology and Information
%  Security, Kyoto, Japan, December 3-7, 2000, Proceedings (2000) vol.~1976 of
%  Lecture Notes in Computer Science Springer pp.~205--219.
%
%\bibitem{Efficient-OT-Naor}
%Naor, M., Pinkas, B.:.
%\newblock Efficient oblivious transfer protocols.
%\newblock SODA '01 Society for Industrial and Applied Mathematics.
%
%\bibitem{Desjardins}
%{Office of the Privacy Commissioner of Canada}:.
%\newblock Investigation into {Desjardins}’ compliance with {PIPEDA} following
%  a breach of personal information between 2017 and 2019 2020.
%\newblock
%  \url{https://www.priv.gc.ca/en/opc-actions-and-decisions/investigations/investigations-into-businesses/2020/pipeda-2020-005/}.
%
%\bibitem{perlman2010privacy}
%Perlman, R., Kaufman, C., Perlner, R.:.
%\newblock Privacy-preserving {DRM}.
%\newblock In Proceedings of the 9th Symposium on Identity and Trust on the
%  Internet (2010).
%
%\bibitem{Shamir79}
%Shamir, A.: How to share a secret.
%\newblock Commun. ACM {\bf 22} (1979) 612--613.
%
%\bibitem{Shannon49}
%Shannon, C.~E.: Communication theory of secrecy systems.
%\newblock Bell System Techn. Jour. {\bf 28} (1949) 656--715.
%
%\bibitem{Singapore}
%{Syam Roslan}:.
%\newblock Let's fight scams 2020.
%\newblock \url{https://www.police.gov.sg/media-room/features/lets-fight-scams}.
%
%\bibitem{bitcoin-hack-3}
%Tidy, J.:.
%\newblock Ronin network: What a \$600m hack says about the state of crypto
%  2022.
%\newblock \url{https://www.bbc.co.uk/news/technology-60933174}.
%
%\bibitem{Tzeng02}
%Tzeng, W.:.
%\newblock Efficient 1-out-n oblivious transfer schemes.
%\newblock In Public Key Cryptography, 5th International Workshop on Practice
%  and Theory in Public Key Cryptosystems, {PKC} 2002, Paris, France, February
%  12-14, 2002, Proceedings (2002) D.~Naccache and P.~Paillier, Eds. Lecture
%  Notes in Computer Science.
%
%\bibitem{2021-Half-Year-Fraud-Update}
%{UK Finance}:.
%\newblock 2021 half year fraud update 2021.\\
%\newblock
%  \url{https://www.ukfinance.org.uk/system/files/Half-year-fraud-update-2021-FINAL.pdf}.
%
%\bibitem{FT-scams}
%Venkataramakrishnan, S.:.
%\newblock Regulator to force {UK} banks to offer scam victims compensation
%  2022.
%\newblock
%  \url{https://www.ft.com/content/aabeea7a-324c-4850-a91d-fc41aa6d8802}.
%
%\bibitem{WuMB99}
%Wu, T.~D., Malkin, M., Boneh, D.:.
%\newblock Building intrusion-tolerant applications.
%\newblock In Proceedings of the 8th {USENIX} Security Symposium, Washington,
%  DC, USA, August 23-26, 1999 (1999) {USENIX} Association.
%
%\bibitem{OT-Survey}
%Yadav, V.~K., Andola, N., Verma, S., Venkatesan, S.: A survey of oblivious
%  transfer protocol.
%\newblock ACM Comput. Surv. (2022).
%
%\end{thebibliography}




==> properties-definition-DQ-OT.tex <==


\subsection{Formal Definitions of Efficiency and Sender-Push Communication in \dqot}\label{sec::properties-definitions}



\begin{definition}[Efficiency]\label{def::efficiency}
A \dqot scheme is considered efficient if the running time of the receiver-side request (or query) generation algorithm, denoted as $\mathtt{Request(1^{\st \lambda}, s, pk)}$, satisfies two conditions: 

\begin{enumerate}[label=$\bullet$,leftmargin=4.7mm]
    \item The running time is upper-bounded by $poly(|{m}|)$, where $poly$ is a fixed polynomial, $m$ is a tuple of messages that the sender holds, and $|{m}|$ represents the number of elements/messages in tuple $m$. 

    
    \item The running time is asymptotically constant with respect to the security parameter $\lambda$, i.e., it is $O(1)$.  
\end{enumerate}
\end{definition}

 

% \begin{definition}[Efficiency]\label{def::efficiency}
% A \dqot scheme is efficient if the running time of client-side request (or query) generation algorithm $\mathtt{Request(1^{\st \lambda}, s, pk)}$ is (i) upper bounded by $poly(|{m}|)$, where $poly$ is a fixed polynomial and ${m}=(m_{\st 0}, m_{\st 1})$, and (ii) $O(1)$ with respect to the security parameter $\lambda$. 
% \end{definition}



\begin{definition}[Sender-push communication]\label{def::Server-push-comm} Let 
%
(a) $\mathtt{Action}_{\st \re}(t)$ represents the set of actions available to \re at time $t$ (these actions may include sending requests, receiving messages, or any other interactions \re can perform within the scheme's execution), 
%
(b) $\mathtt{Action}_{\st \se}(t)$ be the set of actions available to \se at time $t$,  
%
(c) $\mathtt{SendRequest}(\re,\se)$ be the action of \re sending a request to \se, and 
%
(d) $\mathtt{SendMessage}(\se,\re)$ represents the action of \se sending a message to \re. Then, we say that a \dqot scheme supports sender-push communication, if it meets the following conditions: 


\begin{enumerate}[label=$\bullet$,leftmargin=4.7mm]

\item \textit{Receiver-side restricted interaction}: 
%
For all $t$ in the communication timeline (i.e., within the execution of the scheme), the set of actions $\mathtt{Action}_{\st \re}(t)$ available to the receiver \re is restricted such that it does not include direct requests to the sender \se. Formally,
%
$$\forall t: \mathtt{Action}_{\st \re}(t) \cap \{\mathtt{SendRequest}(\re,\se)\}=\emptyset$$

\item \textit{Sender-side non-restricted interaction}: 
%
For all $t$ in the communication timeline, the sender \se has the capability to push messages to the receiver \re without receiving explicit request directly from \re. Formally, 
%
$$\forall t:
\mathtt{Action}_{\st \se}(t) \subseteq \{\mathtt{SendMessage}(\se,\re)\}
$$


\end{enumerate}


\end{definition}

Note that above two definitions are valid for the variants of \dqot; namely, \duqot, \dqothf, and  \duqothf, with a minor difference being that the receiver-side request generation algorithm in these three variants is denoted as $\mathtt{\re.Request}()$.
